The DESI Early Data Release White Dwarf Catalogue

The Early Data Release (EDR) of the Dark Energy Spectroscopic Instrument (DESI) comprises spectroscopy obtained from 2020 December 14 to 2021 June 10. White dwarfs were targeted by DESI both as calibration sources and as science targets and were selected based on Gaia photometry and astrometry. Here we present the DESI EDR white dwarf catalogue, which includes 2706 spectroscopically confirmed white dwarfs of which approximately 1630 (roughly 60 per cent) have been spectroscopically observed for the first time, as well as 66 white dwarf binary systems. We provide spectral classifications for all white dwarfs, and discuss their distribution within the Gaia Hertzsprung-Russell diagram. We provide atmospheric parameters derived from spectroscopic and photometric fits for white dwarfs with pure hydrogen or helium photospheres, a mixture of those two, and white dwarfs displaying carbon features in their spectra. We also discuss the less abundant systems in the sample, such as those with magnetic fields, and cataclysmic variables. The DESI EDR white dwarf sample is significantly less biased than the sample observed by the Sloan Digital Sky Survey, which is skewed to bluer and therefore hotter white dwarfs, making DESI more complete and suitable for performing statistical studies of white dwarfs.

==> DZ_text.tex <==
\subsubsection{The fraction of planetary systems around white dwarfs determined using cool DZs}
 
Helium-atmosphere white dwarfs that display only the signatures of metals, dominated by the DZ spectral class, are relatively easy to identify, with Ca abundances being detectable several orders of magnitude lower than their hotter DBZ counterparts \citep{dufouretal07-2,koester+kepler15-1, hollandsetal17-1}. Additionally, the convection zones of DZs are deep, leading to long diffusion timescales for metals to sink out of their atmosphere \citep{koester09-1}. The ease of detecting metals in addition to their relatively long presence after accretion in the photosphere make them good proxies for determining limits on the occurence rate of planetary systems around white dwarfs. A lower limit on the frequency of planetary systems around white dwarfs has been previously determined utilising samples of warmer DA white dwarfs \citep{zuckermanetal03-1, koesteretal14-1} and was estimated between $\simeq$25\,--\,50\,per\,cent. These studies relied on high resolution ground-based spectroscopy or ultraviolet space-based spectroscopy.
 
If a DZ ceases accretion and loses all of its atmospheric metals to diffusion, it will either transition into a featureless DC white dwarf or a DQ showing molecular carbon features. \cite{hollandsetal22-1} and \cite{blouinetal22-1} have shown that carbon features and abundances consistent with dredge-up can be eradicated from the emergent optical spectrum of white dwarfs due to the presence of metals. At low enough metal abundances, carbon features start to become apparent such as in the DZQ WD\,J101453.59+411416.94 and the DQZ WD\,J142018.91+324921.12 we have identified with DESI. This is thought to be the reason metal-polluted DQs appear to be so rare.
 
Based on these arguments, we estimate the fraction, $f$, of cool polluted helium-atmosphere white dwarfs as the number of DZ, DQZ, and DZQ white dwarfs divided by both the number of these polluted systems and the number of the types they would appear as without the accretion of planetary bodies - DCs and DQs, $f = (n_\mathrm{DZ} + n_\mathrm{DQZ} + n_\mathrm{DZQ})/(n_\mathrm{DC} + n_\mathrm{DQ} + n_\mathrm{DZ} + n_\mathrm{DQZ} + n_\mathrm{DZQ})$. We limit the determination of $f$ to the range of \textit{Gaia} colours $0 < (G_\mathrm{BP} - G_\mathrm{RP}) < 1$ to capture the range in which we detect DZs, while excluding hotter DQs thought to be produced in binary mergers and redder DCs potentially dominated by hydrogen-rich atmosphere white dwarfs (see Section\,\ref{sec:WD_cat} for discussion on DCs and DQs). For helium-dominated atmospheric models with no carbon or metals, the $(G_\mathrm{BP} - G_\mathrm{RP})$ colour range spans the broad temperature range of $\simeq$\,$12000$\,K $> T_{\mathrm{eff}} > 5000$\,K. In this range we have 48 DZs, 1 DQZ, 1 DZQ, 141 DCs and 43 DQs for a total of 234 systems. This results in a lower limit on the percentage of white dwarfs hosting planetary systems of $(f \times 100)$\,=\,21\,$\pm$\,3\,per\,cent. This value is in good agreement with the lower limit on the fraction of planetary systems around white dwarfs determined using DA white dwarfs.
 
The calculations here rely on the zeroth-order assumption that DZ, DQ, DQZ/DZQ, and DC white dwarfs in the colour range we select also share the same approximate $T_\mathrm{eff}$ range. This is a relatively poor assumption for extremely polluted DZs where the Ca\,H\,\&\,K lines saturate the blue end of the optical spectrum, and some of the more extreme DQs in our sample. We investigate the dependence of $f$ on $(G_\mathrm{BP} - G_\mathrm{RP})$ in Fig.\,\ref{fig:DZfrac}, where we calculate $f$ as a running-fraction in the range $0 < (G_\mathrm{BP} - G_\mathrm{RP}) < 1$ with a bin size of 0.3. $f$ varies between $\simeq$15\,--\,25\,per\,cent throughout this colour range, which would suggest our assumptions do not drastically affect our value of $f$.
 
We expect an order of magnitude increase in the number of white dwarfs from data release 1 (DR1) of DESI, which will allow us to probe the frequency of planetary systems around white dwarfs using this method in much more detail, and with additional atmospheric modelling will allow us to determine trends in planetary occurence rates as a function of $T_\mathrm{eff}$, system age, and host-star mass.
 
\begin{figure}
    \includegraphics[width=1\columnwidth]{Figs_CJM/planet_fraction_HRD.pdf}
    \caption{\textbf{Bottom panel:} The fraction of polluted DCs and DQs as a function of $G_\textrm{BP}$ -- $G_\textrm{RP}$ used as a zeroth order proxy for $T_\mathrm{eff}$. The fraction is computed using a bin width of 0.3 (thick black line), and runs from bin centers of 0.15 to 0.85 to cover the range $0 < (G_\mathrm{BP} - G_\mathrm{RP}) < 1$. The horizontal black dashed line is set to the value of $f = (n_\mathrm{DZ}+ n_\mathrm{DQZ} +n_\mathrm{DZQ})/(n_\mathrm{DC} + n_\mathrm{DQ} + n_\mathrm{DZ}+n_\mathrm{DQZ} +n_\mathrm{DZQ}) = 0.21$. \textbf{Top panel:} The \textit{Gaia} HRD showing the polluted (orange triangles) and non-polluted (gray circles) systems used in the calculation of $f$.}
    \label{fig:DZfrac}
\end{figure}

==> contaminant.tex <==
\begin{table*}
\centering
\caption{Placeholder table for contaminants. Gaia data from Nicola's DR3 WD catalogue. Systems from DR2 WD catalogue not reproduced in the DR3 one have '--'. \label{t-WD1}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ003748.95+421102.69 & DUNNO   & 381560256012678272  & 17.961 (0.003) & 0.5681            \\
WDJ013230.30+303446.96 & DUNNO   & --                  & --             & --                \\
WDJ013354.76+320327.04 & STAR    & --                  & --             & --                \\
WDJ013428.73+232120.02 & DUNNO   & 290110266157914880  & 18.665 (0.004) & 0.9977            \\
WDJ013814.00+315247.99 & EXGAL   & --                  & --             & --                \\
WDJ014143.41+320231.97 & DUNNO   & 303909583762954368  & 17.863 (0.003) & 0.9924            \\
WDJ015354.95-022537.70 & STAR    & --                  & --             & --                \\
WDJ015542.95-032832.36 & EXGAL   & --                  & --             & --                \\
WDJ020100.39-033405.39 & STAR    & 2492566506248972544 & 19.939 (0.006) & 0.0503            \\
WDJ020329.50-074128.36 & DUNNO   & 2463435289268619008 & 18.141 (0.003) & 0.9928            \\
WDJ020352.48-073523.18 & STAR    & --                  & --             & --                \\
WDJ020407.94-073924.02 & STAR    & --                  & --             & --                \\
WDJ020427.27-060328.06 & STAR    & --                  & --             & --                \\
WDJ020718.69-050814.50 & STAR    & --                  & --             & --                \\
WDJ022453.77+305852.63 & EXGAL   & --                  & --             & --                \\
WDJ022652.56-061907.54 & UNCLASS & 2488355101836762752 & 19.648 (0.005) & 0.1718            \\
WDJ022807.62-071557.20 & STAR    & --                  & --             & --                \\
WDJ022902.91-041628.48 & EXGAL   & --                  & --             & --                \\
WDJ023010.00-045652.90 & STAR    & --                  & --             & --                \\
WDJ023041.69-041920.21 & EXGAL   & --                  & --             & --                \\
WDJ023120.04-040000.59 & STAR    & --                  & --             & --                \\
WDJ023222.43+263419.53 & EXGAL   & --                  & --             & --                \\
WDJ023324.57-003852.72 & UNCLASS & --                  & --             & --                \\
WDJ023417.43+003857.98 & UNCLASS & 2500531269696983296 & 19.879 (0.006) & 0.0766            \\
WDJ023554.22-040046.09 & STAR    & 2495096383720814464 & 19.940 (0.006) & 0.7613            \\
WDJ023602.27-013450.26 & EXGAL   & --                  & --             & --                \\
WDJ023626.59-033243.03 & STAR    & 2495326112931510016 & 18.636 (0.004) & 0.0766            \\
WDJ023701.46+011414.77 & UNCLASS & --                  & --             & --                \\
WDJ053941.49-193804.95 & EXGAL   & --                  & --             & --                \\
WDJ054244.63-190436.43 & UNCLASS & --                  & --             & --                \\
WDJ055009.83-233802.25 & EXGAL   & --                  & --             & --                \\
WDJ055034.13-214431.76 & DUNNO   & 2917615883114362752 & 18.667 (0.003) & 0.2697            \\
WDJ055130.86-231505.94 & STAR    & --                  & --             & --                \\
WDJ065837.72+571235.89 & DUNNO   & 1000497070938042496 & 16.214 (0.003) & 0.0221            \\
WDJ065942.66+572408.19 & STAR    & --                  & --             & --                \\
WDJ070207.74+365145.94 & EXGAL   & --                  & --             & --                \\
WDJ070358.22+564451.57 & STAR    & 1000503594992328576 & 19.630 (0.007) & 0.2429            \\
WDJ070415.77+572903.78 & STAR    & --                  & --             & --                \\
WDJ070617.53+570800.62 & EXGAL   & --                  & --             & --                \\
WDJ071055.69+545338.02 & EXGAL   & --                  & --             & --                \\
WDJ071200.21+565656.87 & EXGAL   & --                  & --             & --                \\
WDJ072859.56+433719.07 & STAR    & --                  & --             & --                \\
WDJ073222.20+310556.18 & UNCLASS & --                  & --             & --                \\
WDJ073246.05+180831.49 & EXGAL   & --                  & --             & --                \\
WDJ073717.69+395858.25 & DUNNO   & 923592241233927040  & 19.901 (0.005) & 0.9911            \\
WDJ073827.39+152629.77 & EXGAL   & --                  & --             & --                \\
WDJ074035.04+162837.42 & EXGAL   & --                  & --             & --                \\
WDJ074236.21+181117.76 & STAR    & --                  & --             & --                \\
WDJ074251.98+331354.23 & DUNNO   & 894000363240700800  & 19.768 (0.005) & 0.9987            \\
WDJ074253.55+182159.10 & EXGAL   & --                  & --             & --                \\
WDJ074410.51+383247.31 & STAR    & 920174924734438272  & 19.876 (0.011) & 0.9447            \\
WDJ074508.10+692351.75 & UNCLASS & 1098125177973318272 & 19.810 (0.004) & 0.9945            \\
WDJ075030.98+684108.79 & DUNNO   & 1096533467390090880 & 19.724 (0.004) & 0.9934            \\
WDJ080102.79+393343.66 & STAR    & --                  & --             & --                \\
WDJ080537.13+401756.92 & STAR    & 921213791424420992  & 19.959 (0.006) & 0.0679            \\
WDJ081547.91+333046.28 & EXGAL   & --                  & --             & --                \\
WDJ081642.27+315841.36 & EXGAL   & --                  & --             & --                \\
WDJ081728.65+310628.19 & EXGAL   & --                  & --             & --                \\
WDJ082048.28+332414.29 & EXGAL   & --                  & --             & --                \\
WDJ082423.26+311334.12 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ082649.62+323054.61 & EXGAL   & --                  & --             & --                \\
WDJ082847.12+312328.75 & EXGAL   & --                  & --             & --                \\
WDJ082939.55+335031.55 & STAR    & --                  & --             & --                \\
WDJ083047.51+331454.93 & STAR    & 710936143981579136  & 19.509 (0.004) & 0.3851            \\
WDJ083053.71+012308.09 & STAR    & --                  & --             & --                \\
WDJ083107.92+001331.38 & DUNNO   & 3076962575704962176 & 17.922 (0.003) & 0.8185            \\
WDJ083217.88+334307.83 & STAR    & 710974592529008896  & 19.916 (0.006) & 0.0392            \\
WDJ083541.60+312147.88 & STAR    & --                  & --             & --                \\
WDJ083709.10+201159.48 & STAR    & --                  & --             & --                \\
WDJ083819.26+184608.88 & STAR    & 659690312192901760  & 19.870 (0.005) & 0.0520            \\
WDJ084014.86+004239.04 & DUNNO   & 3078353045597053696 & 16.474 (0.003) & 0.0514            \\
WDJ084019.25-055512.20 & STAR    & --                  & --             & --                \\
WDJ084110.90+202912.32 & STAR    & --                  & --             & --                \\
WDJ084242.27-071615.43 & STAR    & --                  & --             & --                \\
WDJ084306.22+184245.44 & STAR    & --                  & --             & --                \\
WDJ084330.82+201049.27 & DUNNO   & 661386274519054464  & 18.504 (0.003) & 0.9972            \\
WDJ084736.00+232510.39 & EXGAL   & --                  & --             & --                \\
WDJ084752.12+192318.93 & STAR    & --                  & --             & --                \\
WDJ084829.65+100054.73 & STAR    & --                  & --             & --                \\
WDJ084912.41+220717.01 & STAR    & --                  & --             & --                \\
WDJ085148.56+095035.22 & DUNNO   & 597684526470998272  & 19.044 (0.003) & 0.9949            \\
WDJ085413.16+085352.94 & DUNNO   & 597324024095840512  & 15.475 (0.003) & 0.6789            \\
WDJ085444.16+001522.92 & STAR    & --                  & --             & --                \\
WDJ085651.76+315048.61 & EXGAL   & --                  & --             & --                \\
WDJ090041.93+011550.88 & UNCLASS & 576696563188488576  & 19.869 (0.005) & 0.9951            \\
WDJ090044.35+311401.98 & STAR    & --                  & --             & --                \\
WDJ091328.49+312942.17 & STAR    & --                  & --             & --                \\
WDJ091354.30-002541.59 & EXGAL   & --                  & --             & --                \\
WDJ091615.62+324101.03 & STAR    & --                  & --             & --                \\
WDJ091913.69+332455.76 & STAR    & --                  & --             & --                \\
WDJ092038.25+322845.82 & EXGAL   & --                  & --             & --                \\
WDJ092427.94+330155.21 & EXGAL   & --                  & --             & --                \\
WDJ092558.25+315907.22 & STAR    & --                  & --             & --                \\
WDJ092611.67+330757.38 & EXGAL   & --                  & --             & --                \\
WDJ092741.00+310516.60 & STAR    & --                  & --             & --                \\
WDJ092841.50+320558.02 & EXGAL   & --                  & --             & --                \\
WDJ093006.80+314258.35 & DUNNO   & 697904599026844160  & 17.254 (0.003) & 0.1235            \\
WDJ093033.77+634004.41 & EXGAL   & --                  & --             & --                \\
WDJ093106.58+684430.96 & DUNNO   & 1071012698700981120 & 19.887 (0.004) & 0.9744            \\
WDJ093559.83+685201.55 & DUNNO   & 1070853961005794048 & 16.665 (0.003) & 0.9762            \\
WDJ094111.52+331443.86 & STAR    & --                  & --             & --                \\
WDJ094146.01+310915.12 & STAR    & --                  & --             & --                \\
WDJ094725.25+650036.77 & EXGAL   & --                  & --             & --                \\
WDJ094954.65+692017.89 & EXGAL   & --                  & --             & --                \\
WDJ095034.25+323505.93 & STAR    & --                  & --             & --                \\
WDJ095235.30+313033.79 & EXGAL   & --                  & --             & --                \\
WDJ095405.84+312505.68 & EXGAL   & --                  & --             & --                \\
WDJ095430.39+021526.06 & EXGAL   & --                  & --             & --                \\
WDJ095451.89+331600.46 & STAR    & --                  & --             & --                \\
WDJ095523.98+013654.36 & EXGAL   & --                  & --             & --                \\
WDJ095526.24+014651.49 & EXGAL   & --                  & --             & --                \\
WDJ095553.82+321004.98 & STAR    & --                  & --             & --                \\
WDJ095617.05+693217.50 & EXGAL   & --                  & --             & --                \\
WDJ095619.73+032059.25 & STAR    & --                  & --             & --                \\
WDJ095622.29+311958.43 & STAR    & --                  & --             & --                \\
WDJ095632.68+032152.83 & EXGAL   & --                  & --             & --                \\
WDJ095637.29+312104.34 & EXGAL   & --                  & --             & --                \\
WDJ095657.70+033213.08 & UNCLASS & --                  & --             & --                \\
WDJ095724.28+362133.05 & STAR    & --                  & --             & --                \\
WDJ095733.31+334421.82 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ095836.57+354414.53 & EXGAL   & --                  & --             & --                \\
WDJ095945.68+320242.74 & STAR    & 746561557672860032  & 19.439 (0.004) & 0.8288            \\
WDJ095951.21+034701.53 & EXGAL   & --                  & --             & --                \\
WDJ100005.13+324024.98 & EXGAL   & --                  & --             & --                \\
WDJ100108.69+005730.78 & EXGAL   & --                  & --             & --                \\
WDJ100114.82+382054.95 & EXGAL   & --                  & --             & --                \\
WDJ100115.45+321950.74 & EXGAL   & --                  & --             & --                \\
WDJ100317.06+025510.33 & DUNNO   & --                  & --             & --                \\
WDJ100341.36+013846.52 & STAR    & --                  & --             & --                \\
WDJ100415.27+395403.68 & STAR    & --                  & --             & --                \\
WDJ100420.51+022436.34 & STAR    & --                  & --             & --                \\
WDJ100438.01+020924.36 & EXGAL   & --                  & --             & --                \\
WDJ100448.49+010232.56 & STAR    & --                  & --             & --                \\
WDJ101232.09+002209.09 & STAR    & 3831884643701293184 & 18.309 (0.004) & 0.8633            \\
WDJ101355.61-001306.47 & DUNNO   & 3831559256977842560 & 18.672 (0.004) & 0.9968            \\
WDJ101356.31+405926.82 & STAR    & --                  & --             & --                \\
WDJ101428.51-004631.85 & STAR    & --                  & --             & --                \\
WDJ102104.99+440355.48 & EXGAL   & --                  & --             & --                \\
WDJ102143.03+322227.35 & EXGAL   & --                  & --             & --                \\
WDJ102431.10+332150.24 & EXGAL   & --                  & --             & --                \\
WDJ102431.94+803138.76 & UNCLASS & --                  & --             & --                \\
WDJ102459.67+424316.60 & STAR    & --                  & --             & --                \\
WDJ102642.72+101540.23 & STAR    & --                  & --             & --                \\
WDJ103225.18-241109.21 & EXGAL   & --                  & --             & --                \\
WDJ103243.85+321003.00 & STAR    & --                  & --             & --                \\
WDJ103303.62+321554.02 & EXGAL   & --                  & --             & --                \\
WDJ103314.77-260526.33 & EXGAL   & --                  & --             & --                \\
WDJ103644.42-261506.71 & DUNNO   & 5468473341906356096 & 18.559 (0.004) & 0.2978            \\
WDJ103742.46+102023.65 & EXGAL   & --                  & --             & --                \\
WDJ103747.64+332825.46 & STAR    & --                  & --             & --                \\
WDJ103756.62-251123.94 & STAR    & --                  & --             & --                \\
WDJ104222.98+802002.82 & UNCLASS & --                  & --             & --                \\
WDJ104408.90+803445.05 & UNCLASS & 1133175581442675200 & 19.717 (0.005) & 0.9491            \\
WDJ104754.06+802834.62 & UNCLASS & 1133160085200468736 & 19.867 (0.005) & 0.9951            \\
WDJ104814.66+470140.92 & STAR    & --                  & --             & --                \\
WDJ104849.94+784321.42 & UNCLASS & 1129680680654544256 & 19.418 (0.004) & 0.9867            \\
WDJ105405.41-263659.09 & STAR    & 5457849379522645120 & 19.740 (0.006) & 0.2841            \\
WDJ105416.72+792239.60 & UNCLASS & 1132809925106843008 & 19.637 (0.005) & 0.9966            \\
WDJ105453.29+783025.72 & UNCLASS & 1129706622256790400 & 19.576 (0.004) & 0.9782            \\
WDJ105528.60+323147.77 & EXGAL   & --                  & --             & --                \\
WDJ105555.25+484739.90 & DUNNO   & 832680191738024192  & 17.035 (0.003) & 0.9796            \\
WDJ105644.54+330221.04 & EXGAL   & --                  & --             & --                \\
WDJ105704.73+804944.52 & UNCLASS & 1133196716976678016 & 19.946 (0.005) & 0.9674            \\
WDJ105711.65+471119.60 & STAR    & --                  & --             & --                \\
WDJ105714.85+802810.20 & UNCLASS & --                  & --             & --                \\
WDJ105715.92+332742.17 & STAR    & --                  & --             & --                \\
WDJ105741.78+325809.46 & EXGAL   & --                  & --             & --                \\
WDJ105751.50+520547.50 & STAR    & 836498039709296512  & 20.088 (0.005) & 0.9183            \\
WDJ105752.17+503115.28 & STAR    & --                  & --             & --                \\
WDJ105759.37+470307.40 & DUNNO   & 831501240400109824  & 17.217 (0.003) & 0.0442            \\
WDJ105817.24+784951.16 & UNCLASS & 1129729785016172288 & 19.796 (0.005) & 0.9667            \\
WDJ105822.62+320450.83 & STAR    & --                  & --             & --                \\
WDJ105853.96+524300.20 & STAR    & 837281093848812672  & 20.340 (0.005) & 0.5169            \\
WDJ105947.75+705911.07 & DUNNO   & 1073746913536371456 & 19.721 (0.005) & 0.6631            \\
WDJ110011.55+515807.94 & EXGAL   & --                  & --             & --                \\
WDJ110147.00+523934.40 & STAR    & 836541779656234368  & 20.327 (0.006) & 0.9939            \\
WDJ110217.42+505825.39 & STAR    & --                  & --             & --                \\
WDJ110236.64+313149.24 & STAR    & --                  & --             & --                \\
WDJ110255.97+521858.12 & DUNNO   & --                  & --             & --                \\
WDJ110309.63+522445.17 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ110333.58+501518.79 & STAR    & --                  & --             & --                \\
WDJ110346.23+784444.51 & DUNNO   & 1129735763610587264 & 19.661 (0.005) & 0.9653            \\
WDJ110414.01+502932.83 & EXGAL   & --                  & --             & --                \\
WDJ110442.90+524556.86 & EXGAL   & --                  & --             & --                \\
WDJ110505.06+792610.72 & DUNNO   & 1129832000941901056 & 19.129 (0.004) & 0.9611            \\
WDJ110527.70+523804.66 & EXGAL   & --                  & --             & --                \\
WDJ110538.37+500517.70 & STAR    & --                  & --             & --                \\
WDJ110603.25+504553.32 & STAR    & 839095219315053824  & 19.735 (0.004) & 0.9927            \\
WDJ110605.76+694225.68 & EXGAL   & --                  & --             & --                \\
WDJ110639.56+524110.56 & EXGAL   & 842508004625241216  & 19.979 (0.005) & 0.1531            \\
WDJ110641.42+735406.05 & DUNNO   & 1078949626465580416 & 19.263 (0.004) & 0.9588            \\
WDJ110758.92+320635.42 & STAR    & --                  & --             & --                \\
WDJ110800.64+501400.22 & STAR    & 838826393018353152  & 17.429 (0.003) & 0.9893            \\
WDJ110945.71+505424.48 & DUNNO   & 838922389831369216  & 18.616 (0.003) & 0.9992            \\
WDJ111016.81+524319.23 & EXGAL   & --                  & --             & --                \\
WDJ111058.51+502053.29 & DUNNO   & 838840510574586880  & 17.542 (0.003) & 0.9980            \\
WDJ111752.16+550937.79 & DUNNO   & 843967876892449920  & 19.911 (0.004) & 0.9755            \\
WDJ111823.74+514758.63 & EXGAL   & --                  & --             & --                \\
WDJ111953.57+515718.19 & EXGAL   & --                  & --             & --                \\
WDJ112119.68+540313.57 & EXGAL   & --                  & --             & --                \\
WDJ112157.25+534038.70 & EXGAL   & --                  & --             & --                \\
WDJ112202.34+323819.55 & STAR    & --                  & --             & --                \\
WDJ112341.02+315151.26 & STAR    & --                  & --             & --                \\
WDJ112341.64+333508.80 & STAR    & 759138699383421184  & 19.437 (0.005) & 0.0865            \\
WDJ112445.61+320821.88 & STAR    & --                  & --             & --                \\
WDJ112457.14+504906.75 & EXGAL   & --                  & --             & --                \\
WDJ112517.83+330936.50 & EXGAL   & --                  & --             & --                \\
WDJ112534.12+792005.08 & DUNNO   & 1129965488525849344 & 19.460 (0.004) & 0.9925            \\
WDJ112547.95+512640.08 & EXGAL   & --                  & --             & --                \\
WDJ112649.30+332108.15 & EXGAL   & --                  & --             & --                \\
WDJ112715.67+504350.53 & STAR    & --                  & --             & --                \\
WDJ112757.71+493155.06 & EXGAL   & --                  & --             & --                \\
WDJ112810.26+305354.11 & STAR    & 4023468153928538240 & 19.914 (0.006) & 0.0566            \\
WDJ112838.24+531757.77 & EXGAL   & --                  & --             & --                \\
WDJ112849.66+325040.41 & STAR    & --                  & --             & --                \\
WDJ112941.08+503637.93 & EXGAL   & --                  & --             & --                \\
WDJ112949.37+493526.15 & EXGAL   & --                  & --             & --                \\
WDJ112954.40+515114.45 & EXGAL   & --                  & --             & --                \\
WDJ112954.78+510000.26 & DUNNO   & 838410876406247680  & 17.719 (0.003) & 0.9788            \\
WDJ113113.64+531536.02 & EXGAL   & --                  & --             & --                \\
WDJ113222.22+803338.10 & DUNNO   & 1133360161957024768 & 19.075 (0.004) & 0.9970            \\
WDJ113242.88+545222.67 & EXGAL   & --                  & --             & --                \\
WDJ113256.43+320724.16 & STAR    & --                  & --             & --                \\
WDJ113313.31+525551.90 & EXGAL   & --                  & --             & --                \\
WDJ113521.78+525120.11 & EXGAL   & --                  & --             & --                \\
WDJ113525.12+532109.66 & EXGAL   & --                  & --             & --                \\
WDJ113600.30+513621.95 & EXGAL   & --                  & --             & --                \\
WDJ113624.05+500356.74 & EXGAL   & --                  & --             & --                \\
WDJ113633.61+750653.85 & DUNNO   & 1079494159598957952 & 13.153 (0.003) & 0.0244            \\
WDJ113651.04+555245.21 & EXGAL   & --                  & --             & --                \\
WDJ113658.15+493449.24 & STAR    & --                  & --             & --                \\
WDJ113714.33+535105.07 & EXGAL   & --                  & --             & --                \\
WDJ113723.10+503603.82 & STAR    & --                  & --             & --                \\
WDJ113854.07+535051.08 & EXGAL   & --                  & --             & --                \\
WDJ113855.13+535530.19 & DUNNO   & --                  & --             & --                \\
WDJ113927.30+003127.36 & STAR    & --                  & --             & --                \\
WDJ113948.99+801423.48 & DUNNO   & 1130293830185522432 & 19.778 (0.005) & 0.6734            \\
WDJ113949.44+510038.37 & EXGAL   & --                  & --             & --                \\
WDJ114026.18+510231.59 & EXGAL   & --                  & --             & --                \\
WDJ114038.69+541146.11 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ114113.63+005138.31 & STAR    & --                  & --             & --                \\
WDJ114118.50+510719.17 & EXGAL   & --                  & --             & --                \\
WDJ114118.98+551048.91 & EXGAL   & --                  & --             & --                \\
WDJ114127.80+510232.11 & EXGAL   & --                  & --             & --                \\
WDJ114128.97+531623.95 & STAR    & 840359588967666432  & 19.037 (0.003) & 0.0593            \\
WDJ114233.30+533045.38 & EXGAL   & --                  & --             & --                \\
WDJ114330.72+542510.07 & STAR    & --                  & --             & --                \\
WDJ114345.00+532121.64 & EXGAL   & --                  & --             & --                \\
WDJ114402.68+533811.63 & EXGAL   & --                  & --             & --                \\
WDJ114429.18+523958.42 & EXGAL   & --                  & --             & --                \\
WDJ114434.83+550439.30 & DUNNO   & 841328602308941184  & 18.761 (0.003) & 0.4427            \\
WDJ114435.30+532704.97 & EXGAL   & --                  & --             & --                \\
WDJ114554.88+001024.09 & DUNNO   & 3795661576720589184 & 19.461 (0.005) & 0.9952            \\
WDJ114609.78+562524.60 & STAR    & --                  & --             & --                \\
WDJ114620.14+004059.13 & EXGAL   & --                  & --             & --                \\
WDJ114624.29+693549.76 & DUNNO   & 1061506737779866624 & 19.832 (0.005) & 0.9906            \\
WDJ114645.75+561644.50 & EXGAL   & --                  & --             & --                \\
WDJ114653.48+511028.96 & EXGAL   & --                  & --             & --                \\
WDJ114902.19+512121.30 & EXGAL   & --                  & --             & --                \\
WDJ114945.24+505023.26 & EXGAL   & --                  & --             & --                \\
WDJ115205.17+562405.80 & EXGAL   & --                  & --             & --                \\
WDJ115229.65-004110.21 & EXGAL   & --                  & --             & --                \\
WDJ115233.98+552245.48 & EXGAL   & --                  & --             & --                \\
WDJ115306.42+534947.92 & EXGAL   & --                  & --             & --                \\
WDJ115320.77+512345.90 & EXGAL   & --                  & --             & --                \\
WDJ115331.13+521837.75 & EXGAL   & --                  & --             & --                \\
WDJ115404.20+510635.27 & EXGAL   & --                  & --             & --                \\
WDJ115457.54+522257.60 & EXGAL   & --                  & --             & --                \\
WDJ115537.61+550215.87 & EXGAL   & --                  & --             & --                \\
WDJ115618.80+531302.40 & EXGAL   & --                  & --             & --                \\
WDJ115625.45+520355.77 & EXGAL   & --                  & --             & --                \\
WDJ115708.14+521424.35 & EXGAL   & --                  & --             & --                \\
WDJ115733.96+282754.96 & STAR    & 4007951674038723840 & 19.239 (0.004) & 0.1924            \\
WDJ115737.52+541754.98 & EXGAL   & --                  & --             & --                \\
WDJ115745.10-002147.22 & EXGAL   & --                  & --             & --                \\
WDJ115752.39+763448.07 & DUNNO   & 1079731727125032064 & 19.870 (0.004) & 0.9948            \\
WDJ115818.08+571939.31 & EXGAL   & --                  & --             & --                \\
WDJ115819.47-010411.12 & STAR    & --                  & --             & --                \\
WDJ115825.27+273027.80 & STAR    & --                  & --             & --                \\
WDJ115828.03-000513.05 & STAR    & --                  & --             & --                \\
WDJ115829.09+003305.33 & STAR    & --                  & --             & --                \\
WDJ115915.21+293219.57 & EXGAL   & --                  & --             & --                \\
WDJ120006.22-000329.44 & STAR    & --                  & --             & --                \\
WDJ120026.50+552539.39 & EXGAL   & --                  & --             & --                \\
WDJ120052.23-020233.35 & STAR    & --                  & --             & --                \\
WDJ120058.06+563831.52 & STAR    & --                  & --             & --                \\
WDJ120134.19+572212.03 & EXGAL   & --                  & --             & --                \\
WDJ120152.16+012755.40 & EXGAL   & --                  & --             & --                \\
WDJ120154.85+580425.76 & EXGAL   & --                  & --             & --                \\
WDJ120224.20+273029.17 & STAR    & 4006908379238662272 & 20.077 (0.006) & 0.0745            \\
WDJ120225.91+531835.34 & EXGAL   & --                  & --             & --                \\
WDJ120250.47+001522.36 & STAR    & --                  & --             & --                \\
WDJ120258.98+711640.15 & EXGAL   & --                  & --             & --                \\
WDJ120310.61+520456.08 & STAR    & --                  & --             & --                \\
WDJ120336.30+544426.31 & EXGAL   & --                  & --             & --                \\
WDJ120347.43-002310.94 & UNCLASS & 3698872156539379968 & 15.175 (0.003) & 0.9994            \\
WDJ120352.69-002242.93 & STAR    & --                  & --             & --                \\
WDJ120357.14+005431.72 & STAR    & --                  & --             & --                \\
WDJ120417.18+542022.45 & EXGAL   & --                  & --             & --                \\
WDJ120443.21+532217.18 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ120449.29+284010.25 & STAR    & --                  & --             & --                \\
WDJ120503.68+265020.66 & EXGAL   & --                  & --             & --                \\
WDJ120547.35+565107.69 & EXGAL   & --                  & --             & --                \\
WDJ120629.50-002316.88 & DUNNO   & --                  & --             & --                \\
WDJ120632.59-003521.85 & STAR    & --                  & --             & --                \\
WDJ120718.43+532014.26 & EXGAL   & 1548947794588126720 & 20.476 (0.007) & 0.6718            \\
WDJ120728.43+540129.16 & DUNNO   & 1573011744729727104 & 15.934 (0.003) & 0.6140            \\
WDJ120743.16+534849.95 & EXGAL   & --                  & --             & --                \\
WDJ120806.46-010754.52 & STAR    & --                  & --             & --                \\
WDJ120829.66+535516.66 & EXGAL   & --                  & --             & --                \\
WDJ120838.15+522619.15 & EXGAL   & --                  & --             & --                \\
WDJ120844.77+525120.61 & EXGAL   & --                  & --             & --                \\
WDJ120855.19+530819.07 & EXGAL   & --                  & --             & --                \\
WDJ120908.80+002405.07 & STAR    & --                  & --             & --                \\
WDJ121013.49+000752.83 & STAR    & --                  & --             & --                \\
WDJ121018.48+564410.75 & EXGAL   & --                  & --             & --                \\
WDJ121029.95+005442.06 & EXGAL   & --                  & --             & --                \\
WDJ121127.91+001554.20 & EXGAL   & --                  & --             & --                \\
WDJ121135.69+532636.07 & EXGAL   & --                  & --             & --                \\
WDJ121143.94+010323.39 & STAR    & --                  & --             & --                \\
WDJ121202.79+751506.70 & STAR    & 1692563082829680512 & 19.824 (0.005) & 0.0460            \\
WDJ121221.60+543810.74 & EXGAL   & --                  & --             & --                \\
WDJ121256.07+580641.60 & EXGAL   & --                  & --             & --                \\
WDJ121256.72-005537.56 & STAR    & --                  & --             & --                \\
WDJ121341.76+540006.78 & EXGAL   & --                  & --             & --                \\
WDJ121442.57+562525.65 & EXGAL   & --                  & --             & --                \\
WDJ121510.44+444115.93 & EXGAL   & --                  & --             & --                \\
WDJ121511.34+570633.52 & EXGAL   & --                  & --             & --                \\
WDJ121512.75-002022.04 & STAR    & --                  & --             & --                \\
WDJ121536.26+455518.50 & EXGAL   & --                  & --             & --                \\
WDJ121540.50-003433.70 & EXGAL   & --                  & --             & --                \\
WDJ121552.59+573810.03 & STAR    & --                  & --             & --                \\
WDJ121552.99-003534.42 & STAR    & --                  & --             & --                \\
WDJ121558.76+453842.36 & EXGAL   & --                  & --             & --                \\
WDJ121614.69+553749.96 & STAR    & --                  & --             & --                \\
WDJ121625.84-014804.60 & STAR    & --                  & --             & --                \\
WDJ121629.17+530034.84 & EXGAL   & --                  & --             & --                \\
WDJ121631.13+573926.95 & EXGAL   & --                  & --             & --                \\
WDJ121637.68+001204.23 & STAR    & 3698446744322170368 & 19.928 (0.006) & 0.1151            \\
WDJ121654.13+560335.09 & EXGAL   & --                  & --             & --                \\
WDJ121707.59+565050.33 & EXGAL   & --                  & --             & --                \\
WDJ121737.05+460633.15 & EXGAL   & --                  & --             & --                \\
WDJ121753.55+002622.35 & STAR    & --                  & --             & --                \\
WDJ121754.74+454930.94 & EXGAL   & --                  & --             & --                \\
WDJ121831.19+441332.49 & EXGAL   & --                  & --             & --                \\
WDJ121933.24+330433.83 & STAR    & --                  & --             & --                \\
WDJ121955.03+313943.85 & DUNNO   & 4015353487533222272 & 17.250 (0.003) & 0.2645            \\
WDJ122034.67+435720.31 & EXGAL   & --                  & --             & --                \\
WDJ122040.67+325040.97 & EXGAL   & --                  & --             & --                \\
WDJ122041.15+532249.60 & EXGAL   & --                  & --             & --                \\
WDJ122042.37+320104.96 & EXGAL   & --                  & --             & --                \\
WDJ122107.60+450804.57 & EXGAL   & --                  & --             & --                \\
WDJ122121.76+450231.04 & EXGAL   & --                  & --             & --                \\
WDJ122217.26+443047.31 & EXGAL   & --                  & --             & --                \\
WDJ122226.45+554007.60 & EXGAL   & --                  & --             & --                \\
WDJ122237.39+574004.61 & EXGAL   & --                  & --             & --                \\
WDJ122317.72+331552.87 & EXGAL   & --                  & --             & --                \\
WDJ122323.44+791906.53 & UNCLASS & 1717851614045315200 & 19.789 (0.005) & 0.9938            \\
WDJ122351.06+435015.79 & EXGAL   & --                  & --             & --                \\
WDJ122357.09+443315.12 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ122454.90+575940.19 & EXGAL   & --                  & --             & --                \\
WDJ122519.57+434312.26 & EXGAL   & --                  & --             & --                \\
WDJ122541.49+561111.37 & EXGAL   & --                  & --             & --                \\
WDJ122552.52+543544.13 & DUNNO   & --                  & --             & --                \\
WDJ122554.60+560000.87 & EXGAL   & --                  & --             & --                \\
WDJ122555.31+612429.28 & DUNNO   & 1583302860031730048 & 16.776 (0.003) & 0.7657            \\
WDJ122557.77-063543.74 & UNCLASS & 3583688757226156032 & 19.221 (0.004) & 0.9977            \\
WDJ122709.51+583245.83 & EXGAL   & --                  & --             & --                \\
WDJ122725.72+622842.09 & EXGAL   & --                  & --             & --                \\
WDJ122731.63+333258.25 & EXGAL   & --                  & --             & --                \\
WDJ122737.44+310439.59 & EXGAL   & --                  & --             & --                \\
WDJ122737.70+571052.37 & EXGAL   & --                  & --             & --                \\
WDJ122742.04+573423.88 & EXGAL   & --                  & --             & --                \\
WDJ122812.32+551946.21 & EXGAL   & --                  & --             & --                \\
WDJ122816.04-073334.90 & UNCLASS & 3583289462706581376 & 19.796 (0.005) & 0.9861            \\
WDJ122824.75+611608.24 & EXGAL   & --                  & --             & --                \\
WDJ122838.49+562411.37 & EXGAL   & --                  & --             & --                \\
WDJ122843.89+331135.81 & EXGAL   & --                  & --             & --                \\
WDJ122917.19+580552.44 & EXGAL   & --                  & --             & --                \\
WDJ122944.23+563905.98 & DUNNO   & 1574626991733382784 & 19.862 (0.005) & 0.8590            \\
WDJ123030.72-080549.65 & UNCLASS & 3580206810059875200 & 19.342 (0.004) & 0.9875            \\
WDJ123156.42+572510.84 & STAR    & --                  & --             & --                \\
WDJ123256.01+585142.10 & EXGAL   & --                  & --             & --                \\
WDJ123309.09+591359.31 & EXGAL   & --                  & --             & --                \\
WDJ123345.38+593042.95 & EXGAL   & --                  & --             & --                \\
WDJ123422.05-055936.71 & DUNNO   & 3679674679221681536 & 19.687 (0.005) & 0.9468            \\
WDJ123453.46+580131.29 & EXGAL   & --                  & --             & --                \\
WDJ123522.70+590520.75 & STAR    & --                  & --             & --                \\
WDJ123538.76+604642.70 & STAR    & 1583025959195283072 & 20.139 (0.006) & 0.9595            \\
WDJ123550.46+563311.95 & DUNNO   & --                  & --             & --                \\
WDJ123556.72+541542.69 & DUNNO   & 1570955275731632512 & 19.382 (0.004) & 0.9962            \\
WDJ123613.93+550705.76 & EXGAL   & --                  & --             & --                \\
WDJ123643.09+542920.77 & EXGAL   & --                  & --             & --                \\
WDJ123644.55+551406.23 & EXGAL   & --                  & --             & --                \\
WDJ123655.33+553227.03 & EXGAL   & --                  & --             & --                \\
WDJ123702.16+540521.48 & EXGAL   & --                  & --             & --                \\
WDJ123703.30+630641.01 & EXGAL   & --                  & --             & --                \\
WDJ123706.87+621702.14 & EXGAL   & --                  & --             & --                \\
WDJ123739.51+555238.69 & EXGAL   & --                  & --             & --                \\
WDJ123806.79+610048.63 & STAR    & --                  & --             & --                \\
WDJ123929.06+575202.49 & EXGAL   & --                  & --             & --                \\
WDJ123939.71+552911.38 & EXGAL   & --                  & --             & --                \\
WDJ123946.78+632316.22 & EXGAL   & --                  & --             & --                \\
WDJ123953.30+624917.12 & EXGAL   & --                  & --             & --                \\
WDJ124001.49+583135.68 & EXGAL   & --                  & --             & --                \\
WDJ124002.04+564558.59 & EXGAL   & --                  & --             & --                \\
WDJ124042.08+584700.89 & EXGAL   & --                  & --             & --                \\
WDJ124056.50+542045.24 & EXGAL   & --                  & --             & --                \\
WDJ124111.14+531723.58 & EXGAL   & --                  & --             & --                \\
WDJ124245.58+580559.42 & EXGAL   & --                  & --             & --                \\
WDJ124328.91+611938.14 & STAR    & --                  & --             & --                \\
WDJ124427.36+611838.64 & EXGAL   & --                  & --             & --                \\
WDJ124438.22+534355.25 & EXGAL   & --                  & --             & --                \\
WDJ124450.34+552014.47 & EXGAL   & --                  & --             & --                \\
WDJ124613.03+545330.99 & EXGAL   & --                  & --             & --                \\
WDJ124707.80+754713.16 & DUNNO   & 1692112214342784000 & 19.403 (0.004) & 0.9959            \\
WDJ124734.99+605639.15 & EXGAL   & --                  & --             & --                \\
WDJ124758.43+590124.37 & EXGAL   & --                  & --             & --                \\
WDJ124815.80+615944.89 & EXGAL   & --                  & --             & --                \\
WDJ124820.16+631002.10 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ124906.16+754303.32 & DUNNO   & 1692107923671422592 & 16.838 (0.003) & 0.9968            \\
WDJ125110.58+290630.27 & EXGAL   & --                  & --             & --                \\
WDJ125142.59+291221.22 & DUNNO   & 1464837457164974976 & 19.837 (0.005) & 0.9952            \\
WDJ125205.33+283426.56 & EXGAL   & --                  & --             & --                \\
WDJ125210.02+583146.24 & EXGAL   & --                  & --             & --                \\
WDJ125222.68+614812.76 & UNCLASS & 1580373864133805568 & 19.025 (0.004) & 0.9954            \\
WDJ125243.77+240131.21 & STAR    & --                  & --             & --                \\
WDJ125251.69+272114.59 & EXGAL   & --                  & --             & --                \\
WDJ125328.18+272742.44 & EXGAL   & --                  & --             & --                \\
WDJ125344.98+303622.01 & DUNNO   & --                  & --             & --                \\
WDJ125352.74+291307.58 & STAR    & --                  & --             & --                \\
WDJ125359.85+262809.39 & STAR    & --                  & --             & --                \\
WDJ125409.21+252108.06 & STAR    & --                  & --             & --                \\
WDJ125433.71+272916.57 & EXGAL   & --                  & --             & --                \\
WDJ125435.11+252527.72 & EXGAL   & --                  & --             & --                \\
WDJ125511.00+252549.59 & EXGAL   & --                  & --             & --                \\
WDJ125545.61+303917.64 & DUNNO   & --                  & --             & --                \\
WDJ125551.57+261251.23 & STAR    & 3958543194899117696 & 19.476 (0.004) & 0.9183            \\
WDJ125554.51+274404.09 & EXGAL   & --                  & --             & --                \\
WDJ125559.63+270832.43 & STAR    & --                  & --             & --                \\
WDJ125629.80+281538.32 & EXGAL   & --                  & --             & --                \\
WDJ125630.28+231746.16 & EXGAL   & --                  & --             & --                \\
WDJ125650.56+283816.64 & EXGAL   & --                  & --             & --                \\
WDJ125715.84+310029.61 & EXGAL   & --                  & --             & --                \\
WDJ125719.09+294335.59 & EXGAL   & --                  & --             & --                \\
WDJ125735.38+295803.54 & UNCLASS & --                  & --             & --                \\
WDJ125806.38+240604.70 & DUNNO   & --                  & --             & --                \\
WDJ125815.86+281722.93 & EXGAL   & --                  & --             & --                \\
WDJ125824.38+294052.10 & EXGAL   & --                  & --             & --                \\
WDJ125843.13+235656.48 & STAR    & --                  & --             & --                \\
WDJ125843.19+263717.66 & STAR    & 3958571163726655360 & 19.445 (0.004) & 0.9942            \\
WDJ125851.32+255704.56 & DUNNO   & 3958324082847872000 & 19.885 (0.004) & 0.9608            \\
WDJ125905.23+274739.40 & EXGAL   & --                  & --             & --                \\
WDJ125911.38+275603.56 & STAR    & 1460807918848407296 & 20.217 (0.006) & 0.9834            \\
WDJ125918.00+263356.56 & EXGAL   & --                  & --             & --                \\
WDJ125927.16+284341.71 & EXGAL   & --                  & --             & --                \\
WDJ125927.26+271228.97 & EXGAL   & --                  & --             & --                \\
WDJ125944.77+314805.97 & EXGAL   & --                  & --             & --                \\
WDJ125949.99+273010.34 & STAR    & --                  & --             & --                \\
WDJ130001.13+294817.32 & EXGAL   & --                  & --             & --                \\
WDJ130007.32+233826.57 & EXGAL   & --                  & --             & --                \\
WDJ130029.81+230505.94 & STAR    & --                  & --             & --                \\
WDJ130106.06+250824.99 & EXGAL   & --                  & --             & --                \\
WDJ130112.10+275617.27 & EXGAL   & --                  & --             & --                \\
WDJ130124.12+270525.74 & STAR    & --                  & --             & --                \\
WDJ130145.07+321543.25 & EXGAL   & --                  & --             & --                \\
WDJ130156.48+313749.40 & EXGAL   & --                  & --             & --                \\
WDJ130213.09+245400.33 & EXGAL   & --                  & --             & --                \\
WDJ130227.09+242209.84 & EXGAL   & --                  & --             & --                \\
WDJ130231.42+282142.03 & EXGAL   & --                  & --             & --                \\
WDJ130259.50+260046.52 & DUNNO   & --                  & --             & --                \\
WDJ130307.11+281808.15 & EXGAL   & --                  & --             & --                \\
WDJ130313.37+315730.69 & EXGAL   & --                  & --             & --                \\
WDJ130314.59+282635.10 & EXGAL   & --                  & --             & --                \\
WDJ130421.21+271640.97 & EXGAL   & --                  & --             & --                \\
WDJ130430.10+332157.08 & EXGAL   & --                  & --             & --                \\
WDJ130453.54+333004.44 & STAR    & --                  & --             & --                \\
WDJ130506.58+312221.71 & EXGAL   & --                  & --             & --                \\
WDJ130511.29+274452.28 & EXGAL   & --                  & --             & --                \\
WDJ130525.35+282735.15 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ130631.89+173925.20 & STAR    & --                  & --             & --                \\
WDJ130636.42+312025.58 & EXGAL   & --                  & --             & --                \\
WDJ130725.95+173304.26 & STAR    & --                  & --             & --                \\
WDJ130751.98+244707.93 & EXGAL   & --                  & --             & --                \\
WDJ130807.04+331929.39 & STAR    & --                  & --             & --                \\
WDJ130848.80+000559.25 & EXGAL   & --                  & --             & --                \\
WDJ130945.57-002135.10 & STAR    & --                  & --             & --                \\
WDJ131009.28+273235.74 & EXGAL   & --                  & --             & --                \\
WDJ131027.50+184042.59 & EXGAL   & --                  & --             & --                \\
WDJ131034.19+004205.65 & STAR    & --                  & --             & --                \\
WDJ131035.45+071920.26 & EXGAL   & --                  & --             & --                \\
WDJ131107.83+065541.94 & EXGAL   & --                  & --             & --                \\
WDJ131155.60+063511.80 & STAR    & --                  & --             & --                \\
WDJ131155.77-012557.38 & EXGAL   & --                  & --             & --                \\
WDJ131212.75+170110.68 & STAR    & --                  & --             & --                \\
WDJ131223.93+181053.00 & STAR    & --                  & --             & --                \\
WDJ131244.83+181208.82 & STAR    & --                  & --             & --                \\
WDJ131245.25+180919.88 & STAR    & --                  & --             & --                \\
WDJ131245.91+180532.93 & STAR    & --                  & --             & --                \\
WDJ131255.23+180610.01 & STAR    & --                  & --             & --                \\
WDJ131257.89+180531.60 & STAR    & --                  & --             & --                \\
WDJ131303.14+181346.47 & STAR    & --                  & --             & --                \\
WDJ131311.15+180712.50 & STAR    & --                  & --             & --                \\
WDJ131317.71+181910.76 & STAR    & --                  & --             & --                \\
WDJ131359.34+192519.00 & EXGAL   & --                  & --             & --                \\
WDJ131534.10+001824.45 & STAR    & --                  & --             & --                \\
WDJ131557.31-000805.60 & STAR    & --                  & --             & --                \\
WDJ131606.11+173658.77 & STAR    & --                  & --             & --                \\
WDJ131620.06+174031.97 & STAR    & --                  & --             & --                \\
WDJ131645.00+173811.52 & STAR    & --                  & --             & --                \\
WDJ131733.12+195032.90 & EXGAL   & --                  & --             & --                \\
WDJ131900.79+165107.68 & EXGAL   & --                  & --             & --                \\
WDJ132318.10+034605.19 & DUNNO   & 3715676160249364096 & 19.854 (0.006) & 0.0993            \\
WDJ132332.96+184313.88 & EXGAL   & --                  & --             & --                \\
WDJ132518.07+202710.15 & EXGAL   & --                  & --             & --                \\
WDJ132535.88+810929.16 & DUNNO   & 1719016198723069568 & 19.521 (0.004) & 0.9931            \\
WDJ132616.99+045240.65 & STAR    & --                  & --             & --                \\
WDJ132727.76+061129.47 & STAR    & --                  & --             & --                \\
WDJ132920.74+323157.68 & STAR    & --                  & --             & --                \\
WDJ132920.91+320838.63 & EXGAL   & --                  & --             & --                \\
WDJ132957.04+052902.83 & STAR    & --                  & --             & --                \\
WDJ133214.18+024840.23 & STAR    & --                  & --             & --                \\
WDJ133257.74+335117.80 & STAR    & --                  & --             & --                \\
WDJ133331.46+321005.16 & EXGAL   & --                  & --             & --                \\
WDJ133413.16+313929.60 & STAR    & --                  & --             & --                \\
WDJ133501.97+033934.99 & STAR    & --                  & --             & --                \\
WDJ133656.36+800943.41 & DUNNO   & 1718710568850372864 & 18.711 (0.003) & 0.9950            \\
WDJ133800.72+313012.49 & EXGAL   & --                  & --             & --                \\
WDJ133813.65+323203.11 & EXGAL   & --                  & --             & --                \\
WDJ133933.41+315721.45 & STAR    & 1456850364182697088 & 19.852 (0.004) & 0.0544            \\
WDJ134308.01+812448.67 & DUNNO   & 1718939095470066688 & 19.686 (0.005) & 0.9793            \\
WDJ134447.14+810619.08 & DUNNO   & 1718861098863847168 & 18.811 (0.004) & 0.9983            \\
WDJ134741.97+810415.83 & DUNNO   & 1718857456731568128 & 19.372 (0.004) & 0.9952            \\
WDJ135126.40+700535.84 & EXGAL   & --                  & --             & --                \\
WDJ135355.66+052431.79 & STAR    & --                  & --             & --                \\
WDJ135556.22+054137.88 & STAR    & --                  & --             & --                \\
WDJ135703.25+041655.78 & STAR    & --                  & --             & --                \\
WDJ135708.33+042335.34 & STAR    & --                  & --             & --                \\
WDJ135718.51+041804.41 & STAR    & --                  & --             & --                \\
WDJ135738.59+060234.84 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ135815.15+060916.31 & EXGAL   & --                  & --             & --                \\
WDJ135910.18+783736.40 & DUNNO   & 1715011502496355840 & 19.774 (0.005) & 0.9941            \\
WDJ135940.12+041350.01 & STAR    & --                  & --             & --                \\
WDJ135950.27+040229.75 & EXGAL   & --                  & --             & --                \\
WDJ140033.11+031827.25 & DUNNO   & --                  & --             & --                \\
WDJ140056.87+050914.83 & STAR    & 3671833168451171200 & 18.968 (0.004) & 0.2338            \\
WDJ140132.58+055243.66 & EXGAL   & --                  & --             & --                \\
WDJ140208.04+032410.45 & EXGAL   & --                  & --             & --                \\
WDJ140229.69+790515.47 & DUNNO   & 1715403551406505344 & 19.149 (0.004) & 0.9809            \\
WDJ140231.04+052855.36 & EXGAL   & --                  & --             & --                \\
WDJ140244.37+230154.96 & EXGAL   & --                  & --             & --                \\
WDJ140252.04+033827.38 & EXGAL   & --                  & --             & --                \\
WDJ140315.22+241746.36 & STAR    & --                  & --             & --                \\
WDJ140347.56+034218.86 & EXGAL   & --                  & --             & --                \\
WDJ140355.57+043941.10 & EXGAL   & --                  & --             & --                \\
WDJ140408.95+034413.46 & DUNNO   & --                  & --             & --                \\
WDJ140415.85+784215.26 & DUNNO   & 1715007624141215360 & 18.974 (0.004) & 0.9911            \\
WDJ140508.88+044430.98 & STAR    & --                  & --             & --                \\
WDJ140517.29+050900.21 & STAR    & 3672158589532816896 & 18.761 (0.004) & 0.0979            \\
WDJ140525.35+060048.70 & EXGAL   & --                  & --             & --                \\
WDJ140704.09-010635.34 & STAR    & --                  & --             & --                \\
WDJ140724.75+004641.83 & DUNNO   & 3661013256774699392 & 19.723 (0.005) & 0.8652            \\
WDJ140755.92+000747.63 & STAR    & --                  & --             & --                \\
WDJ140826.75-003051.72 & STAR    & --                  & --             & --                \\
WDJ140933.37+812230.31 & DUNNO   & 1721881972701637248 & 19.360 (0.004) & 0.9908            \\
WDJ140935.36+005611.96 & EXGAL   & --                  & --             & --                \\
WDJ140954.45-000720.14 & STAR    & --                  & --             & --                \\
WDJ141012.64+000624.14 & STAR    & 3659974768041996288 & 19.525 (0.005) & 0.0203            \\
WDJ141020.45-003245.09 & STAR    & --                  & --             & --                \\
WDJ141021.86+010644.78 & EXGAL   & --                  & --             & --                \\
WDJ141028.47+005323.72 & STAR    & 3660277301243052928 & 19.799 (0.005) & 0.1091            \\
WDJ141035.10+001248.58 & STAR    & --                  & --             & --                \\
WDJ141108.98+010745.65 & DUNNO   & 3666295134540172160 & 19.840 (0.006) & 0.9865            \\
WDJ141204.15+795405.70 & DUNNO   & 1715550748526849792 & 18.375 (0.003) & 0.9960            \\
WDJ141208.20-001217.44 & EXGAL   & --                  & --             & --                \\
WDJ141222.44+784443.82 & DUNNO   & 1715336305103347840 & 19.873 (0.005) & 0.9895            \\
WDJ141225.91-001825.33 & STAR    & --                  & --             & --                \\
WDJ141238.49-014937.99 & EXGAL   & --                  & --             & --                \\
WDJ141323.87-005604.48 & STAR    & --                  & --             & --                \\
WDJ141326.74+001812.73 & STAR    & --                  & --             & --                \\
WDJ141327.47+523851.79 & EXGAL   & --                  & --             & --                \\
WDJ141347.49+000228.03 & STAR    & --                  & --             & --                \\
WDJ141407.97+003327.92 & STAR    & --                  & --             & --                \\
WDJ141409.58+321133.51 & EXGAL   & --                  & --             & --                \\
WDJ141409.86+520137.16 & EXGAL   & --                  & --             & --                \\
WDJ141506.61+804505.52 & DUNNO   & 1721800711920129408 & 19.703 (0.004) & 0.9944            \\
WDJ141556.68-005814.84 & DUNNO   & --                  & --             & --                \\
WDJ141604.98+002236.52 & EXGAL   & --                  & --             & --                \\
WDJ141653.02+312656.08 & STAR    & --                  & --             & --                \\
WDJ141728.43-000805.11 & EXGAL   & --                  & --             & --                \\
WDJ141910.09-011428.85 & DUNNO   & --                  & --             & --                \\
WDJ141923.78+310754.42 & EXGAL   & --                  & --             & --                \\
WDJ141954.33-012014.44 & EXGAL   & --                  & --             & --                \\
WDJ142027.40-013613.98 & STAR    & --                  & --             & --                \\
WDJ142035.91-002932.33 & STAR    & --                  & --             & --                \\
WDJ142038.34+513714.92 & EXGAL   & --                  & --             & --                \\
WDJ142111.13-010353.51 & STAR    & --                  & --             & --                \\
WDJ142139.97-005148.43 & EXGAL   & --                  & --             & --                \\
WDJ142215.28-005420.45 & EXGAL   & --                  & --             & --                \\
WDJ142222.41+323852.42 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ142256.30-001356.60 & STAR    & --                  & --             & --                \\
WDJ142326.27+521752.91 & EXGAL   & --                  & --             & --                \\
WDJ142338.61+343136.66 & EXGAL   & --                  & --             & --                \\
WDJ142349.06+334857.07 & DUNNO   & 1479727249786784384 & 19.604 (0.003) & 0.8946            \\
WDJ142415.65+000000.55 & STAR    & --                  & --             & --                \\
WDJ142443.52+333010.11 & EXGAL   & --                  & --             & --                \\
WDJ142445.78+342945.17 & EXGAL   & --                  & --             & --                \\
WDJ142508.87-014502.00 & STAR    & --                  & --             & --                \\
WDJ142532.62+315813.18 & EXGAL   & --                  & --             & --                \\
WDJ142550.32+335618.79 & EXGAL   & --                  & --             & --                \\
WDJ142610.76+341738.84 & EXGAL   & --                  & --             & --                \\
WDJ142614.46+024327.30 & STAR    & --                  & --             & --                \\
WDJ142654.90-021157.87 & STAR    & --                  & --             & --                \\
WDJ142702.70-001344.94 & EXGAL   & --                  & --             & --                \\
WDJ142729.04+000142.05 & EXGAL   & --                  & --             & --                \\
WDJ142741.21+332937.27 & EXGAL   & --                  & --             & --                \\
WDJ142802.59+013713.66 & STAR    & --                  & --             & --                \\
WDJ142810.54+515945.47 & STAR    & --                  & --             & --                \\
WDJ142817.90+032407.51 & DUNNO   & 3668348781742691328 & 17.266 (0.003) & 0.9978            \\
WDJ142824.85+541639.12 & EXGAL   & --                  & --             & --                \\
WDJ142842.98+001737.50 & STAR    & --                  & --             & --                \\
WDJ142850.06+331748.23 & EXGAL   & --                  & --             & --                \\
WDJ142852.65+335148.26 & EXGAL   & --                  & --             & --                \\
WDJ142907.79-010038.14 & DUNNO   & 3652672391630956032 & 19.591 (0.005) & 0.6260            \\
WDJ142925.77-002626.77 & STAR    & --                  & --             & --                \\
WDJ142951.32+024747.57 & STAR    & --                  & --             & --                \\
WDJ143012.21+334232.41 & EXGAL   & --                  & --             & --                \\
WDJ143012.74+331905.61 & EXGAL   & --                  & --             & --                \\
WDJ143041.52+014711.61 & STAR    & --                  & --             & --                \\
WDJ143041.82+015221.25 & EXGAL   & --                  & --             & --                \\
WDJ143052.23-005003.28 & STAR    & --                  & --             & --                \\
WDJ143103.70+142852.38 & STAR    & --                  & --             & --                \\
WDJ143136.23+024435.12 & EXGAL   & --                  & --             & --                \\
WDJ143136.90+140827.50 & EXGAL   & --                  & --             & --                \\
WDJ143150.78+514947.86 & EXGAL   & --                  & --             & --                \\
WDJ143153.98+530034.15 & EXGAL   & --                  & --             & --                \\
WDJ143157.11+352800.03 & STAR    & --                  & --             & --                \\
WDJ143212.60+355027.14 & EXGAL   & 1480420251349953920 & 20.533 (0.008) & 0.8564            \\
WDJ143226.66+005055.82 & STAR    & --                  & --             & --                \\
WDJ143233.19+153227.63 & STAR    & --                  & --             & --                \\
WDJ143258.00+011857.40 & DUNNO   & 3655054139974647424 & 17.925 (0.003) & 0.1198            \\
WDJ143259.51+034553.31 & EXGAL   & --                  & --             & --                \\
WDJ143310.18+351405.91 & EXGAL   & --                  & --             & --                \\
WDJ143314.75+530935.75 & DUNNO   & 1605239049014274560 & 17.120 (0.003) & 0.0640            \\
WDJ143321.36+155828.09 & STAR    & --                  & --             & --                \\
WDJ143328.94+030304.41 & EXGAL   & --                  & --             & --                \\
WDJ143332.09+135345.43 & STAR    & --                  & --             & --                \\
WDJ143334.29+031059.34 & EXGAL   & --                  & --             & --                \\
WDJ143341.60+332412.86 & EXGAL   & --                  & --             & --                \\
WDJ143347.43+030512.29 & EXGAL   & --                  & --             & --                \\
WDJ143348.77+022422.33 & STAR    & --                  & --             & --                \\
WDJ143358.52+003009.40 & DUNNO   & --                  & --             & --                \\
WDJ143404.07+024208.00 & DUNNO   & 3656064556800894464 & 16.823 (0.003) & 0.0510            \\
WDJ143421.13-011226.39 & EXGAL   & --                  & --             & --                \\
WDJ143422.61+145110.49 & EXGAL   & --                  & --             & --                \\
WDJ143426.88+641739.73 & EXGAL   & --                  & --             & --                \\
WDJ143429.80-001746.28 & STAR    & 3653143635442071040 & 18.711 (0.004) & 0.6058            \\
WDJ143448.08-010224.08 & STAR    & --                  & --             & --                \\
WDJ143450.30+024705.01 & EXGAL   & --                  & --             & --                \\
WDJ143452.74-002828.06 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ143458.69-011413.87 & STAR    & --                  & --             & --                \\
WDJ143507.14-005604.00 & STAR    & --                  & --             & --                \\
WDJ143523.29-004345.90 & STAR    & 3650114721426027392 & 19.816 (0.007) & 0.0422            \\
WDJ143524.91+025911.94 & EXGAL   & --                  & --             & --                \\
WDJ143526.58+350037.34 & EXGAL   & --                  & --             & --                \\
WDJ143533.15-004959.42 & STAR    & 3650007622122080896 & 19.574 (0.006) & 0.1638            \\
WDJ143534.09+020334.73 & EXGAL   & --                  & --             & --                \\
WDJ143543.31+650337.38 & DUNNO   & 1668928221397609984 & 19.087 (0.004) & 0.9955            \\
WDJ143543.89-012434.22 & STAR    & --                  & --             & --                \\
WDJ143546.37-000903.54 & EXGAL   & --                  & --             & --                \\
WDJ143555.16+004614.88 & STAR    & --                  & --             & --                \\
WDJ143632.87+013812.53 & STAR    & 3655166702478073472 & 18.324 (0.003) & 0.2143            \\
WDJ143639.91-014214.45 & STAR    & --                  & --             & --                \\
WDJ143709.92+143046.97 & STAR    & --                  & --             & --                \\
WDJ143716.72+151756.69 & STAR    & 1234099616317176576 & 19.670 (0.005) & 0.0193            \\
WDJ143726.25+142332.82 & STAR    & --                  & --             & --                \\
WDJ143741.35+531453.23 & EXGAL   & --                  & --             & --                \\
WDJ143809.76+340329.42 & DUNNO   & 1287601409745805696 & 19.732 (0.004) & 0.9702            \\
WDJ143813.65+134828.17 & STAR    & --                  & --             & --                \\
WDJ143828.80+003630.05 & EXGAL   & --                  & --             & --                \\
WDJ143854.45+341258.79 & EXGAL   & --                  & --             & --                \\
WDJ143908.77-010747.07 & EXGAL   & --                  & --             & --                \\
WDJ143943.63+142546.14 & STAR    & --                  & --             & --                \\
WDJ143949.27+135652.06 & STAR    & --                  & --             & --                \\
WDJ144001.76-014959.41 & EXGAL   & --                  & --             & --                \\
WDJ144023.58+135454.66 & STAR    & --                  & --             & --                \\
WDJ144048.22-015301.69 & STAR    & --                  & --             & --                \\
WDJ144056.66+002208.78 & STAR    & --                  & --             & --                \\
WDJ144115.95+002704.39 & STAR    & --                  & --             & --                \\
WDJ144119.67+001234.79 & EXGAL   & --                  & --             & --                \\
WDJ144132.53-020705.76 & DUNNO   & --                  & --             & --                \\
WDJ144404.65-014441.20 & EXGAL   & --                  & --             & --                \\
WDJ144412.85-002400.32 & STAR    & --                  & --             & --                \\
WDJ144433.73-005346.95 & STAR    & 3650577959418538240 & 19.457 (0.006) & 0.0296            \\
WDJ144542.95-002339.08 & STAR    & --                  & --             & --                \\
WDJ145031.27+661023.32 & EXGAL   & --                  & --             & --                \\
WDJ145359.43+650915.71 & EXGAL   & --                  & --             & --                \\
WDJ145404.39+505448.64 & EXGAL   & --                  & --             & --                \\
WDJ145420.12+522315.67 & EXGAL   & --                  & --             & --                \\
WDJ145422.36+344731.13 & EXGAL   & --                  & --             & --                \\
WDJ145630.95-080141.45 & DUNNO   & --                  & --             & --                \\
WDJ145655.47+324257.23 & EXGAL   & --                  & --             & --                \\
WDJ145848.85+323619.42 & EXGAL   & --                  & --             & --                \\
WDJ145957.33+510949.22 & STAR    & 1592584490515955968 & 19.730 (0.004) & 0.9983            \\
WDJ150006.70+684112.23 & EXGAL   & --                  & --             & --                \\
WDJ150008.19-072826.16 & UNCLASS & --                  & --             & --                \\
WDJ150045.78+311155.62 & EXGAL   & --                  & --             & --                \\
WDJ150137.80+514918.48 & STAR    & --                  & --             & --                \\
WDJ150235.78-065511.49 & UNCLASS & --                  & --             & --                \\
WDJ150533.95+314838.09 & STAR    & 1288619312696849536 & 18.467 (0.003) & 0.1392            \\
WDJ150627.19+325756.12 & EXGAL   & --                  & --             & --                \\
WDJ150921.24+320040.92 & EXGAL   & --                  & --             & --                \\
WDJ150933.18+685039.41 & STAR    & --                  & --             & --                \\
WDJ151020.73+162631.54 & EXGAL   & --                  & --             & --                \\
WDJ151051.51+323143.84 & STAR    & 1276760220798496896 & 19.300 (0.004) & 0.7479            \\
WDJ151326.43+743121.24 & STAR    & --                  & --             & --                \\
WDJ151419.33+171148.03 & EXGAL   & --                  & --             & --                \\
WDJ151608.85+183857.41 & EXGAL   & --                  & --             & --                \\
WDJ151646.42+735206.96 & DUNNO   & 1697669356564165632 & 16.626 (0.003) & 0.9692            \\
WDJ151703.46+035757.35 & EXGAL   & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ151801.94+020432.59 & STAR    & --                  & --             & --                \\
WDJ151803.29+012914.63 & EXGAL   & --                  & --             & --                \\
WDJ151809.94+020500.79 & STAR    & 4421526169599105536 & 18.803 (0.007) & 0.0459            \\
WDJ151823.40+020853.65 & STAR    & --                  & --             & --                \\
WDJ151836.32+021649.37 & STAR    & 4421624197934593536 & 19.600 (0.005) & 0.0400            \\
WDJ151839.75+015938.62 & STAR    & 4421474801790134656 & 19.030 (0.011) & 0.0428            \\
WDJ151854.31+020343.05 & STAR    & 4421569295365031168 & 19.561 (0.005) & 0.1048            \\
WDJ151903.95+015952.29 & STAR    & --                  & --             & --                \\
WDJ152225.90+022633.76 & EXGAL   & --                  & --             & --                \\
WDJ153503.87+324749.17 & EXGAL   & --                  & --             & --                \\
WDJ153707.72+434351.52 & DUNNO   & 1391314763883537280 & 17.949 (0.003) & 0.0582            \\
WDJ153816.74+434617.88 & EXGAL   & --                  & --             & --                \\
WDJ154048.63+435851.35 & EXGAL   & --                  & --             & --                \\
WDJ154247.00+444614.82 & EXGAL   & --                  & --             & --                \\
WDJ154316.33+421851.48 & EXGAL   & --                  & --             & --                \\
WDJ154401.95+755659.98 & STAR    & --                  & --             & --                \\
WDJ154402.53+415324.11 & EXGAL   & --                  & --             & --                \\
WDJ154645.64+422955.44 & DUNNO   & --                  & --             & --                \\
WDJ154720.32+425736.47 & EXGAL   & --                  & --             & --                \\
WDJ154826.41+431824.30 & EXGAL   & --                  & --             & --                \\
WDJ154828.43+443059.97 & EXGAL   & --                  & --             & --                \\
WDJ155231.80+440213.07 & EXGAL   & --                  & --             & --                \\
WDJ155800.15+143629.05 & STAR    & --                  & --             & --                \\
WDJ155824.75+430407.41 & STAR    & 1384415294059868544 & 19.252 (0.006) & 0.4481            \\
WDJ155940.14+160913.08 & EXGAL   & --                  & --             & --                \\
WDJ155940.47+542622.23 & EXGAL   & --                  & --             & --                \\
WDJ155947.43+444740.85 & EXGAL   & --                  & --             & --                \\
WDJ160019.63+441950.32 & EXGAL   & --                  & --             & --                \\
WDJ160037.57+415510.66 & STAR    & --                  & --             & --                \\
WDJ160049.05+552622.68 & EXGAL   & --                  & --             & --                \\
WDJ160109.36+144223.44 & STAR    & --                  & --             & --                \\
WDJ160130.77+153328.12 & EXGAL   & --                  & --             & --                \\
WDJ160149.22+442834.93 & EXGAL   & --                  & --             & --                \\
WDJ160248.49+445819.03 & EXGAL   & --                  & --             & --                \\
WDJ160304.68+201254.66 & STAR    & --                  & --             & --                \\
WDJ160333.94+545425.50 & EXGAL   & --                  & --             & --                \\
WDJ160351.38+433556.40 & UNCLASS & 1385988008003848192 & 20.032 (0.006) & 0.9916            \\
WDJ160354.06+551048.61 & EXGAL   & --                  & --             & --                \\
WDJ160454.71+204555.15 & EXGAL   & --                  & --             & --                \\
WDJ160508.01+432628.73 & STAR    & 1385229555435660032 & 19.948 (0.005) & 0.0581            \\
WDJ160533.63+155148.15 & STAR    & --                  & --             & --                \\
WDJ160634.92+423545.32 & EXGAL   & --                  & --             & --                \\
WDJ160643.64+414803.36 & EXGAL   & --                  & --             & --                \\
WDJ160745.87+140533.68 & STAR    & 4458535769646731392 & 18.924 (0.004) & 0.6721            \\
WDJ160800.44+154925.51 & DUNNO   & --                  & --             & --                \\
WDJ160836.22+182830.67 & STAR    & --                  & --             & --                \\
WDJ160902.63+540151.06 & EXGAL   & --                  & --             & --                \\
WDJ160941.42+183651.18 & EXGAL   & --                  & --             & --                \\
WDJ161004.93+435824.70 & EXGAL   & --                  & --             & --                \\
WDJ161008.89+543650.16 & STAR    & --                  & --             & --                \\
WDJ161036.98+560349.33 & STAR    & --                  & --             & --                \\
WDJ161104.80+185348.76 & EXGAL   & --                  & --             & --                \\
WDJ161129.04+545055.52 & EXGAL   & --                  & --             & --                \\
WDJ161142.67+563202.07 & EXGAL   & --                  & --             & --                \\
WDJ161148.26+191902.19 & EXGAL   & --                  & --             & --                \\
WDJ161227.48+541130.55 & DUNNO   & 1428949088396986240 & 20.103 (0.006) & 0.9768            \\
WDJ161243.90+734002.52 & STAR    & --                  & --             & --                \\
WDJ161246.04+734310.12 & STAR    & --                  & --             & --                \\
WDJ161246.81+193654.83 & EXGAL   & --                  & --             & --                \\
WDJ161319.42+555847.42 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ161420.49+195512.01 & STAR    & --                  & --             & --                \\
WDJ161447.70+434026.88 & EXGAL   & --                  & --             & --                \\
WDJ161512.17+191346.76 & STAR    & --                  & --             & --                \\
WDJ161552.77+541859.83 & EXGAL   & --                  & --             & --                \\
WDJ161602.40+555736.43 & EXGAL   & --                  & --             & --                \\
WDJ161608.68+430546.45 & EXGAL   & --                  & --             & --                \\
WDJ161611.42+431729.52 & EXGAL   & --                  & --             & --                \\
WDJ161801.22+433526.57 & STAR    & --                  & --             & --                \\
WDJ161825.56+540205.04 & EXGAL   & --                  & --             & --                \\
WDJ161830.09+444620.10 & EXGAL   & --                  & --             & --                \\
WDJ161856.22+433253.56 & EXGAL   & --                  & --             & --                \\
WDJ161944.85+535502.37 & STAR    & 1428309447508058880 & 19.533 (0.004) & 0.9951            \\
WDJ161952.96+540121.91 & EXGAL   & --                  & --             & --                \\
WDJ162002.44+434625.08 & EXGAL   & --                  & --             & --                \\
WDJ162025.36+432626.05 & EXGAL   & --                  & --             & --                \\
WDJ162039.27+433301.84 & STAR    & --                  & --             & --                \\
WDJ162259.79+420644.43 & DUNNO   & 1381312820138258944 & 18.635 (0.003) & 0.9949            \\
WDJ162310.50+425831.19 & DUNNO   & 1382202909161403776 & 17.739 (0.003) & 0.2809            \\
WDJ162328.41+434742.57 & EXGAL   & --                  & --             & --                \\
WDJ162557.51+430616.91 & EXGAL   & --                  & --             & --                \\
WDJ162712.69+415642.13 & EXGAL   & --                  & --             & --                \\
WDJ162806.83+442232.44 & STAR    & --                  & --             & --                \\
WDJ162906.35+314411.95 & STAR    & --                  & --             & --                \\
WDJ162933.28+420554.82 & EXGAL   & --                  & --             & --                \\
WDJ163007.90+311318.06 & STAR    & --                  & --             & --                \\
WDJ163053.92+305013.36 & STAR    & --                  & --             & --                \\
WDJ163205.86+312112.74 & EXGAL   & --                  & --             & --                \\
WDJ163226.10+424227.93 & EXGAL   & --                  & --             & --                \\
WDJ163233.57+323215.05 & EXGAL   & --                  & --             & --                \\
WDJ163335.47+325428.51 & EXGAL   & --                  & --             & --                \\
WDJ163539.37+215038.74 & EXGAL   & --                  & --             & --                \\
WDJ163558.62+324731.10 & EXGAL   & --                  & --             & --                \\
WDJ163638.01+222844.27 & EXGAL   & --                  & --             & --                \\
WDJ163803.38+371440.76 & STAR    & --                  & --             & --                \\
WDJ163905.44+243307.29 & EXGAL   & --                  & --             & --                \\
WDJ164005.77+231724.97 & EXGAL   & --                  & --             & --                \\
WDJ164105.73+362701.86 & STAR    & --                  & --             & --                \\
WDJ164113.56+362440.44 & STAR    & --                  & --             & --                \\
WDJ164120.45+363159.14 & STAR    & --                  & --             & --                \\
WDJ164123.88+362824.74 & STAR    & 1328104669341383936 & 18.200 (0.003) & 0.1668            \\
WDJ164125.48+364116.10 & STAR    & --                  & --             & --                \\
WDJ164127.13+304200.77 & DUNNO   & --                  & --             & --                \\
WDJ164128.19+362630.37 & STAR    & --                  & --             & --                \\
WDJ164132.07+363200.97 & DUNNO   & 1328105283517446016 & 18.696 (0.003) & 0.5493            \\
WDJ164135.42+362242.91 & DUNNO   & 1328056428259951616 & 18.263 (0.003) & 0.3397            \\
WDJ164144.25+363228.39 & DUNNO   & --                  & --             & --                \\
WDJ164152.65+362113.94 & STAR    & --                  & --             & --                \\
WDJ164155.77+363124.51 & STAR    & --                  & --             & --                \\
WDJ164159.85+363051.42 & DUNNO   & 1328059207109557248 & 18.539 (0.004) & 0.2801            \\
WDJ164204.09+362753.72 & STAR    & 1328058489852173440 & 18.297 (0.003) & 0.2458            \\
WDJ164204.58+362854.22 & STAR    & 1328058558563274624 & 18.045 (0.003) & 0.1284            \\
WDJ164205.79+233352.22 & STAR    & --                  & --             & --                \\
WDJ164207.13+362245.05 & STAR    & 1328053537746970112 & 18.267 (0.003) & 0.1999            \\
WDJ164236.25+351432.32 & STAR    & 1326802190433968640 & 18.205 (0.003) & 0.1104            \\
WDJ164338.93+232357.74 & EXGAL   & --                  & --             & --                \\
WDJ164445.97+344946.30 & DUNNO   & 1326961413461592064 & 19.923 (0.005) & 0.8178            \\
WDJ164502.15+335131.81 & EXGAL   & --                  & --             & --                \\
WDJ164755.41+334232.56 & EXGAL   & --                  & --             & --                \\
WDJ164756.94+330848.84 & EXGAL   & --                  & --             & --                \\
WDJ164820.10+331451.83 & DUNNO   & 1314383481475856768 & 20.400 (0.007) & 0.8243            \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{lllll}
\hline
WDJ name & WD type & Gaia DR3 source ID  & $G$ mag & $P_{\textrm{WD}}$ \\
\hline
WDJ164919.50+355019.53 & EXGAL   & --                  & --             & --                \\
WDJ164959.19+335459.82 & STAR    & --                  & --             & --                \\
WDJ165008.94+751423.11 & EXGAL   & --                  & --             & --                \\
WDJ165149.80+295600.71 & DUNNO   & 1311296843099487104 & 19.215 (0.004) & 0.4547            \\
WDJ165259.37+352010.22 & STAR    & 1315030131752334336 & 20.051 (0.006) & 0.8650            \\
WDJ165350.49+351120.26 & STAR    & 1314978901382346496 & 20.043 (0.005) & 0.9371            \\
WDJ165449.45+350803.68 & EXGAL   & --                  & --             & --                \\
WDJ165458.42+343853.65 & STAR    & --                  & --             & --                \\
WDJ165503.73+340800.88 & EXGAL   & --                  & --             & --                \\
WDJ165504.38+345703.03 & EXGAL   & --                  & --             & --                \\
WDJ165519.60+351755.67 & DUNNO   & 1338985157226553216 & 18.466 (0.003) & 0.9958            \\
WDJ165707.99+350922.88 & DUNNO   & 1338795628910635520 & 20.274 (0.006) & 0.9941            \\
WDJ171123.71+581131.25 & EXGAL   & --                  & --             & --                \\
WDJ171150.74+564601.50 & EXGAL   & --                  & --             & --                \\
WDJ171649.84+430746.62 & STAR    & --                  & --             & --                \\
WDJ171714.29+430414.26 & STAR    & --                  & --             & --                \\
WDJ171725.71+430734.40 & STAR    & --                  & --             & --                \\
WDJ171750.25+575912.79 & STAR    & --                  & --             & --                \\
WDJ171750.43+424648.54 & STAR    & --                  & --             & --                \\
WDJ171832.94+585242.20 & EXGAL   & --                  & --             & --                \\
WDJ172017.48+563831.41 & EXGAL   & --                  & --             & --                \\
WDJ172035.08+582559.70 & STAR    & --                  & --             & --                \\
WDJ172042.43+573955.47 & STAR    & --                  & --             & --                \\
WDJ172140.33+575132.10 & STAR    & --                  & --             & --                \\
WDJ172156.44+565639.97 & STAR    & --                  & --             & --                \\
WDJ172307.49+575355.35 & STAR    & --                  & --             & --                \\
WDJ172335.96+575642.78 & STAR    & --                  & --             & --                \\
WDJ172456.63+562220.42 & EXGAL   & --                  & --             & --                \\
WDJ172751.38+570834.42 & EXGAL   & --                  & --             & --                \\
WDJ175109.00+633030.88 & EXGAL   & --                  & --             & --                \\
WDJ175144.46+611729.83 & DUNNO   & 1436226824580848128 & 20.216 (0.007) & 0.9917            \\
WDJ175158.77+692245.60 & STAR    & --                  & --             & --                \\
WDJ175303.30+810743.55 & EXGAL   & --                  & --             & --                \\
WDJ175456.35+712807.04 & DUNNO   & 1639208387739290112 & 19.699 (0.005) & 0.9729            \\
WDJ175709.15+623520.79 & EXGAL   & --                  & --             & --                \\
WDJ175832.85+624648.36 & STAR    & 1436569807785173248 & 20.370 (0.007) & 0.7602            \\
WDJ175859.48+645338.88 & EXGAL   & --                  & --             & --                \\
WDJ175934.35+645636.09 & EXGAL   & --                  & --             & --                \\
WDJ175936.80+630943.00 & EXGAL   & --                  & --             & --                \\
WDJ180044.26+703508.30 & STAR    & --                  & --             & --                \\
WDJ180445.14+620706.93 & STAR    & --                  & --             & --                \\
WDJ180537.01+703317.48 & DUNNO   & --                  & --             & --                \\
WDJ180654.30+620159.13 & EXGAL   & --                  & --             & --                \\
WDJ180919.83+624716.86 & EXGAL   & --                  & --             & --                \\
WDJ181038.72+625244.37 & EXGAL   & --                  & --             & --                \\
WDJ181114.81+645701.42 & EXGAL   & --                  & --             & --                \\
WDJ182555.71+352637.38 & EXGAL   & --                  & --             & --                \\
WDJ182728.79+353647.47 & DUNNO   & --                  & --             & --                \\
WDJ182941.64+341752.54 & EXGAL   & --                  & --             & --                \\
WDJ183005.57+332657.49 & EXGAL   & --                  & --             & --                \\
WDJ183045.31+343534.84 & DUNNO   & --                  & --             & --                \\
WDJ183138.48+354342.52 & EXGAL   & --                  & --             & --                \\
WDJ183337.58+353714.98 & EXGAL   & --                  & --             & --                \\
WDJ183928.53+344421.32 & EXGAL   & --                  & --             & --                \\
WDJ190029.75+650130.73 & EXGAL   & --                  & --             & --                \\
WDJ190934.77+662231.74 & EXGAL   & --                  & --             & --                \\
WDJ234437.96+275526.59 & STAR    & --                  & --             & --                \\
%
\hline
\end{tabular}
\end{table*}

==> table_categories.tex <==
\begin{table}
\centering
\caption{Classifications of the white dwarf candidates visually inspected from the DESI EDR. \label{t-cat}}
\begin{tabular}{lr}
\hline
Class                & Number        \\
\hline
White dwarfs         & 2706          \\
\hline
DA	                 & 1953          \\
DA:	                 & 18            \\
DC	                 & 197           \\
DC:	                 & 23            \\
DB	                 & 139           \\
DB:	                 & 6             \\
DAZ	                 & 61            \\
DAZ:	             & 9             \\
DAH	                 & 53            \\
DAH:	             & 12            \\
DQ	                 & 50            \\
DQ:	                 & 5             \\
DZ	                 & 48            \\
DZ:	                 & 1             \\
DBZ	                 & 21            \\
DBA	                 & 15            \\
DBA:	             & 1             \\
DAO	                 & 10            \\
DAO:	             & 1             \\
DBZA	             & 7             \\
DBAZ	             & 6             \\
DBAZ:	             & 1             \\
DH:	                 & 6             \\
DZA	                 & 6             \\
DZAB	             & 4             \\
DZB	                 & 4             \\
DCH:	             & 3             \\
DAP	                 & 2             \\
DAB	                 & 1             \\
DABZ	             & 1             \\
DAe	                 & 1             \\
DAe:	             & 5             \\
DAHe	             & 1             \\
DAHe:	             & 3             \\
DAOH:	             & 1             \\
DAQ:	             & 1             \\
DAZH:	             & 1             \\
DO	                 & 1             \\
DQA	                 & 1             \\
DQH	                 & 1             \\
DQZ	                 & 1             \\
DZAP	             & 1             \\
DZBA	             & 1             \\
DZBA:	             & 2             \\
DZQ:	             & 1             \\
WD	                 & 20            \\
\hline
White dwarf binaries & 66            \\
\hline
WD+MS	             & 53            \\
CV	                 & 12            \\
DA+DQ	             & 1             \\
\hline         
Contaminants         & 817           \\
\hline                          
EXGAL	             & 445           \\
STAR	             & 329           \\
sdX	                 & 42            \\
sdX:	             & 1             \\
\hline                             
UNCLASS	             & 84            \\
%
\hline
\end{tabular}
\end{table}

==> table_contam.tex <==
\begin{table*}
\centering
\caption{Placeholder table for Contaminants. Gaia data from Nicola's DR3 WD catalogue. Systems from DR2 WD catalogue not reproduced in the DR3 one have '--'. \label{t-Contam1}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J003748.95+421102.69 & sdX     & 381560256012678272  & 18.000 & 0.4430 & 381560256012678272  & 17.961 & 0.5681            \\
J013230.30+303446.96 & sdX:    & 303286989598463616  & 19.709 & 0.5534 & --                  & --     & --                \\
J013354.76+320327.04 & STAR    & 315905534795143296  & 19.945 & 0.0089 & --                  & --     & --                \\
J013402.82+250728.31 & UNCLASS & 292106017200971520  & 19.896 & 0.9510 & 292106017200971520  & 19.835 & 0.9918            \\
J013814.00+315247.99 & EXGAL   & 303848389069461760  & 19.887 & 0.0075 & --                  & --     & --                \\
J014143.41+320231.97 & sdX     & 303909583762954368  & 17.891 & 0.8905 & 303909583762954368  & 17.863 & 0.9924            \\
J015354.95-022537.70 & STAR    & 2504924643283490816 & 19.781 & 0.5082 & --                  & --     & --                \\
J015542.95-032832.36 & EXGAL   & 2504250088604443520 & 19.658 & 0.0159 & --                  & --     & --                \\
J020100.39-033405.39 & STAR    & 2492566506248972544 & 19.971 & 0.3576 & 2492566506248972544 & 19.939 & 0.0503            \\
J020352.48-073523.18 & STAR    & 2463440580668438400 & 19.910 & 0.3863 & --                  & --     & --                \\
J020407.94-073924.02 & STAR    & 2463436457499955328 & 19.363 & 0.0139 & --                  & --     & --                \\
J020427.27-060328.06 & STAR    & 2490719807750557056 & 19.131 & 0.0136 & --                  & --     & --                \\
J020718.69-050814.50 & STAR    & 2491345502881853952 & 19.880 & 0.5392 & --                  & --     & --                \\
J022453.77+305852.63 & EXGAL   & 132398276774268928  & 19.820 & 0.0124 & --                  & --     & --                \\
J022652.56-061907.54 & UNCLASS & 2488355101836762752 & 19.690 & 0.0325 & 2488355101836762752 & 19.648 & 0.1718            \\
J022807.62-071557.20 & STAR    & 5178375690068316032 & 18.895 & 0.0284 & --                  & --     & --                \\
J022902.91-041628.48 & EXGAL   & 2489222238553976960 & 19.541 & 0.0095 & --                  & --     & --                \\
J023010.00-045652.90 & STAR    & 2489123248147602816 & 20.312 & 0.0124 & --                  & --     & --                \\
J023041.69-041920.21 & EXGAL   & 2489297864337935872 & 20.033 & 0.0066 & --                  & --     & --                \\
J023120.04-040000.59 & STAR    & 2489335526906754304 & 18.992 & 0.0024 & --                  & --     & --                \\
J023222.43+263419.53 & EXGAL   & 127284035876979840  & 19.728 & 0.0064 & --                  & --     & --                \\
J023324.57-003852.72 & UNCLASS & 2500103555378105472 & 19.863 & 0.0310 & --                  & --     & --                \\
J023417.43+003857.98 & UNCLASS & 2500531269696983296 & 19.920 & 0.3499 & 2500531269696983296 & 19.879 & 0.0766            \\
J023554.22-040046.09 & STAR    & 2495096383720814464 & 19.972 & 0.7893 & 2495096383720814464 & 19.940 & 0.7613            \\
J023602.27-013450.26 & EXGAL   & 2496786878553524096 & 19.606 & 0.0174 & --                  & --     & --                \\
J023626.59-033243.03 & STAR    & 2495326112931510016 & 18.665 & 0.0022 & 2495326112931510016 & 18.636 & 0.0766            \\
J023701.46+011414.77 & UNCLASS & 2502079240334810496 & 20.010 & 0.6520 & --                  & --     & --                \\
J053941.49-193804.95 & EXGAL   & 2967059894518912768 & 20.414 & 0.0162 & --                  & --     & --                \\
J054244.63-190436.43 & STAR    & 2967193382105185152 & 19.952 & 0.8546 & --                  & --     & --                \\
J055009.83-233802.25 & EXGAL   & 2915728915003377792 & 20.654 & 0.0292 & --                  & --     & --                \\
J055034.13-214431.76 & sdX     & 2917615883114362752 & 18.706 & 0.3339 & 2917615883114362752 & 18.667 & 0.2697            \\
J055130.86-231505.94 & STAR    & 2915764584706902016 & 20.698 & 0.0177 & --                  & --     & --                \\
J065837.72+571235.89 & sdX     & 1000497070938042496 & 16.251 & 0.0863 & 1000497070938042496 & 16.214 & 0.0221            \\
J065942.66+572408.19 & STAR    & 1000587638912716800 & 19.482 & 0.0636 & --                  & --     & --                \\
J070207.74+365145.94 & EXGAL   & 940118210237746688  & 20.240 & 0.0380 & --                  & --     & --                \\
J070358.22+564451.57 & STAR    & 1000503594992328576 & 19.587 & 0.9106 & 1000503594992328576 & 19.630 & 0.2429            \\
J070415.77+572903.78 & STAR    & 1000554206887367296 & 19.476 & 0.9186 & --                  & --     & --                \\
J070617.53+570800.62 & EXGAL   & 988533040102609408  & 19.582 & 0.0197 & --                  & --     & --                \\
J071055.69+545338.02 & EXGAL   & 988052416082164736  & 20.341 & 0.0364 & --                  & --     & --                \\
J071200.21+565656.87 & EXGAL   & 989958007171463552  & 19.836 & 0.0113 & --                  & --     & --                \\
J072106.97+413545.51 & UNCLASS & 948884169768747648  & 19.795 & 0.9898 & 948884169768747648  & 19.741 & 0.9978            \\
J072859.56+433719.07 & STAR    & 973029689929125120  & 20.295 & 0.0091 & --                  & --     & --                \\
J073222.20+310556.18 & STAR    & 891875282141915392  & 19.883 & 0.2757 & --                  & --     & --                \\
J073246.05+180831.49 & EXGAL   & 3170146632836394880 & 19.776 & 0.1533 & --                  & --     & --                \\
J073827.39+152629.77 & EXGAL   & 3165775657503569664 & 19.966 & 0.0097 & --                  & --     & --                \\
J074035.04+162837.42 & EXGAL   & 3165977658405563136 & 20.001 & 0.0138 & --                  & --     & --                \\
J074236.21+181117.76 & STAR    & 671256178084465024  & 20.182 & 0.0103 & --                  & --     & --                \\
J074253.55+182159.10 & EXGAL   & 671277343683911936  & 20.309 & 0.2944 & --                  & --     & --                \\
J074410.51+383247.31 & STAR    & 920174924734438272  & 19.903 & 0.9929 & 920174924734438272  & 19.876 & 0.9447            \\
J075030.98+684108.79 & UNCLASS & 1096533467390090880 & 19.782 & 0.9983 & 1096533467390090880 & 19.724 & 0.9934            \\
J080102.79+393343.66 & STAR    & 921268526487432704  & 19.878 & 0.2540 & --                  & --     & --                \\
J080537.13+401756.92 & STAR    & 921213791424420992  & 19.997 & 0.9675 & 921213791424420992  & 19.959 & 0.0679            \\
J081547.91+333046.28 & EXGAL   & 902465232681526016  & 20.114 & 0.0420 & --                  & --     & --                \\
J081642.27+315841.36 & EXGAL   & 901181655934487424  & 20.282 & 0.0160 & --                  & --     & --                \\
J081728.65+310628.19 & EXGAL   & 900882554412133120  & 19.951 & 0.0289 & --                  & --     & --                \\
J082048.28+332414.29 & EXGAL   & 901738730371968000  & 20.085 & 0.0609 & --                  & --     & --                \\
J082423.26+311334.12 & EXGAL   & 709076388782944128  & 20.046 & 0.0128 & --                  & --     & --                \\
J082649.62+323054.61 & EXGAL   & 709298288269010816  & 19.796 & 0.0204 & --                  & --     & --                \\
J082847.12+312328.75 & EXGAL   & 708976986060001408  & 20.310 & 0.0491 & --                  & --     & --                \\
J082939.55+335031.55 & STAR    & 903126241031541376  & 19.669 & 0.0131 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J083047.51+331454.93 & STAR    & 710936143981579136  & 19.557 & 0.3286 & 710936143981579136  & 19.509 & 0.3851            \\
J083053.71+012308.09 & STAR    & 3077853794303489920 & 19.456 & 0.0874 & --                  & --     & --                \\
J083107.92+001331.38 & STAR    & 3076962575704962176 & 17.952 & 0.6628 & 3076962575704962176 & 17.922 & 0.8185            \\
J083217.88+334307.83 & STAR    & 710974592529008896  & 19.957 & 0.2379 & 710974592529008896  & 19.916 & 0.0392            \\
J083541.60+312147.88 & STAR    & 709653872905637504  & 20.057 & 0.0216 & --                  & --     & --                \\
J083709.10+201159.48 & STAR    & 664390900497235328  & 17.936 & 0.0033 & --                  & --     & --                \\
J083819.26+184608.88 & STAR    & 659690312192901760  & 19.917 & 0.6553 & 659690312192901760  & 19.870 & 0.0520            \\
J084014.86+004239.04 & sdX     & 3078353045597053696 & 16.503 & 0.0960 & 3078353045597053696 & 16.474 & 0.0514            \\
J084019.25-055512.20 & STAR    & 5755284179827691904 & 19.995 & 0.0154 & --                  & --     & --                \\
J084110.90+202912.32 & STAR    & 664437728524069376  & 19.588 & 0.0025 & --                  & --     & --                \\
J084242.27-071615.43 & STAR    & 5754049947960923136 & 19.262 & 0.0074 & --                  & --     & --                \\
J084306.22+184245.44 & STAR    & 660936333745391488  & 20.284 & 0.1375 & --                  & --     & --                \\
J084736.00+232510.39 & EXGAL   & 689394787048107776  & 20.078 & 0.0264 & --                  & --     & --                \\
J084752.12+192318.93 & STAR    & 661089165861254144  & 19.940 & 0.2106 & --                  & --     & --                \\
J084829.65+100054.73 & STAR    & 598446827331165440  & 18.428 & 0.4012 & --                  & --     & --                \\
J084912.41+220717.01 & STAR    & 686050656792080256  & 20.190 & 0.5535 & --                  & --     & --                \\
J085444.16+001522.92 & STAR    & 3074705205317631360 & 18.148 & 0.5862 & --                  & --     & --                \\
J085651.76+315048.61 & EXGAL   & 711986589902953856  & 19.900 & 0.0050 & --                  & --     & --                \\
J090041.93+011550.88 & UNCLASS & 576696563188488576  & 19.930 & 0.9953 & 576696563188488576  & 19.869 & 0.9951            \\
J090044.35+311401.98 & STAR    & 711797478199952640  & 19.311 & 0.1019 & --                  & --     & --                \\
J091328.49+312942.17 & STAR    & 699974322290911104  & 20.088 & 0.1261 & --                  & --     & --                \\
J091354.30-002541.59 & EXGAL   & 3842420305851802880 & 19.767 & 0.0035 & --                  & --     & --                \\
J091615.62+324101.03 & STAR    & 701761337923277696  & 19.442 & 0.5717 & --                  & --     & --                \\
J091913.69+332455.76 & STAR    & 701902522087907584  & 19.160 & 0.1539 & --                  & --     & --                \\
J092038.25+322845.82 & EXGAL   & 701589303009610368  & 19.695 & 0.0322 & --                  & --     & --                \\
J092427.94+330155.21 & EXGAL   & 701278411800474496  & 19.578 & 0.0105 & --                  & --     & --                \\
J092558.25+315907.22 & STAR    & 700961133976224768  & 19.975 & 0.3748 & --                  & --     & --                \\
J092611.67+330757.38 & EXGAL   & 701271922106548992  & 19.087 & 0.0036 & --                  & --     & --                \\
J092741.00+310516.60 & STAR    & 697481626351426432  & 19.546 & 0.3456 & --                  & --     & --                \\
J092841.50+320558.02 & EXGAL   & 700930622528606336  & 19.766 & 0.0404 & --                  & --     & --                \\
J093006.80+314258.35 & sdX     & 697904599026844160  & 17.281 & 0.2798 & 697904599026844160  & 17.254 & 0.1235            \\
J093033.77+634004.41 & EXGAL   & 1064401438362327296 & 20.027 & 0.0034 & --                  & --     & --                \\
J093559.83+685201.55 & sdX     & 1070853961005794048 & 16.697 & 0.8800 & 1070853961005794048 & 16.665 & 0.9762            \\
J094111.52+331443.86 & STAR    & 794031357294206720  & 19.770 & 0.3940 & --                  & --     & --                \\
J094146.01+310915.12 & STAR    & 792946070597824768  & 19.940 & 0.0180 & --                  & --     & --                \\
J094725.25+650036.77 & EXGAL   & 1064785752036285440 & 20.602 & 0.0134 & --                  & --     & --                \\
J094954.65+692017.89 & EXGAL   & 1070916388354444672 & 20.571 & 0.0208 & --                  & --     & --                \\
J095034.25+323505.93 & STAR    & 793330457285789568  & 19.922 & 0.0108 & --                  & --     & --                \\
J095235.30+313033.79 & EXGAL   & 745151640167867136  & 19.335 & 0.0015 & --                  & --     & --                \\
J095405.84+312505.68 & EXGAL   & 745123705700753664  & 20.056 & 0.0118 & --                  & --     & --                \\
J095430.39+021526.06 & EXGAL   & 3846819035262106752 & 19.548 & 0.0118 & --                  & --     & --                \\
J095451.89+331600.46 & STAR    & 794957386602396416  & 19.772 & 0.0333 & --                  & --     & --                \\
J095523.98+013654.36 & EXGAL   & 3834747462741043456 & 19.606 & 0.0065 & --                  & --     & --                \\
J095526.24+014651.49 & EXGAL   & 3834758595296291584 & 19.306 & 0.0071 & --                  & --     & --                \\
J095553.82+321004.98 & STAR    & 745288529365502080  & 19.131 & 0.0358 & --                  & --     & --                \\
J095617.05+693217.50 & EXGAL   & 1070536648822055040 & 20.480 & 0.0950 & --                  & --     & --                \\
J095619.73+032059.25 & STAR    & 3848458647617328640 & 19.978 & 0.0210 & --                  & --     & --                \\
J095622.29+311958.43 & STAR    & 744923117843262336  & 19.554 & 0.0232 & --                  & --     & --                \\
J095632.68+032152.83 & EXGAL   & 3848458548832927360 & 19.858 & 0.0841 & --                  & --     & --                \\
J095637.29+312104.34 & EXGAL   & 745016297158909312  & 19.859 & 0.0129 & --                  & --     & --                \\
J095657.70+033213.08 & UNCLASS & 3848556332353501184 & 19.613 & 0.4661 & --                  & --     & --                \\
J095724.28+362133.05 & STAR    & 796629297111944704  & 19.183 & 0.0881 & --                  & --     & --                \\
J095733.31+334421.82 & STAR    & 794953881908970240  & 19.689 & 0.0696 & --                  & --     & --                \\
J095836.57+354414.53 & EXGAL   & 795813150246298496  & 18.630 & 0.0019 & --                  & --     & --                \\
J095945.68+320242.74 & STAR    & 746561557672860032  & 19.478 & 0.3593 & 746561557672860032  & 19.439 & 0.8288            \\
J095951.21+034701.53 & EXGAL   & 3848581208804556800 & 19.678 & 0.0066 & --                  & --     & --                \\
J100005.13+324024.98 & EXGAL   & 746794757216316672  & 19.759 & 0.0082 & --                  & --     & --                \\
J100108.69+005730.78 & EXGAL   & 3833678703079340544 & 19.729 & 0.0111 & --                  & --     & --                \\
J100114.82+382054.95 & EXGAL   & 802896582109442048  & 19.848 & 0.0080 & --                  & --     & --                \\
J100115.45+321950.74 & EXGAL   & 746595028352571904  & 20.096 & 0.0179 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J100310.67+004044.51 & UNCLASS & 3833611357992285056 & 19.764 & 0.5280 & 3833611357992285056 & 19.725 & 0.9922            \\
J100317.06+025510.33 & sdX     & 3836406625787704064 & 18.548 & 0.5707 & --                  & --     & --                \\
J100341.36+013846.52 & STAR    & 3835979259361419776 & 19.966 & 0.6855 & --                  & --     & --                \\
J100415.27+395403.68 & STAR    & 803632876942907648  & 19.734 & 0.2274 & --                  & --     & --                \\
J100420.51+022436.34 & STAR    & 3836164836308476544 & 19.432 & 0.2047 & --                  & --     & --                \\
J100438.01+020924.36 & EXGAL   & 3836109349626313472 & 20.241 & 0.3923 & --                  & --     & --                \\
J100448.49+010232.56 & STAR    & 3835126558029426816 & 18.092 & 0.0782 & --                  & --     & --                \\
J101232.09+002209.09 & STAR    & 3831884643701293184 & 18.328 & 0.7304 & 3831884643701293184 & 18.309 & 0.8633            \\
J101356.31+405926.82 & STAR    & 805074581504158848  & 19.981 & 0.4283 & --                  & --     & --                \\
J101428.51-004631.85 & STAR    & 3831474594582695808 & 19.900 & 0.0189 & --                  & --     & --                \\
J102104.99+440355.48 & EXGAL   & 806081111381255296  & 19.858 & 0.0120 & --                  & --     & --                \\
J102143.03+322227.35 & EXGAL   & 749012545184800512  & 19.654 & 0.0029 & --                  & --     & --                \\
J102431.10+332150.24 & EXGAL   & 749175852725608448  & 20.297 & 0.0308 & --                  & --     & --                \\
J102431.94+803138.76 & UNCLASS & 1133840373660526848 & 19.683 & 0.0026 & --                  & --     & --                \\
J102459.67+424316.60 & STAR    & 804964973941402240  & 19.533 & 0.1245 & --                  & --     & --                \\
J102642.72+101540.23 & STAR    & 3876383807716818048 & 19.693 & 0.1766 & --                  & --     & --                \\
J102900.47+793200.05 & UNCLASS & 1132966468074614272 & 18.839 & 0.9850 & 1132966468074614272 & 18.811 & 1.0000            \\
J103000.44-234803.49 & sdX     & 5474237501551920640 & 15.089 & 0.1386 & 5474237501551920640 & 15.071 & 0.1431            \\
J103036.94+791654.55 & UNCLASS & 1132758626017491712 & 19.260 & 0.9992 & 1132758626017491712 & 19.209 & 0.9923            \\
J103225.18-241109.21 & EXGAL   & 5471165530486853888 & 20.340 & 0.0076 & --                  & --     & --                \\
J103243.85+321003.00 & STAR    & 748443204319596672  & 19.808 & 0.3069 & --                  & --     & --                \\
J103303.62+321554.02 & EXGAL   & 748445467766978816  & 19.290 & 0.0028 & --                  & --     & --                \\
J103314.77-260526.33 & EXGAL   & 5469229805906418816 & 19.975 & 0.0042 & --                  & --     & --                \\
J103644.42-261506.71 & sdX     & 5468473341906356096 & 18.608 & 0.5243 & 5468473341906356096 & 18.559 & 0.2978            \\
J103742.46+102023.65 & EXGAL   & 3870192934481613696 & 18.982 & 0.0198 & --                  & --     & --                \\
J103747.64+332825.46 & STAR    & 748628575108175104  & 19.917 & 0.2760 & --                  & --     & --                \\
J103756.62-251123.94 & STAR    & 5470799186955866624 & 19.934 & 0.2353 & --                  & --     & --                \\
J104222.98+802002.82 & UNCLASS & 1133154518922989184 & 19.960 & 0.0817 & --                  & --     & --                \\
J104408.90+803445.05 & UNCLASS & 1133175581442675200 & 19.772 & 0.9910 & 1133175581442675200 & 19.717 & 0.9491            \\
J104754.06+802834.62 & UNCLASS & 1133160085200468736 & 19.923 & 0.9987 & 1133160085200468736 & 19.867 & 0.9951            \\
J104814.66+470140.92 & STAR    & 832075456047122816  & 19.915 & 0.0041 & --                  & --     & --                \\
J104849.94+784321.42 & UNCLASS & 1129680680654544256 & 19.462 & 0.9673 & 1129680680654544256 & 19.418 & 0.9867            \\
J105405.41-263659.09 & STAR    & 5457849379522645120 & 19.765 & 0.1422 & 5457849379522645120 & 19.740 & 0.2841            \\
J105416.72+792239.60 & UNCLASS & 1132809925106843008 & 19.716 & 0.9933 & 1132809925106843008 & 19.637 & 0.9966            \\
J105453.29+783025.72 & UNCLASS & 1129706622256790400 & 19.635 & 0.9863 & 1129706622256790400 & 19.576 & 0.9782            \\
J105528.60+323147.77 & EXGAL   & 737210211277910656  & 19.834 & 0.0345 & --                  & --     & --                \\
J105644.54+330221.04 & EXGAL   & 737251580403181824  & 18.668 & 0.0126 & --                  & --     & --                \\
J105704.73+804944.52 & UNCLASS & 1133196716976678016 & 19.998 & 0.9758 & 1133196716976678016 & 19.946 & 0.9674            \\
J105711.65+471119.60 & STAR    & 831565145212907648  & 19.705 & 0.2752 & --                  & --     & --                \\
J105714.85+802810.20 & UNCLASS & 1133121430494537472 & 19.289 & 0.0114 & --                  & --     & --                \\
J105715.92+332742.17 & STAR    & 737404863490884352  & 19.891 & 0.2900 & --                  & --     & --                \\
J105733.03+524332.36 & UNCLASS & 837327827390030208  & 20.152 & 0.9485 & 837327827390030208  & 20.083 & 0.9799            \\
J105741.78+325809.46 & EXGAL   & 737329336490767616  & 19.982 & 0.0087 & --                  & --     & --                \\
J105751.50+520547.50 & STAR    & 836498039706921984  & 20.150 & 0.9743 & 836498039709296512  & 20.088 & 0.9183            \\
J105752.17+503115.28 & STAR    & 836030884704319616  & 19.938 & 0.0143 & --                  & --     & --                \\
J105759.37+470307.40 & sdX     & 831501240400109824  & 17.230 & 0.2913 & 831501240400109824  & 17.217 & 0.0442            \\
J105810.87+784659.38 & UNCLASS & 1129727272459583744 & 19.694 & 0.9757 & 1129727272459583744 & 19.662 & 0.9762            \\
J105817.24+784951.16 & UNCLASS & 1129729785016172288 & 19.851 & 0.9927 & 1129729785016172288 & 19.796 & 0.9667            \\
J105822.62+320450.83 & STAR    & 736959900584035968  & 19.962 & 0.0173 & --                  & --     & --                \\
J105853.96+524300.20 & STAR    & 837281093848812672  & 20.402 & 0.9423 & 837281093848812672  & 20.340 & 0.5169            \\
J110011.55+515807.94 & EXGAL   & 836460342779044992  & 20.247 & 0.0273 & --                  & --     & --                \\
J110147.00+523934.40 & STAR    & 836541779655583488  & 20.381 & 0.9936 & 836541779656234368  & 20.327 & 0.9939            \\
J110217.42+505825.39 & STAR    & 836157358605716864  & 19.813 & 0.0323 & --                  & --     & --                \\
J110236.64+313149.24 & STAR    & 733869413916772736  & 18.963 & 0.1923 & --                  & --     & --                \\
J110255.97+521858.12 & sdX     & 836471823228155392  & 17.105 & 0.1220 & --                  & --     & --                \\
J110309.63+522445.17 & STAR    & 842478008573717248  & 20.392 & 0.0132 & --                  & --     & --                \\
J110333.58+501518.79 & STAR    & 833063710842279296  & 19.425 & 0.0208 & --                  & --     & --                \\
J110346.23+784444.51 & UNCLASS & 1129735763610587264 & 19.719 & 0.9804 & 1129735763610587264 & 19.661 & 0.9653            \\
J110414.01+502932.83 & EXGAL   & 833075083915323264  & 19.535 & 0.0041 & --                  & --     & --                \\
J110442.90+524556.86 & EXGAL   & 842538717935032576  & 20.065 & 0.0143 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J110505.06+792610.72 & UNCLASS & 1129832000941901056 & 19.149 & 0.9896 & 1129832000941901056 & 19.129 & 0.9611            \\
J110527.70+523804.66 & EXGAL   & 842487693723492992  & 19.948 & 0.0064 & --                  & --     & --                \\
J110538.37+500517.70 & STAR    & 832861503781801216  & 20.038 & 0.6440 & --                  & --     & --                \\
J110603.25+504553.32 & STAR    & 839095219315053824  & 19.802 & 0.9962 & 839095219315053824  & 19.735 & 0.9927            \\
J110605.76+694225.68 & EXGAL   & 1072675538239660288 & 19.893 & 0.0020 & --                  & --     & --                \\
J110639.56+524110.56 & EXGAL   & 842508004625241216  & 19.994 & 0.0173 & 842508004625241216  & 19.979 & 0.1531            \\
J110758.92+320635.42 & STAR    & 757827428688306432  & 19.144 & 0.0103 & --                  & --     & --                \\
J110800.64+501400.22 & STAR    & 838826393018353152  & 17.455 & 0.9952 & 838826393018353152  & 17.429 & 0.9893            \\
J110914.52+802442.79 & UNCLASS & 1133296699520406656 & 18.907 & 0.9996 & 1133296699520406656 & 18.864 & 0.9994            \\
J110945.71+505424.48 & UNCLASS & 838922389831369216  & 18.647 & 0.9987 & 838922389831369216  & 18.616 & 0.9992            \\
J111016.81+524319.23 & EXGAL   & 842403512364524928  & 20.299 & 0.0073 & --                  & --     & --                \\
J111058.51+502053.29 & UNCLASS & 838840510574586880  & 17.578 & 0.9819 & 838840510574586880  & 17.542 & 0.9980            \\
J111257.59+690255.98 & UNCLASS & 1062019690018642048 & 19.790 & 0.9776 & 1062019690018642048 & 19.707 & 0.9368            \\
J111724.14+802505.61 & UNCLASS & 1133252959572911104 & 19.239 & 0.9992 & 1133252959572911104 & 19.197 & 0.9992            \\
J111752.16+550937.79 & UNCLASS & 843967876892449920  & 19.948 & 0.7942 & 843967876892449920  & 19.911 & 0.9755            \\
J111823.74+514758.63 & EXGAL   & 839433697097976448  & 20.718 & 0.0323 & --                  & --     & --                \\
J111953.57+515718.19 & EXGAL   & 839439091576744320  & 20.443 & 0.0227 & --                  & --     & --                \\
J112119.68+540313.57 & EXGAL   & 842869297273822208  & 20.648 & 0.0354 & --                  & --     & --                \\
J112157.25+534038.70 & EXGAL   & 842798584932264192  & 20.514 & 0.0097 & --                  & --     & --                \\
J112202.34+323819.55 & STAR    & 757385394949495936  & 19.704 & 0.0063 & --                  & --     & --                \\
J112341.02+315151.26 & STAR    & 4023819207375763200 & 19.861 & 0.2860 & --                  & --     & --                \\
J112341.64+333508.80 & STAR    & 759138699383421184  & 19.488 & 0.4606 & 759138699383421184  & 19.437 & 0.0865            \\
J112445.61+320821.88 & STAR    & 4023922664547648128 & 19.939 & 0.0263 & --                  & --     & --                \\
J112457.14+504906.75 & EXGAL   & 838349372474789248  & 20.231 & 0.0197 & --                  & --     & --                \\
J112517.83+330936.50 & EXGAL   & 758879455157841920  & 19.895 & 0.0060 & --                  & --     & --                \\
J112534.12+792005.08 & UNCLASS & 1129965488525849344 & 19.505 & 0.9954 & 1129965488525849344 & 19.460 & 0.9925            \\
J112547.95+512640.08 & EXGAL   & 838659950149738112  & 20.672 & 0.0293 & --                  & --     & --                \\
J112649.30+332108.15 & EXGAL   & 758886120951547136  & 20.135 & 0.0107 & --                  & --     & --                \\
J112715.67+504350.53 & STAR    & 838377444380532736  & 19.984 & 0.0070 & --                  & --     & --                \\
J112757.71+493155.06 & EXGAL   & 790033636094324992  & 20.639 & 0.0299 & --                  & --     & --                \\
J112810.26+305354.11 & STAR    & 4023468153928538240 & 19.978 & 0.2640 & 4023468153928538240 & 19.914 & 0.0566            \\
J112838.24+531757.77 & EXGAL   & 839630509679779840  & 20.186 & 0.0493 & --                  & --     & --                \\
J112849.66+325040.41 & STAR    & 4025456826865896064 & 19.527 & 0.1680 & --                  & --     & --                \\
J112941.08+503637.93 & EXGAL   & 790348165139657856  & 20.115 & 0.0145 & --                  & --     & --                \\
J112949.37+493526.15 & EXGAL   & 789993160322550528  & 20.316 & 0.0336 & --                  & --     & --                \\
J112954.40+515114.45 & EXGAL   & 838693004225505920  & 19.773 & 0.0032 & --                  & --     & --                \\
J112954.78+510000.26 & sdX     & 838410876406247680  & 17.755 & 0.7271 & 838410876406247680  & 17.719 & 0.9788            \\
J113102.80+792119.18 & UNCLASS & 1129959892182939008 & 19.538 & 0.9767 & 1129959892182939008 & 19.517 & 0.9853            \\
J113113.64+531536.02 & EXGAL   & 841118045832920960  & 20.075 & 0.0056 & --                  & --     & --                \\
J113242.88+545222.67 & EXGAL   & 844453723592772480  & 20.352 & 0.0093 & --                  & --     & --                \\
J113256.43+320724.16 & STAR    & 4025148894890743296 & 19.956 & 0.5105 & --                  & --     & --                \\
J113313.31+525551.90 & EXGAL   & 840301147349004032  & 20.173 & 0.0249 & --                  & --     & --                \\
J113521.78+525120.11 & EXGAL   & 840262011606126336  & 20.406 & 0.1004 & --                  & --     & --                \\
J113525.12+532109.66 & EXGAL   & 841085782037928064  & 20.335 & 0.0095 & --                  & --     & --                \\
J113600.30+513621.95 & EXGAL   & 791917202592403456  & 20.338 & 0.0160 & --                  & --     & --                \\
J113624.05+500356.74 & EXGAL   & 790768663912416640  & 20.495 & 0.0129 & --                  & --     & --                \\
J113633.61+750653.85 & sdX     & 1079494159598957952 & 13.171 & 0.0511 & 1079494159598957952 & 13.153 & 0.0244            \\
J113651.04+555245.21 & EXGAL   & 844659332268007296  & 20.425 & 0.0127 & --                  & --     & --                \\
J113658.15+493449.24 & STAR    & 790716467174928768  & 19.804 & 0.3261 & --                  & --     & --                \\
J113714.33+535105.07 & EXGAL   & 841116671443008640  & 20.242 & 0.0087 & --                  & --     & --                \\
J113723.10+503603.82 & STAR    & 791568554327066752  & 20.293 & 0.3740 & --                  & --     & --                \\
J113854.07+535051.08 & EXGAL   & 841195767560442496  & 20.431 & 0.0419 & --                  & --     & --                \\
J113855.13+535530.19 & UNCLASS & 841208240145481728  & 19.880 & 0.1744 & --                  & --     & --                \\
J113927.30+003127.36 & STAR    & 3798831571822624512 & 19.955 & 0.2852 & --                  & --     & --                \\
J113948.99+801423.48 & UNCLASS & 1130293830185522432 & 19.807 & 0.2351 & 1130293830185522432 & 19.778 & 0.6734            \\
J113949.44+510038.37 & EXGAL   & 791720733608593024  & 20.754 & 0.0144 & --                  & --     & --                \\
J114026.18+510231.59 & EXGAL   & 791722176717610496  & 20.532 & 0.0386 & --                  & --     & --                \\
J114038.69+541146.11 & EXGAL   & 841221159407282688  & 20.049 & 0.0047 & --                  & --     & --                \\
J114113.63+005138.31 & STAR    & 3798938361889055488 & 19.865 & 0.2227 & --                  & --     & --                \\
J114118.50+510719.17 & EXGAL   & 791727953448757504  & 20.520 & 0.0359 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J114118.98+551048.91 & EXGAL   & 841575614468793088  & 20.384 & 0.0116 & --                  & --     & --                \\
J114127.80+510232.11 & EXGAL   & 791679605001280000  & 19.501 & 0.0035 & --                  & --     & --                \\
J114128.97+531623.95 & STAR    & 840359588967666432  & 19.069 & 0.0012 & 840359588967666432  & 19.037 & 0.0593            \\
J114233.30+533045.38 & EXGAL   & 840397384679982208  & 20.397 & 0.0979 & --                  & --     & --                \\
J114330.72+542510.07 & STAR    & 841249987227866496  & 19.982 & 0.5145 & --                  & --     & --                \\
J114345.00+532121.64 & EXGAL   & 840199541306698880  & 20.503 & 0.0157 & --                  & --     & --                \\
J114402.68+533811.63 & EXGAL   & 840405699736738304  & 20.674 & 0.1131 & --                  & --     & --                \\
J114429.18+523958.42 & EXGAL   & 792068213641945344  & 20.752 & 0.0615 & --                  & --     & --                \\
J114430.04+804827.19 & UNCLASS & 1130368081579922688 & 19.002 & 0.9291 & 1130368081579922688 & 18.956 & 0.9804            \\
J114434.83+550439.30 & sdX     & 841328602308941184  & 18.803 & 0.4825 & 841328602308941184  & 18.761 & 0.4427            \\
J114435.30+532704.97 & EXGAL   & 840201740329904000  & 20.547 & 0.0132 & --                  & --     & --                \\
J114531.79+714250.86 & sdX     & 1074719530355569536 & 18.776 & 0.5170 & 1074719530355569536 & 18.731 & 0.2580            \\
J114609.78+562524.60 & STAR    & 845019834642656256  & 19.904 & 0.0245 & --                  & --     & --                \\
J114620.14+004059.13 & EXGAL   & 3796255244279616640 & 19.321 & 0.0060 & --                  & --     & --                \\
J114645.75+561644.50 & EXGAL   & 845002757852642432  & 19.945 & 0.0065 & --                  & --     & --                \\
J114653.48+511028.96 & EXGAL   & 791315082537237376  & 20.641 & 0.0357 & --                  & --     & --                \\
J114902.19+512121.30 & EXGAL   & 791313227115725824  & 20.783 & 0.0288 & --                  & --     & --                \\
J114945.24+505023.26 & EXGAL   & 791073396137773312  & 20.496 & 0.0318 & --                  & --     & --                \\
J115133.90+785741.19 & UNCLASS & 1129191947735781632 & 19.523 & 0.6354 & 1129191947735781632 & 19.464 & 0.9917            \\
J115205.17+562405.80 & EXGAL   & 842107503221786496  & 20.683 & 0.0145 & --                  & --     & --                \\
J115229.65-004110.21 & EXGAL   & 3794934185355466624 & 20.096 & 0.0420 & --                  & --     & --                \\
J115233.98+552245.48 & EXGAL   & 841769746990552960  & 20.497 & 0.0410 & --                  & --     & --                \\
J115306.42+534947.92 & EXGAL   & 840643228608455552  & 20.210 & 0.0060 & --                  & --     & --                \\
J115320.77+512345.90 & EXGAL   & 791371432507602432  & 20.473 & 0.0081 & --                  & --     & --                \\
J115331.13+521837.75 & EXGAL   & 792229566974122880  & 20.603 & 0.0513 & --                  & --     & --                \\
J115404.20+510635.27 & EXGAL   & 791162662737931904  & 20.456 & 0.0091 & --                  & --     & --                \\
J115457.54+522257.60 & EXGAL   & 792224932704210816  & 20.208 & 0.0196 & --                  & --     & --                \\
J115537.61+550215.87 & EXGAL   & 840941024460776832  & 19.669 & 0.0035 & --                  & --     & --                \\
J115618.80+531302.40 & EXGAL   & 792504788477845760  & 20.542 & 0.0123 & --                  & --     & --                \\
J115625.45+520355.77 & EXGAL   & 791449326035022464  & 20.359 & 0.0296 & --                  & --     & --                \\
J115708.14+521424.35 & EXGAL   & 791477878977677696  & 20.462 & 0.0175 & --                  & --     & --                \\
J115733.96+282754.96 & STAR    & 4007951674038723840 & 19.265 & 0.0073 & 4007951674038723840 & 19.239 & 0.1924            \\
J115737.52+541754.98 & EXGAL   & 840680165326652032  & 20.623 & 0.0572 & --                  & --     & --                \\
J115745.10-002147.22 & EXGAL   & 3794996681422992896 & 20.050 & 0.0036 & --                  & --     & --                \\
J115752.39+763448.07 & UNCLASS & 1079731727125032064 & 19.920 & 0.9771 & 1079731727125032064 & 19.870 & 0.9948            \\
J115800.84+790012.12 & UNCLASS & 1129183529599654912 & 19.878 & 0.9298 & 1129183529599654912 & 19.821 & 0.6922            \\
J115818.08+571939.31 & EXGAL   & 845174178587035648  & 20.768 & 0.0263 & --                  & --     & --                \\
J115819.47-010411.12 & STAR    & 3602664438136130048 & 18.807 & 0.2624 & --                  & --     & --                \\
J115825.27+273027.80 & STAR    & 4007287775174260992 & 18.608 & 0.0429 & --                  & --     & --                \\
J115828.03-000513.05 & STAR    & 3795029288814897536 & 19.771 & 0.0035 & --                  & --     & --                \\
J115829.09+003305.33 & STAR    & 3891188968007997184 & 19.683 & 0.2764 & --                  & --     & --                \\
J115915.21+293219.57 & EXGAL   & 4008186557210901888 & 19.467 & 0.0064 & --                  & --     & --                \\
J120006.22-000329.44 & STAR    & 3602878533666072832 & 19.655 & 0.0718 & --                  & --     & --                \\
J120026.50+552539.39 & EXGAL   & 1573409527419167744 & 20.645 & 0.0156 & --                  & --     & --                \\
J120052.23-020233.35 & STAR    & 3602332694862136704 & 19.901 & 0.0050 & --                  & --     & --                \\
J120058.06+563831.52 & STAR    & 1573961890277700352 & 19.713 & 0.0054 & --                  & --     & --                \\
J120134.19+572212.03 & EXGAL   & 1575505986856080640 & 20.125 & 0.0060 & --                  & --     & --                \\
J120152.16+012755.40 & EXGAL   & 3891378599403608832 & 20.153 & 0.0171 & --                  & --     & --                \\
J120154.85+580425.76 & EXGAL   & 1575644933342143616 & 20.378 & 0.0104 & --                  & --     & --                \\
J120224.20+273029.17 & STAR    & 4006908379238662272 & 20.114 & 0.1736 & 4006908379238662272 & 20.077 & 0.0745            \\
J120225.91+531835.34 & EXGAL   & 1549078739550658560 & 20.265 & 0.0149 & --                  & --     & --                \\
J120250.47+001522.36 & STAR    & 3698976678863434112 & 19.706 & 0.2279 & --                  & --     & --                \\
J120258.98+711640.15 & EXGAL   & 1684190988979096192 & 19.984 & 0.0053 & --                  & --     & --                \\
J120310.61+520456.08 & STAR    & 1548640515447850368 & 19.895 & 0.2131 & --                  & --     & --                \\
J120336.30+544426.31 & EXGAL   & 1573280983343017856 & 20.258 & 0.0049 & --                  & --     & --                \\
J120347.43-002310.94 & UNCLASS & 3698872156539379968 & 15.193 & 0.9996 & 3698872156539379968 & 15.175 & 0.9994            \\
J120352.69-002242.93 & STAR    & 3698684513711307648 & 19.844 & 0.2760 & --                  & --     & --                \\
J120357.14+005431.72 & STAR    & 3891262738366041472 & 19.831 & 0.0080 & --                  & --     & --                \\
J120417.18+542022.45 & EXGAL   & 1573221712793972480 & 20.118 & 0.0207 & --                  & --     & --                \\
J120443.21+532217.18 & EXGAL   & 1549127500314582656 & 20.418 & 0.0139 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J120449.29+284010.25 & STAR    & 4007832312603262080 & 19.958 & 0.0061 & --                  & --     & --                \\
J120503.68+265020.66 & EXGAL   & 4006638582277752832 & 19.401 & 0.0027 & --                  & --     & --                \\
J120547.35+565107.69 & EXGAL   & 1575433109850994816 & 20.345 & 0.1752 & --                  & --     & --                \\
J120629.50-002316.88 & UNCLASS & 3698696196022603520 & 20.015 & 0.0780 & --                  & --     & --                \\
J120632.59-003521.85 & STAR    & 3698637475229659648 & 19.825 & 0.6676 & --                  & --     & --                \\
J120718.43+532014.26 & EXGAL   & 1548947794588126720 & 20.555 & 0.0193 & 1548947794588126720 & 20.476 & 0.6718            \\
J120728.43+540129.16 & sdX     & 1573011744729727104 & 15.959 & 0.3814 & 1573011744729727104 & 15.934 & 0.6140            \\
J120743.16+534849.95 & EXGAL   & 1572985180355171712 & 20.551 & 0.0105 & --                  & --     & --                \\
J120806.46-010754.52 & STAR    & 3697820297572207488 & 19.508 & 0.1978 & --                  & --     & --                \\
J120829.66+535516.66 & EXGAL   & 1573007376746193536 & 20.678 & 0.0169 & --                  & --     & --                \\
J120838.15+522619.15 & EXGAL   & 1548801662620508672 & 20.657 & 0.0145 & --                  & --     & --                \\
J120844.77+525120.61 & EXGAL   & 1548913228691177088 & 19.839 & 0.0084 & --                  & --     & --                \\
J120855.19+530819.07 & EXGAL   & 1548941614130401920 & 20.522 & 0.0405 & --                  & --     & --                \\
J120908.80+002405.07 & STAR    & 3698844630092743296 & 19.398 & 0.1059 & --                  & --     & --                \\
J121013.49+000752.83 & STAR    & 3698786149817801088 & 19.888 & 0.2743 & --                  & --     & --                \\
J121018.48+564410.75 & EXGAL   & 1575221037250003328 & 20.428 & 0.0059 & --                  & --     & --                \\
J121029.95+005442.06 & EXGAL   & 3699273955024514816 & 19.924 & 0.0435 & --                  & --     & --                \\
J121127.91+001554.20 & EXGAL   & 3699157685964458624 & 19.850 & 0.0621 & --                  & --     & --                \\
J121135.69+532636.07 & EXGAL   & 1572915567525502208 & 20.249 & 0.0257 & --                  & --     & --                \\
J121143.94+010323.39 & STAR    & 3699279315142445696 & 19.642 & 0.0151 & --                  & --     & --                \\
J121202.79+751506.70 & STAR    & 1692563082829680512 & 19.863 & 0.0021 & 1692563082829680512 & 19.824 & 0.0460            \\
J121221.60+543810.74 & EXGAL   & 1573464189468172160 & 20.196 & 0.0076 & --                  & --     & --                \\
J121256.07+580641.60 & EXGAL   & 1575731691681795456 & 20.683 & 0.0194 & --                  & --     & --                \\
J121256.72-005537.56 & STAR    & 3697723957160505344 & 19.931 & 0.2891 & --                  & --     & --                \\
J121341.76+540006.78 & EXGAL   & 1573038609748452096 & 20.583 & 0.0165 & --                  & --     & --                \\
J121442.57+562525.65 & EXGAL   & 1575174170567292032 & 20.492 & 0.0152 & --                  & --     & --                \\
J121510.44+444115.93 & EXGAL   & 1538849192603291648 & 20.660 & 0.0460 & --                  & --     & --                \\
J121511.34+570633.52 & EXGAL   & 1575290821879404032 & 18.795 & 0.0030 & --                  & --     & --                \\
J121512.75-002022.04 & STAR    & 3698310851556597632 & 19.938 & 0.0234 & --                  & --     & --                \\
J121536.26+455518.50 & EXGAL   & 1539025599794901504 & 20.509 & 0.0147 & --                  & --     & --                \\
J121540.50-003433.70 & EXGAL   & 3698103353097121408 & 19.868 & 0.0178 & --                  & --     & --                \\
J121552.59+573810.03 & STAR    & 1575700939716325504 & 20.564 & 0.0312 & --                  & --     & --                \\
J121552.99-003534.42 & STAR    & 3698102700262086528 & 19.385 & 0.0263 & --                  & --     & --                \\
J121558.76+453842.36 & EXGAL   & 1538995015332792064 & 19.270 & 0.0026 & --                  & --     & --                \\
J121614.69+553749.96 & STAR    & 1572878081050492544 & 19.969 & 0.0045 & --                  & --     & --                \\
J121625.84-014804.60 & STAR    & 3694582407627057664 & 18.741 & 0.0849 & --                  & --     & --                \\
J121629.17+530034.84 & EXGAL   & 1572149242280430592 & 20.581 & 0.0264 & --                  & --     & --                \\
J121631.13+573926.95 & EXGAL   & 1574955676990971392 & 20.339 & 0.0245 & --                  & --     & --                \\
J121637.68+001204.23 & STAR    & 3698446744322170368 & 19.966 & 0.1923 & 3698446744322170368 & 19.928 & 0.1151            \\
J121654.13+560335.09 & EXGAL   & 1574389909539047680 & 20.441 & 0.0374 & --                  & --     & --                \\
J121707.59+565050.33 & EXGAL   & 1574530715746955136 & 20.408 & 0.0070 & --                  & --     & --                \\
J121737.05+460633.15 & EXGAL   & 1545029375664409856 & 20.644 & 0.0163 & --                  & --     & --                \\
J121753.55+002622.35 & STAR    & 3698480554304426240 & 19.958 & 0.0067 & --                  & --     & --                \\
J121754.74+454930.94 & EXGAL   & 1539012435720669568 & 20.252 & 0.0098 & --                  & --     & --                \\
J121831.19+441332.49 & EXGAL   & 1538633963202090496 & 20.630 & 0.0215 & --                  & --     & --                \\
J121933.24+330433.83 & STAR    & 4016339401570307584 & 19.160 & 0.0082 & --                  & --     & --                \\
J121955.03+313943.85 & sdX     & 4015353487533222272 & 17.275 & 0.2053 & 4015353487533222272 & 17.250 & 0.2645            \\
J122034.67+435720.31 & EXGAL   & 1538568404821191552 & 20.162 & 0.0127 & --                  & --     & --                \\
J122040.67+325040.97 & EXGAL   & 4016282639283022592 & 20.141 & 0.0121 & --                  & --     & --                \\
J122041.15+532249.60 & EXGAL   & 1572218923829499264 & 20.486 & 0.0083 & --                  & --     & --                \\
J122042.37+320104.96 & EXGAL   & 4015471508939495296 & 19.941 & 0.0054 & --                  & --     & --                \\
J122107.60+450804.57 & EXGAL   & 1538744326681956480 & 20.554 & 0.0141 & --                  & --     & --                \\
J122121.76+450231.04 & EXGAL   & 1538741955859981824 & 20.392 & 0.0133 & --                  & --     & --                \\
J122217.26+443047.31 & EXGAL   & 1538691039023281536 & 20.423 & 0.0145 & --                  & --     & --                \\
J122226.45+554007.60 & EXGAL   & 1574326898074311680 & 19.943 & 0.1324 & --                  & --     & --                \\
J122237.39+574004.61 & EXGAL   & 1575011515861390848 & 19.800 & 0.0060 & --                  & --     & --                \\
J122317.72+331552.87 & EXGAL   & 4016664345911126400 & 20.025 & 0.0116 & --                  & --     & --                \\
J122323.44+791906.53 & UNCLASS & 1717851614045315200 & 19.833 & 0.9922 & 1717851614045315200 & 19.789 & 0.9938            \\
J122351.06+435015.79 & EXGAL   & 1535574610752998912 & 19.627 & 0.0061 & --                  & --     & --                \\
J122357.09+443315.12 & EXGAL   & 1535692151122781696 & 20.512 & 0.0182 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J122454.90+575940.19 & EXGAL   & 1575037247010173056 & 20.543 & 0.0377 & --                  & --     & --                \\
J122519.57+434312.26 & EXGAL   & 1535559110215860864 & 20.333 & 0.0278 & --                  & --     & --                \\
J122541.49+561111.37 & EXGAL   & 1574262537989348480 & 20.256 & 0.0057 & --                  & --     & --                \\
J122552.52+543544.13 & EXGAL   & 1572575410411858048 & 20.708 & 0.0361 & --                  & --     & --                \\
J122554.60+560000.87 & EXGAL   & 1574236252789655552 & 20.343 & 0.0358 & --                  & --     & --                \\
J122555.31+612429.28 & sdX     & 1583302860031730048 & 16.812 & 0.4377 & 1583302860031730048 & 16.776 & 0.7657            \\
J122557.77-063543.74 & UNCLASS & 3583688757226156032 & 19.262 & 0.9990 & 3583688757226156032 & 19.221 & 0.9977            \\
J122709.51+583245.83 & EXGAL   & 1580889672526376192 & 20.412 & 0.0099 & --                  & --     & --                \\
J122725.72+622842.09 & EXGAL   & 1583477510581776896 & 20.273 & 0.0292 & --                  & --     & --                \\
J122731.63+333258.25 & EXGAL   & 4016030129565602304 & 20.476 & 0.0669 & --                  & --     & --                \\
J122737.44+310439.59 & EXGAL   & 4012130917735865984 & 19.395 & 0.0060 & --                  & --     & --                \\
J122737.70+571052.37 & EXGAL   & 1574784226192273408 & 20.146 & 0.0031 & --                  & --     & --                \\
J122742.04+573423.88 & EXGAL   & 1574822395565396096 & 19.973 & 0.0026 & --                  & --     & --                \\
J122812.32+551946.21 & EXGAL   & 1574073559428297344 & 20.598 & 0.1098 & --                  & --     & --                \\
J122816.04-073334.90 & UNCLASS & 3583289462706581376 & 19.846 & 0.9737 & 3583289462706581376 & 19.796 & 0.9861            \\
J122824.75+611608.24 & EXGAL   & 1583110342417216128 & 19.901 & 0.0068 & --                  & --     & --                \\
J122838.49+562411.37 & EXGAL   & 1574602050858561280 & 20.524 & 0.0843 & --                  & --     & --                \\
J122843.89+331135.81 & EXGAL   & 4015959898260227200 & 20.276 & 0.0114 & --                  & --     & --                \\
J122917.19+580552.44 & EXGAL   & 1580798069464285952 & 20.306 & 0.0256 & --                  & --     & --                \\
J122944.23+563905.98 & UNCLASS & 1574626991733382784 & 19.895 & 0.7650 & 1574626991733382784 & 19.862 & 0.8590            \\
J123030.72-080549.65 & UNCLASS & 3580206810059875200 & 19.387 & 0.9903 & 3580206810059875200 & 19.342 & 0.9875            \\
J123156.42+572510.84 & STAR    & 1574759482885107328 & 19.963 & 0.0061 & --                  & --     & --                \\
J123256.01+585142.10 & EXGAL   & 1580952688286911232 & 20.571 & 0.0196 & --                  & --     & --                \\
J123309.09+591359.31 & EXGAL   & 1581334012662729856 & 20.423 & 0.0106 & --                  & --     & --                \\
J123345.38+593042.95 & EXGAL   & 1581368234962382336 & 19.957 & 0.0032 & --                  & --     & --                \\
J123422.05-055936.71 & UNCLASS & 3679674679221681536 & 19.735 & 0.9726 & 3679674679221681536 & 19.687 & 0.9468            \\
J123453.46+580131.29 & EXGAL   & 1577897042394481920 & 20.060 & 0.0075 & --                  & --     & --                \\
J123522.70+590520.75 & STAR    & 1578332002321541760 & 19.941 & 0.0025 & --                  & --     & --                \\
J123538.76+604642.70 & STAR    & 1583025959195283072 & 20.227 & 0.9530 & 1583025959195283072 & 20.139 & 0.9595            \\
J123550.46+563311.95 & STAR    & 1571696900620842240 & 19.766 & 0.0049 & --                  & --     & --                \\
J123613.93+550705.76 & EXGAL   & 1571108348366352256 & 20.460 & 0.0334 & --                  & --     & --                \\
J123643.09+542920.77 & EXGAL   & 1571054575375370880 & 20.486 & 0.0129 & --                  & --     & --                \\
J123644.55+551406.23 & EXGAL   & 1571105088487294592 & 19.977 & 0.0026 & --                  & --     & --                \\
J123655.33+553227.03 & EXGAL   & 1571489981980259968 & 20.052 & 0.0146 & --                  & --     & --                \\
J123702.16+540521.48 & EXGAL   & 1570949331497594368 & 20.065 & 0.0033 & --                  & --     & --                \\
J123703.30+630641.01 & EXGAL   & 1583733765510412416 & 20.408 & 0.0245 & --                  & --     & --                \\
J123706.87+621702.14 & EXGAL   & 1583591967165111296 & 20.089 & 0.0627 & --                  & --     & --                \\
J123739.51+555238.69 & EXGAL   & 1571524827050650624 & 20.022 & 0.0042 & --                  & --     & --                \\
J123806.79+610048.63 & STAR    & 1580054696524831488 & 18.917 & 0.0444 & --                  & --     & --                \\
J123929.06+575202.49 & EXGAL   & 1577823340754820992 & 20.501 & 0.0101 & --                  & --     & --                \\
J123939.71+552911.38 & EXGAL   & 1571321584902494976 & 20.484 & 0.1583 & --                  & --     & --                \\
J123946.78+632316.22 & EXGAL   & 1583765273390595072 & 20.127 & 0.0105 & --                  & --     & --                \\
J123953.30+624917.12 & EXGAL   & 1580718286151638528 & 20.337 & 0.0378 & --                  & --     & --                \\
J124001.49+583135.68 & EXGAL   & 1578250642756968576 & 20.016 & 0.0340 & --                  & --     & --                \\
J124002.04+564558.59 & EXGAL   & 1577669477846228096 & 20.336 & 0.0116 & --                  & --     & --                \\
J124042.08+584700.89 & EXGAL   & 1578271735340707200 & 20.289 & 0.0183 & --                  & --     & --                \\
J124056.50+542045.24 & EXGAL   & 1570853334684204928 & 20.145 & 0.0095 & --                  & --     & --                \\
J124111.14+531723.58 & EXGAL   & 1570658167073814656 & 20.395 & 0.0404 & --                  & --     & --                \\
J124245.58+580559.42 & EXGAL   & 1578041215855692160 & 20.006 & 0.3112 & --                  & --     & --                \\
J124328.91+611938.14 & STAR    & 1580122419569004544 & 20.386 & 0.0078 & --                  & --     & --                \\
J124427.36+611838.64 & EXGAL   & 1580112111647483264 & 19.945 & 0.0149 & --                  & --     & --                \\
J124438.22+534355.25 & EXGAL   & 1570028941481593216 & 20.325 & 0.0155 & --                  & --     & --                \\
J124450.34+552014.47 & EXGAL   & 1571339520687552768 & 20.547 & 0.3308 & --                  & --     & --                \\
J124613.03+545330.99 & EXGAL   & 1570485719843552640 & 20.738 & 0.0227 & --                  & --     & --                \\
J124734.99+605639.15 & EXGAL   & 1579911313336208640 & 20.515 & 0.0312 & --                  & --     & --                \\
J124758.43+590124.37 & EXGAL   & 1578149689550119296 & 20.490 & 0.0135 & --                  & --     & --                \\
J124815.80+615944.89 & EXGAL   & 1580436123980165760 & 20.268 & 0.0593 & --                  & --     & --                \\
J124820.16+631002.10 & EXGAL   & 1676783063747035136 & 20.130 & 0.0058 & --                  & --     & --                \\
J125110.58+290630.27 & EXGAL   & 1464824920156463360 & 19.732 & 0.0352 & --                  & --     & --                \\
J125142.59+291221.22 & UNCLASS & 1464837457164974976 & 19.891 & 0.9655 & 1464837457164974976 & 19.837 & 0.9952            \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J125205.33+283426.56 & EXGAL   & 1464030007608944128 & 20.181 & 0.0091 & --                  & --     & --                \\
J125210.02+583146.24 & EXGAL   & 1577371578914865024 & 19.865 & 0.0158 & --                  & --     & --                \\
J125222.68+614812.76 & UNCLASS & 1580373864133805568 & 19.064 & 0.9963 & 1580373864133805568 & 19.025 & 0.9954            \\
J125243.77+240131.21 & STAR    & 3957589162403797504 & 19.905 & 0.1893 & --                  & --     & --                \\
J125251.69+272114.59 & EXGAL   & 3961706146255413632 & 20.352 & 0.0324 & --                  & --     & --                \\
J125328.18+272742.44 & EXGAL   & 3961731744260272000 & 20.368 & 0.0124 & --                  & --     & --                \\
J125344.98+303622.01 & UNCLASS & 1465075776310504704 & 20.402 & 0.1942 & --                  & --     & --                \\
J125352.74+291307.58 & STAR    & 1464181430975965440 & 19.761 & 0.2080 & --                  & --     & --                \\
J125359.85+262809.39 & STAR    & 3958517734333294592 & 19.413 & 0.0043 & --                  & --     & --                \\
J125409.21+252108.06 & STAR    & 3958196195901344512 & 18.968 & 0.0061 & --                  & --     & --                \\
J125433.71+272916.57 & EXGAL   & 3961687390133009536 & 20.436 & 0.0194 & --                  & --     & --                \\
J125435.11+252527.72 & EXGAL   & 3958202522388363008 & 20.443 & 0.0248 & --                  & --     & --                \\
J125511.00+252549.59 & EXGAL   & 3958200593948051840 & 20.011 & 0.0080 & --                  & --     & --                \\
J125545.61+303917.64 & UNCLASS & 1465440436214038272 & 20.510 & 0.3449 & --                  & --     & --                \\
J125554.51+274404.09 & EXGAL   & 1463700768300558720 & 20.399 & 0.0105 & --                  & --     & --                \\
J125559.63+270832.43 & STAR    & 3958661461118841856 & 19.975 & 0.0278 & --                  & --     & --                \\
J125629.80+281538.32 & EXGAL   & 1463789004108380288 & 20.011 & 0.0144 & --                  & --     & --                \\
J125630.28+231746.16 & EXGAL   & 3956646502981525248 & 20.365 & 0.0392 & --                  & --     & --                \\
J125650.56+283816.64 & EXGAL   & 1463903765634886912 & 20.127 & 0.0181 & --                  & --     & --                \\
J125715.84+310029.61 & EXGAL   & 1465475758024790272 & 20.463 & 0.1121 & --                  & --     & --                \\
J125719.09+294335.59 & EXGAL   & 1464210804256576512 & 20.059 & 0.0048 & --                  & --     & --                \\
J125735.38+295803.54 & UNCLASS & 1464593296864333312 & 20.326 & 0.0105 & --                  & --     & --                \\
J125806.38+240604.70 & sdX     & 3956898501598215808 & 19.224 & 0.7427 & --                  & --     & --                \\
J125815.86+281722.93 & EXGAL   & 1463833298107456896 & 20.260 & 0.0133 & --                  & --     & --                \\
J125824.38+294052.10 & EXGAL   & 1464538527441139328 & 20.373 & 0.0111 & --                  & --     & --                \\
J125843.13+235656.48 & STAR    & 3956881111275437184 & 19.573 & 0.0033 & --                  & --     & --                \\
J125851.32+255704.56 & sdX     & 3958324082847872000 & 19.949 & 0.8252 & 3958324082847872000 & 19.885 & 0.9608            \\
J125905.23+274739.40 & EXGAL   & 1460712196912120064 & 20.427 & 0.0165 & --                  & --     & --                \\
J125911.38+275603.56 & STAR    & 1460807918848407296 & 20.278 & 0.9906 & 1460807918848407296 & 20.217 & 0.9834            \\
J125918.00+263356.56 & EXGAL   & 1460384881749677696 & 20.110 & 0.0096 & --                  & --     & --                \\
J125927.16+284341.71 & EXGAL   & 1463918402883496192 & 20.322 & 0.0182 & --                  & --     & --                \\
J125927.26+271228.97 & EXGAL   & 1460630863116220416 & 20.041 & 0.0105 & --                  & --     & --                \\
J125944.77+314805.97 & EXGAL   & 1465620897855876736 & 20.298 & 0.0095 & --                  & --     & --                \\
J125949.99+273010.34 & STAR    & 1460688243879808256 & 19.871 & 0.0072 & --                  & --     & --                \\
J130001.13+294817.32 & EXGAL   & 1464555024411166336 & 20.523 & 0.0455 & --                  & --     & --                \\
J130007.32+233826.57 & EXGAL   & 3956670073762392320 & 19.467 & 0.0022 & --                  & --     & --                \\
J130029.81+230505.94 & STAR    & 3956589843773219968 & 19.797 & 0.0026 & --                  & --     & --                \\
J130106.06+250824.99 & EXGAL   & 3957476672916664320 & 20.551 & 0.0440 & --                  & --     & --                \\
J130112.10+275617.27 & EXGAL   & 1460795652421808512 & 20.364 & 0.0161 & --                  & --     & --                \\
J130124.12+270525.74 & STAR    & 1460429652488361088 & 19.991 & 0.1170 & --                  & --     & --                \\
J130145.07+321543.25 & EXGAL   & 1467158285693239424 & 20.493 & 0.0105 & --                  & --     & --                \\
J130156.48+313749.40 & EXGAL   & 1467054626658113920 & 20.517 & 0.0112 & --                  & --     & --                \\
J130213.09+245400.33 & EXGAL   & 3957410732282248192 & 20.363 & 0.0079 & --                  & --     & --                \\
J130227.09+242209.84 & EXGAL   & 3957097405828352128 & 20.349 & 0.4067 & --                  & --     & --                \\
J130231.42+282142.03 & EXGAL   & 1460835823252324736 & 19.643 & 0.0021 & --                  & --     & --                \\
J130259.50+260046.52 & STAR    & 1459545885657901952 & 19.988 & 0.3261 & --                  & --     & --                \\
J130307.11+281808.15 & EXGAL   & 1460831901946381184 & 20.310 & 0.0100 & --                  & --     & --                \\
J130313.37+315730.69 & EXGAL   & 1467089669296194048 & 19.728 & 0.0021 & --                  & --     & --                \\
J130314.59+282635.10 & EXGAL   & 1461209103153689216 & 20.676 & 0.0716 & --                  & --     & --                \\
J130421.21+271640.97 & EXGAL   & 1460515173877469824 & 19.797 & 0.0282 & --                  & --     & --                \\
J130430.10+332157.08 & EXGAL   & 1467325720698576384 & 20.384 & 0.0175 & --                  & --     & --                \\
J130453.54+333004.44 & STAR    & 1467704094433360000 & 19.442 & 0.0150 & --                  & --     & --                \\
J130506.58+312221.71 & EXGAL   & 1466261152924833664 & 19.870 & 0.0095 & --                  & --     & --                \\
J130511.29+274452.28 & EXGAL   & 1460567228881460480 & 19.892 & 0.0026 & --                  & --     & --                \\
J130525.35+282735.15 & STAR    & 1461177629632864256 & 19.660 & 0.2634 & --                  & --     & --                \\
J130631.89+173925.20 & STAR    & 3937922064774476928 & 19.980 & 0.0045 & --                  & --     & --                \\
J130632.00+272216.12 & STAR    & 1460484971667728128 & 19.846 & 0.7581 & 1460484971667728128 & 19.795 & 0.8402            \\
J130636.42+312025.58 & EXGAL   & 1466248753355506560 & 19.833 & 0.0033 & --                  & --     & --                \\
J130725.95+173304.26 & STAR    & 3937869936755899648 & 20.058 & 0.0168 & --                  & --     & --                \\
J130751.98+244707.93 & EXGAL   & 1459169371644630656 & 20.233 & 0.0212 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J130807.04+331929.39 & STAR    & 1467639803066586368 & 19.796 & 0.3522 & --                  & --     & --                \\
J130848.80+000559.25 & EXGAL   & 3687702351055605376 & 19.837 & 0.0055 & --                  & --     & --                \\
J130945.57-002135.10 & STAR    & 3687622292864704512 & 19.110 & 0.0023 & --                  & --     & --                \\
J131009.28+273235.74 & EXGAL   & 1460124366213288832 & 20.017 & 0.0069 & --                  & --     & --                \\
J131027.50+184042.59 & EXGAL   & 3938111210838762624 & 20.292 & 0.0447 & --                  & --     & --                \\
J131034.19+004205.65 & STAR    & 3690843106019949952 & 19.469 & 0.0021 & --                  & --     & --                \\
J131035.45+071920.26 & EXGAL   & 3729933905483480448 & 19.916 & 0.0142 & --                  & --     & --                \\
J131107.83+065541.94 & EXGAL   & 3729840554369055232 & 19.701 & 0.0052 & --                  & --     & --                \\
J131155.60+063511.80 & STAR    & 3729628520424231680 & 19.160 & 0.0032 & --                  & --     & --                \\
J131155.77-012557.38 & EXGAL   & 3685809851025632256 & 19.761 & 0.0183 & --                  & --     & --                \\
J131212.75+170110.68 & STAR    & 3937042245018401920 & 20.187 & 0.0105 & --                  & --     & --                \\
J131223.93+181053.00 & STAR    & 3938021703720018304 & 19.687 & 0.0045 & --                  & --     & --                \\
J131244.83+181208.82 & STAR    & 3938022360852519680 & 17.021 & 0.0907 & --                  & --     & --                \\
J131245.25+180919.88 & STAR    & 3938021948533370880 & 19.991 & 0.1473 & --                  & --     & --                \\
J131245.91+180532.93 & STAR    & 3937269534687324672 & 19.630 & 0.0013 & --                  & --     & --                \\
J131255.23+180610.01 & STAR    & 3937270874717137792 & 19.230 & 0.0044 & --                  & --     & --                \\
J131257.89+180531.60 & STAR    & 3937270118802875904 & 19.105 & 0.0067 & --                  & --     & --                \\
J131303.14+181346.47 & STAR    & 3939523842762282752 & 19.767 & 0.0058 & --                  & --     & --                \\
J131311.15+180712.50 & STAR    & 3937270604134437760 & 19.459 & 0.0023 & --                  & --     & --                \\
J131317.71+181910.76 & STAR    & 3939524839194747904 & 19.811 & 0.0039 & --                  & --     & --                \\
J131359.34+192519.00 & EXGAL   & 3939753537613041792 & 19.647 & 0.0029 & --                  & --     & --                \\
J131534.10+001824.45 & STAR    & 3687589925991536000 & 19.073 & 0.0060 & --                  & --     & --                \\
J131557.31-000805.60 & STAR    & 3687495917746939776 & 19.020 & 0.0079 & --                  & --     & --                \\
J131606.11+173658.77 & STAR    & 3938491852316051456 & 19.673 & 0.0026 & --                  & --     & --                \\
J131620.06+174031.97 & STAR    & 3938681586790399616 & 19.722 & 0.0076 & --                  & --     & --                \\
J131645.00+173811.52 & STAR    & 3938492672654573056 & 20.203 & 0.0212 & --                  & --     & --                \\
J131733.12+195032.90 & EXGAL   & 3940157676855671168 & 20.029 & 0.0187 & --                  & --     & --                \\
J131848.20+183957.02 & UNCLASS & 3938848575118846720 & 19.897 & 0.9500 & 3938848575119939840 & 19.849 & 0.9871            \\
J131900.79+165107.68 & EXGAL   & 3744738520313481600 & 20.499 & 0.0288 & --                  & --     & --                \\
J132318.10+034605.19 & UNCLASS & 3715676160249364096 & 19.893 & 0.2851 & 3715676160249364096 & 19.854 & 0.0993            \\
J132332.96+184313.88 & EXGAL   & 3939040336819619840 & 20.361 & 0.0142 & --                  & --     & --                \\
J132518.07+202710.15 & EXGAL   & 3939501508932592896 & 20.462 & 0.0198 & --                  & --     & --                \\
J132535.88+810929.16 & UNCLASS & 1719016198723069568 & 19.548 & 0.9895 & 1719016198723069568 & 19.521 & 0.9931            \\
J132616.99+045240.65 & STAR    & 3716260726772996736 & 19.801 & 0.3562 & --                  & --     & --                \\
J132727.76+061129.47 & STAR    & 3718115804752527872 & 19.390 & 0.0389 & --                  & --     & --                \\
J132920.74+323157.68 & STAR    & 1468726326713303296 & 19.876 & 0.0036 & --                  & --     & --                \\
J132920.91+320838.63 & EXGAL   & 1468681697710767616 & 20.448 & 0.1565 & --                  & --     & --                \\
J132957.04+052902.83 & STAR    & 3717829004016050304 & 19.825 & 0.3731 & --                  & --     & --                \\
J133214.18+024840.23 & STAR    & 3711948029852026112 & 19.950 & 0.3777 & --                  & --     & --                \\
J133257.74+335117.80 & STAR    & 1470017462602179968 & 19.702 & 0.1432 & --                  & --     & --                \\
J133331.46+321005.16 & EXGAL   & 1468831501876592128 & 20.436 & 0.2108 & --                  & --     & --                \\
J133413.16+313929.60 & STAR    & 1468384039297201792 & 20.148 & 0.0411 & --                  & --     & --                \\
J133501.97+033934.99 & STAR    & 3712847116830521472 & 19.817 & 0.0226 & --                  & --     & --                \\
J133656.36+800943.41 & UNCLASS & 1718710568850372864 & 18.751 & 0.9983 & 1718710568850372864 & 18.711 & 0.9950            \\
J133800.72+313012.49 & EXGAL   & 1456743230521885184 & 20.604 & 0.0133 & --                  & --     & --                \\
J133813.65+323203.11 & EXGAL   & 1468904962992983168 & 20.293 & 0.0080 & --                  & --     & --                \\
J133933.41+315721.45 & STAR    & 1456850364182697088 & 19.888 & 0.0053 & 1456850364182697088 & 19.852 & 0.0544            \\
J134308.01+812448.67 & UNCLASS & 1718939095470066688 & 19.737 & 0.9751 & 1718939095470066688 & 19.686 & 0.9793            \\
J134447.14+810619.08 & UNCLASS & 1718861098863847168 & 18.847 & 0.9991 & 1718861098863847168 & 18.811 & 0.9983            \\
J134628.74+710619.17 & UNCLASS & 1686806967659895296 & 19.422 & 0.9778 & 1686806967659895296 & 19.378 & 0.9843            \\
J134741.97+810415.83 & UNCLASS & 1718857456731568128 & 19.411 & 0.9947 & 1718857456731568128 & 19.372 & 0.9952            \\
J135126.40+700535.84 & EXGAL   & 1674716119325832832 & 19.907 & 0.0051 & --                  & --     & --                \\
J135355.66+052431.79 & STAR    & 3720034967938491648 & 18.997 & 0.0129 & --                  & --     & --                \\
J135556.22+054137.88 & STAR    & 3720128018405519104 & 18.533 & 0.3490 & --                  & --     & --                \\
J135703.25+041655.78 & STAR    & 3671658655340045312 & 19.984 & 0.3206 & --                  & --     & --                \\
J135708.33+042335.34 & STAR    & 3671684115906265600 & 19.509 & 0.0105 & --                  & --     & --                \\
J135718.51+041804.41 & STAR    & 3671647385345877632 & 19.991 & 0.3788 & --                  & --     & --                \\
J135738.59+060234.84 & STAR    & 3720165191347510272 & 19.969 & 0.4582 & --                  & --     & --                \\
J135815.15+060916.31 & EXGAL   & 3720540021732834176 & 19.259 & 0.0039 & --                  & --     & --                \\
J135910.18+783736.40 & UNCLASS & 1715011502496355840 & 19.811 & 0.9878 & 1715011502496355840 & 19.774 & 0.9941            \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J135940.12+041350.01 & STAR    & 3671621787340729216 & 18.177 & 0.0021 & --                  & --     & --                \\
J135950.27+040229.75 & EXGAL   & 3671598701891789056 & 20.217 & 0.2793 & --                  & --     & --                \\
J140033.11+031827.25 & STAR    & 3670736680479974912 & 19.888 & 0.3211 & --                  & --     & --                \\
J140056.87+050914.83 & STAR    & 3671833168451171200 & 19.001 & 0.0100 & 3671833168451171200 & 18.968 & 0.2338            \\
J140132.58+055243.66 & EXGAL   & 3672457175659383808 & 19.450 & 0.0179 & --                  & --     & --                \\
J140208.04+032410.45 & EXGAL   & 3670754925501085312 & 19.733 & 0.0467 & --                  & --     & --                \\
J140229.69+790515.47 & UNCLASS & 1715403551406505344 & 19.181 & 0.8576 & 1715403551406505344 & 19.149 & 0.9809            \\
J140231.04+052855.36 & EXGAL   & 3672220368342955264 & 19.994 & 0.0066 & --                  & --     & --                \\
J140235.61+062145.54 & STAR    & 3672615917651101952 & 18.903 & 0.0033 & 3672615917651101952 & 18.874 & 0.3500            \\
J140244.37+230154.96 & EXGAL   & 1256633694811096832 & 19.914 & 0.0235 & --                  & --     & --                \\
J140252.04+033827.38 & EXGAL   & 3670766951409636224 & 19.538 & 0.0269 & --                  & --     & --                \\
J140315.22+241746.36 & STAR    & 1257053158497223296 & 19.839 & 0.4845 & --                  & --     & --                \\
J140347.56+034218.86 & EXGAL   & 3670858004716265472 & 20.167 & 0.0117 & --                  & --     & --                \\
J140355.57+043941.10 & EXGAL   & 3670991668394100096 & 18.546 & 0.0011 & --                  & --     & --                \\
J140408.95+034413.46 & UNCLASS & 3670859001148683264 & 19.749 & 0.3112 & --                  & --     & --                \\
J140415.85+784215.26 & UNCLASS & 1715007624141215360 & 19.014 & 0.9855 & 1715007624141215360 & 18.974 & 0.9911            \\
J140419.74+705224.61 & sdX     & 1675104319945152640 & 16.870 & 0.9478 & 1675104319945152640 & 16.840 & 0.9822            \\
J140508.88+044430.98 & STAR    & 3671357045556481152 & 19.181 & 0.0154 & --                  & --     & --                \\
J140517.29+050900.21 & STAR    & 3672158589532816896 & 18.768 & 0.1266 & 3672158589532816896 & 18.761 & 0.0979            \\
J140525.35+060048.70 & EXGAL   & 3672348770684974848 & 19.189 & 0.0529 & --                  & --     & --                \\
J140704.09-010635.34 & STAR    & 3659376324478397184 & 17.628 & 0.0121 & --                  & --     & --                \\
J140724.75+004641.83 & STAR    & 3661013252481137152 & 19.767 & 0.2429 & 3661013256774699392 & 19.723 & 0.8652            \\
J140755.92+000747.63 & STAR    & 3660082825124230784 & 18.979 & 0.0881 & --                  & --     & --                \\
J140826.75-003051.72 & STAR    & 3659824886568655488 & 19.227 & 0.0122 & --                  & --     & --                \\
J140933.37+812230.31 & UNCLASS & 1721881972701637248 & 19.391 & 0.9948 & 1721881972701637248 & 19.360 & 0.9908            \\
J140935.36+005611.96 & EXGAL   & 3660280599778702464 & 20.185 & 0.0180 & --                  & --     & --                \\
J140954.45-000720.14 & STAR    & 3659872852762730112 & 19.708 & 0.0328 & --                  & --     & --                \\
J141012.64+000624.14 & STAR    & 3659974768041996288 & 19.555 & 0.2121 & 3659974768041996288 & 19.525 & 0.0203            \\
J141020.45-003245.09 & STAR    & 3659794649998073728 & 19.657 & 0.0172 & --                  & --     & --                \\
J141021.86+010644.78 & EXGAL   & 3666300219781445248 & 19.872 & 0.0067 & --                  & --     & --                \\
J141028.47+005323.72 & STAR    & 3660277301243052928 & 19.838 & 0.0076 & 3660277301243052928 & 19.799 & 0.1091            \\
J141035.10+001248.58 & STAR    & 3659982941364984448 & 18.953 & 0.0048 & --                  & --     & --                \\
J141108.98+010745.65 & UNCLASS & 3666295134540172160 & 19.888 & 0.9941 & 3666295134540172160 & 19.840 & 0.9865            \\
J141204.15+795405.70 & UNCLASS & 1715550748526849792 & 18.404 & 0.9898 & 1715550748526849792 & 18.375 & 0.9960            \\
J141208.20-001217.44 & EXGAL   & 3659906495242005760 & 20.222 & 0.0189 & --                  & --     & --                \\
J141222.44+784443.82 & UNCLASS & 1715336305103347840 & 19.930 & 0.9989 & 1715336305103347840 & 19.873 & 0.9895            \\
J141225.91-001825.33 & STAR    & 3659892820066023808 & 19.159 & 0.0115 & --                  & --     & --                \\
J141238.49-014937.99 & EXGAL   & 3647445278992771456 & 20.179 & 0.0083 & --                  & --     & --                \\
J141323.87-005604.48 & STAR    & 3647750947520344704 & 19.354 & 0.0092 & --                  & --     & --                \\
J141326.74+001812.73 & STAR    & 3659995688827980032 & 19.435 & 0.0052 & --                  & --     & --                \\
J141327.47+523851.79 & EXGAL   & 1608099669032672256 & 20.293 & 0.0053 & --                  & --     & --                \\
J141347.49+000228.03 & STAR    & 3659928756057403264 & 19.961 & 0.0354 & --                  & --     & --                \\
J141407.97+003327.92 & STAR    & 3666011254382148096 & 19.099 & 0.0060 & --                  & --     & --                \\
J141409.58+321133.51 & EXGAL   & 1477690198338347264 & 20.368 & 0.3582 & --                  & --     & --                \\
J141409.86+520137.16 & EXGAL   & 1607878873354077568 & 19.914 & 0.0100 & --                  & --     & --                \\
J141506.61+804505.52 & UNCLASS & 1721800711920129408 & 19.741 & 0.9964 & 1721800711920129408 & 19.703 & 0.9944            \\
J141556.68-005814.84 & sdX     & 3647784512689022336 & 18.593 & 0.4385 & --                  & --     & --                \\
J141604.98+002236.52 & EXGAL   & 3665966728456461568 & 20.115 & 0.0106 & --                  & --     & --                \\
J141653.02+312656.08 & STAR    & 1477408345404062080 & 19.880 & 0.1787 & --                  & --     & --                \\
J141728.43-000805.11 & EXGAL   & 3653859108274227840 & 19.478 & 0.0045 & --                  & --     & --                \\
J141910.09-011428.85 & UNCLASS & 3647537191292748672 & 19.915 & 0.3223 & --                  & --     & --                \\
J141923.78+310754.42 & EXGAL   & 1477357561710962560 & 19.729 & 0.0064 & --                  & --     & --                \\
J141954.33-012014.44 & EXGAL   & 3647537470465882368 & 20.236 & 0.0396 & --                  & --     & --                \\
J142027.40-013613.98 & STAR    & 3646761554558561792 & 20.261 & 0.0259 & --                  & --     & --                \\
J142035.91-002932.33 & STAR    & 3653652503168004352 & 19.448 & 0.0189 & --                  & --     & --                \\
J142038.34+513714.92 & EXGAL   & 1604814122130615680 & 20.671 & 0.0289 & --                  & --     & --                \\
J142111.13-010353.51 & STAR    & 3653547980843699456 & 19.194 & 0.0144 & --                  & --     & --                \\
J142139.97-005148.43 & EXGAL   & 3653557945167391232 & 19.333 & 0.0077 & --                  & --     & --                \\
J142215.28-005420.45 & EXGAL   & 3652829449994496128 & 19.561 & 0.0199 & --                  & --     & --                \\
J142222.41+323852.42 & EXGAL   & 1477958685333750016 & 20.519 & 0.0145 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J142256.30-001356.60 & STAR    & 3653710777283678080 & 19.662 & 0.1508 & --                  & --     & --                \\
J142326.27+521752.91 & EXGAL   & 1604953858889789824 & 19.895 & 0.0053 & --                  & --     & --                \\
J142338.61+343136.66 & EXGAL   & 1479827099186802432 & 20.582 & 0.0114 & --                  & --     & --                \\
J142349.06+334857.07 & UNCLASS & 1479727249786784384 & 19.640 & 0.8615 & 1479727249786784384 & 19.604 & 0.8946            \\
J142415.65+000000.55 & STAR    & 3653742319523968512 & 19.903 & 0.3988 & --                  & --     & --                \\
J142443.52+333010.11 & EXGAL   & 1479523393459167744 & 20.260 & 0.0113 & --                  & --     & --                \\
J142445.78+342945.17 & EXGAL   & 1479783359239430272 & 20.618 & 0.0199 & --                  & --     & --                \\
J142508.87-014502.00 & STAR    & 3652504819187030784 & 19.954 & 0.3164 & --                  & --     & --                \\
J142532.62+315813.18 & EXGAL   & 1285716533280417536 & 20.073 & 0.0133 & --                  & --     & --                \\
J142550.32+335618.79 & EXGAL   & 1479559952221930880 & 20.161 & 0.0459 & --                  & --     & --                \\
J142610.76+341738.84 & EXGAL   & 1479855171093066752 & 20.490 & 0.0133 & --                  & --     & --                \\
J142614.46+024327.30 & STAR    & 3668208594010490368 & 19.845 & 0.0111 & --                  & --     & --                \\
J142654.90-021157.87 & STAR    & 3652428403128330240 & 19.496 & 0.0239 & --                  & --     & --                \\
J142702.70-001344.94 & EXGAL   & 3652963281175658112 & 20.094 & 0.0350 & --                  & --     & --                \\
J142729.04+000142.05 & EXGAL   & 3653354947833547392 & 20.267 & 0.0423 & --                  & --     & --                \\
J142741.21+332937.27 & EXGAL   & 1479476354977448064 & 20.001 & 0.0060 & --                  & --     & --                \\
J142802.59+013713.66 & STAR    & 3654568194490481536 & 19.237 & 0.0107 & --                  & --     & --                \\
J142810.54+515945.47 & STAR    & 1604688670429400320 & 18.811 & 0.2079 & --                  & --     & --                \\
J142817.90+032407.51 & UNCLASS & 3668348781742691328 & 17.296 & 0.9991 & 3668348781742691328 & 17.266 & 0.9978            \\
J142824.85+541639.12 & EXGAL   & 1608531605302280960 & 20.231 & 0.0127 & --                  & --     & --                \\
J142842.98+001737.50 & STAR    & 3653389582450014592 & 19.053 & 0.0046 & --                  & --     & --                \\
J142850.06+331748.23 & EXGAL   & 1287321648458307584 & 20.113 & 0.0035 & --                  & --     & --                \\
J142852.65+335148.26 & EXGAL   & 1479593659124115456 & 20.318 & 0.0206 & --                  & --     & --                \\
J142907.79-010038.14 & STAR    & 3652672391630956032 & 19.634 & 0.1981 & 3652672391630956032 & 19.591 & 0.6260            \\
J142925.77-002626.77 & STAR    & 3653267571018334336 & 19.668 & 0.0983 & --                  & --     & --                \\
J142951.32+024747.57 & STAR    & 3656201205481293952 & 19.721 & 0.5645 & --                  & --     & --                \\
J143012.21+334232.41 & EXGAL   & 1287427893067195136 & 20.380 & 0.0105 & --                  & --     & --                \\
J143012.74+331905.61 & EXGAL   & 1287401401706884096 & 20.246 & 0.0140 & --                  & --     & --                \\
J143041.52+014711.61 & STAR    & 3655881870367465984 & 19.177 & 0.0975 & --                  & --     & --                \\
J143041.82+015221.25 & EXGAL   & 3655894514751198848 & 19.458 & 0.0081 & --                  & --     & --                \\
J143052.23-005003.28 & STAR    & 3653006338223085056 & 19.385 & 0.0171 & --                  & --     & --                \\
J143103.70+142852.38 & STAR    & 1228124462110099712 & 19.830 & 0.5123 & --                  & --     & --                \\
J143136.23+024435.12 & EXGAL   & 3656241097136560768 & 19.886 & 0.0265 & --                  & --     & --                \\
J143136.90+140827.50 & EXGAL   & 1227919437551402240 & 19.754 & 0.0708 & --                  & --     & --                \\
J143150.78+514947.86 & EXGAL   & 1605001825084608000 & 20.517 & 0.0126 & --                  & --     & --                \\
J143153.98+530034.15 & EXGAL   & 1605401394483971840 & 20.299 & 0.0122 & --                  & --     & --                \\
J143157.11+352800.03 & STAR    & 1480129258726068864 & 19.131 & 0.0166 & --                  & --     & --                \\
J143212.60+355027.14 & EXGAL   & 1480420251349953920 & 20.544 & 0.1157 & 1480420251349953920 & 20.533 & 0.8564            \\
J143226.66+005055.82 & STAR    & 3653520428628751744 & 19.466 & 0.0041 & --                  & --     & --                \\
J143233.19+153227.63 & STAR    & 1228339137460246016 & 19.484 & 0.1163 & --                  & --     & --                \\
J143258.00+011857.40 & sdX     & 3655054139974647424 & 17.960 & 0.2404 & 3655054139974647424 & 17.925 & 0.1198            \\
J143259.51+034553.31 & EXGAL   & 3656744364225116032 & 20.042 & 0.0527 & --                  & --     & --                \\
J143310.18+351405.91 & EXGAL   & 1480064937298147456 & 20.625 & 0.0216 & --                  & --     & --                \\
J143314.75+530935.75 & sdX     & 1605239049014274560 & 17.143 & 0.1140 & 1605239049014274560 & 17.120 & 0.0640            \\
J143321.36+155828.09 & STAR    & 1234372913675731328 & 19.800 & 0.2591 & --                  & --     & --                \\
J143328.94+030304.41 & EXGAL   & 3656281435469700864 & 19.741 & 0.7472 & --                  & --     & --                \\
J143332.09+135345.43 & STAR    & 1227844151068897024 & 19.870 & 0.3492 & --                  & --     & --                \\
J143334.29+031059.34 & EXGAL   & 3656285008882976256 & 20.280 & 0.0123 & --                  & --     & --                \\
J143341.60+332412.86 & EXGAL   & 1287365285325723648 & 20.308 & 0.0071 & --                  & --     & --                \\
J143347.43+030512.29 & EXGAL   & 3656271402426766848 & 19.886 & 0.0084 & --                  & --     & --                \\
J143348.77+022422.33 & STAR    & 3656022294322787456 & 19.078 & 0.5402 & --                  & --     & --                \\
J143358.52+003009.40 & UNCLASS & 3653448926013159040 & 19.685 & 0.2502 & --                  & --     & --                \\
J143404.07+024208.00 & sdX     & 3656064556800894464 & 16.848 & 0.2217 & 3656064556800894464 & 16.823 & 0.0510            \\
J143415.09+334132.54 & STAR    & 1287753756527709696 & 20.408 & 0.8947 & 1287753756527709696 & 20.339 & 0.9935            \\
J143421.13-011226.39 & EXGAL   & 3649967902264106112 & 20.017 & 0.0159 & --                  & --     & --                \\
J143422.61+145110.49 & EXGAL   & 1228062094889783296 & 19.665 & 0.0088 & --                  & --     & --                \\
J143426.88+641739.73 & EXGAL   & 1668866000207320704 & 19.978 & 0.0133 & --                  & --     & --                \\
J143429.80-001746.28 & sdX     & 3653143635442071040 & 18.752 & 0.8081 & 3653143635442071040 & 18.711 & 0.6058            \\
J143448.08-010224.08 & STAR    & 3649995183896392704 & 19.767 & 0.1407 & --                  & --     & --                \\
J143450.30+024705.01 & EXGAL   & 3656070707194647552 & 20.042 & 0.0101 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J143452.74-002828.06 & EXGAL   & 3653126283774153984 & 18.802 & 0.0020 & --                  & --     & --                \\
J143458.69-011413.87 & STAR    & 3649943472490329472 & 19.505 & 0.0118 & --                  & --     & --                \\
J143507.14-005604.00 & STAR    & 3650004907702719872 & 19.126 & 0.0117 & --                  & --     & --                \\
J143523.29-004345.90 & STAR    & 3650114721426027392 & 19.855 & 0.5058 & 3650114721426027392 & 19.816 & 0.0422            \\
J143524.91+025911.94 & EXGAL   & 3656451550534331520 & 19.756 & 0.0045 & --                  & --     & --                \\
J143526.58+350037.34 & EXGAL   & 1287983554458266368 & 20.473 & 0.0218 & --                  & --     & --                \\
J143533.15-004959.42 & STAR    & 3650007622122080896 & 19.616 & 0.4593 & 3650007622122080896 & 19.574 & 0.1638            \\
J143534.09+020334.73 & EXGAL   & 3655949829634750208 & 19.966 & 0.0098 & --                  & --     & --                \\
J143543.89-012434.22 & STAR    & 3649925605426265600 & 19.944 & 0.5910 & --                  & --     & --                \\
J143546.37-000903.54 & EXGAL   & 3653163461011392128 & 19.958 & 0.0091 & --                  & --     & --                \\
J143555.16+004614.88 & STAR    & 3654773317833512576 & 19.120 & 0.1464 & --                  & --     & --                \\
J143632.87+013812.53 & sdX     & 3655166702478073472 & 18.365 & 0.4798 & 3655166702478073472 & 18.324 & 0.2143            \\
J143639.91-014214.45 & STAR    & 3649691856126331392 & 19.753 & 0.2404 & --                  & --     & --                \\
J143709.92+143046.97 & STAR    & 1227982620815199872 & 19.548 & 0.2693 & --                  & --     & --                \\
J143716.72+151756.69 & STAR    & 1234099616317176576 & 19.706 & 0.3764 & 1234099616317176576 & 19.670 & 0.0193            \\
J143726.25+142332.82 & STAR    & 1179942140298902656 & 19.884 & 0.0147 & --                  & --     & --                \\
J143741.35+531453.23 & EXGAL   & 1606681019859190656 & 20.580 & 0.0490 & --                  & --     & --                \\
J143813.65+134828.17 & STAR    & 1179856825070355072 & 19.853 & 0.2466 & --                  & --     & --                \\
J143828.80+003630.05 & EXGAL   & 3654727413222523648 & 20.168 & 0.0233 & --                  & --     & --                \\
J143854.45+341258.79 & EXGAL   & 1287686411440530176 & 19.924 & 0.0045 & --                  & --     & --                \\
J143908.77-010747.07 & EXGAL   & 3649842729736818944 & 20.432 & 0.0172 & --                  & --     & --                \\
J143943.63+142546.14 & STAR    & 1185935028426097792 & 19.413 & 0.3797 & --                  & --     & --                \\
J143949.27+135652.06 & STAR    & 1179853904490938880 & 19.953 & 0.2453 & --                  & --     & --                \\
J144001.76-014959.41 & EXGAL   & 3649650864957786240 & 20.502 & 0.1482 & --                  & --     & --                \\
J144023.58+135454.66 & STAR    & 1185854317400389120 & 18.333 & 0.4181 & --                  & --     & --                \\
J144048.22-015301.69 & STAR    & 3648989989750045568 & 19.011 & 0.0143 & --                  & --     & --                \\
J144056.66+002208.78 & STAR    & 3651697056097863040 & 19.924 & 0.3489 & --                  & --     & --                \\
J144115.95+002704.39 & STAR    & 3651791717176233600 & 19.563 & 0.3420 & --                  & --     & --                \\
J144119.67+001234.79 & EXGAL   & 3651642973869561984 & 19.614 & 0.0134 & --                  & --     & --                \\
J144132.53-020705.76 & STAR    & 3648877221089005952 & 19.252 & 0.0023 & --                  & --     & --                \\
J144404.65-014441.20 & EXGAL   & 3648957863395348608 & 20.136 & 0.0618 & --                  & --     & --                \\
J144412.85-002400.32 & STAR    & 3651361430172969856 & 19.956 & 0.6142 & --                  & --     & --                \\
J144433.73-005346.95 & STAR    & 3650577959418538240 & 19.486 & 0.5335 & 3650577959418538240 & 19.457 & 0.0296            \\
J144542.95-002339.08 & STAR    & 3651441900679918720 & 19.499 & 0.1768 & --                  & --     & --                \\
J145031.27+661023.32 & EXGAL   & 1669268421462988928 & 20.585 & 0.0103 & --                  & --     & --                \\
J145359.43+650915.71 & EXGAL   & 1621125991307354880 & 20.401 & 0.0045 & --                  & --     & --                \\
J145404.39+505448.64 & EXGAL   & 1593269520620432512 & 19.856 & 0.0073 & --                  & --     & --                \\
J145420.12+522315.67 & EXGAL   & 1593687369398705408 & 20.446 & 0.0128 & --                  & --     & --                \\
J145422.36+344731.13 & EXGAL   & 1293129028358003456 & 20.291 & 0.0066 & --                  & --     & --                \\
J145630.95-080141.45 & UNCLASS & 6332472744403469056 & 19.753 & 0.0059 & --                  & --     & --                \\
J145655.47+324257.23 & EXGAL   & 1289330593640908928 & 20.413 & 0.0091 & --                  & --     & --                \\
J145848.85+323619.42 & EXGAL   & 1289334648093942912 & 20.543 & 0.0215 & --                  & --     & --                \\
J145957.33+510949.22 & STAR    & 1592584490515955968 & 19.765 & 0.9971 & 1592584490515955968 & 19.730 & 0.9983            \\
J150006.70+684112.23 & EXGAL   & 1693834290070765440 & 19.965 & 0.1574 & --                  & --     & --                \\
J150008.19-072826.16 & UNCLASS & 6332603444553282176 & 19.791 & 0.6969 & --                  & --     & --                \\
J150045.78+311155.62 & EXGAL   & 1288246372096861696 & 20.224 & 0.0064 & --                  & --     & --                \\
J150137.80+514918.48 & STAR    & 1593751587749299072 & 20.544 & 0.3326 & --                  & --     & --                \\
J150235.78-065511.49 & UNCLASS & 6333031021432605696 & 19.626 & 0.0619 & --                  & --     & --                \\
J150533.95+314838.09 & STAR    & 1288619312696849536 & 18.496 & 0.0945 & 1288619312696849536 & 18.467 & 0.1392            \\
J150627.19+325756.12 & EXGAL   & 1288835748986099072 & 19.859 & 0.0141 & --                  & --     & --                \\
J150921.24+320040.92 & EXGAL   & 1276718473716164096 & 20.605 & 0.0113 & --                  & --     & --                \\
J150933.18+685039.41 & STAR    & 1694015262812672128 & 19.167 & 0.0013 & --                  & --     & --                \\
J151020.73+162631.54 & EXGAL   & 1184393345620740352 & 19.926 & 0.0070 & --                  & --     & --                \\
J151051.51+323143.84 & STAR    & 1276760220798496896 & 19.330 & 0.7238 & 1276760220798496896 & 19.300 & 0.7479            \\
J151326.43+743121.24 & STAR    & 1700749737172642176 & 19.599 & 0.0092 & --                  & --     & --                \\
J151419.33+171148.03 & EXGAL   & 1208485015478952832 & 20.540 & 0.1120 & --                  & --     & --                \\
J151608.85+183857.41 & EXGAL   & 1212057500557145216 & 20.449 & 0.0156 & --                  & --     & --                \\
J151703.46+035757.35 & EXGAL   & 1155763604725892992 & 19.947 & 0.0062 & --                  & --     & --                \\
J151801.94+020432.59 & STAR    & 4421526311334667776 & 19.759 & 0.2878 & --                  & --     & --                \\
J151803.29+012914.63 & EXGAL   & 4421420788282102784 & 19.880 & 0.0062 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J151809.94+020500.79 & STAR    & 4421526169599105536 & 18.686 & 0.2952 & 4421526169599105536 & 18.803 & 0.0459            \\
J151823.40+020853.65 & STAR    & 4421620663176597888 & 19.878 & 0.2731 & --                  & --     & --                \\
J151836.32+021649.37 & STAR    & 4421624197934593536 & 19.663 & 0.1682 & 4421624197934593536 & 19.600 & 0.0400            \\
J151839.75+015938.62 & STAR    & 4421474801790134656 & 19.012 & 0.5013 & 4421474801790134656 & 19.030 & 0.0428            \\
J151854.31+020343.05 & STAR    & 4421569295365031168 & 19.604 & 0.4724 & 4421569295365031168 & 19.561 & 0.1048            \\
J151903.95+015952.29 & STAR    & 4421568088480330624 & 19.834 & 0.2019 & --                  & --     & --                \\
J152225.90+022633.76 & EXGAL   & 4421972365160776192 & 19.716 & 0.0114 & --                  & --     & --                \\
J153503.87+324749.17 & EXGAL   & 1370592577472233344 & 20.227 & 0.0055 & --                  & --     & --                \\
J153707.72+434351.52 & sdX     & 1391314763883537280 & 17.984 & 0.1902 & 1391314763883537280 & 17.949 & 0.0582            \\
J153816.74+434617.88 & EXGAL   & 1391309197609663872 & 19.916 & 0.0027 & --                  & --     & --                \\
J154048.63+435851.35 & EXGAL   & 1397273017394103552 & 20.141 & 0.0712 & --                  & --     & --                \\
J154247.00+444614.82 & EXGAL   & 1397458422542460544 & 20.348 & 0.0475 & --                  & --     & --                \\
J154316.33+421851.48 & EXGAL   & 1390186394370459264 & 20.471 & 0.0118 & --                  & --     & --                \\
J154401.95+755659.98 & STAR    & 1706909338750225152 & 18.893 & 0.1073 & --                  & --     & --                \\
J154402.53+415324.11 & EXGAL   & 1390114646941897472 & 20.357 & 0.0045 & --                  & --     & --                \\
J154645.64+422955.44 & sdX     & 1396159040316943488 & 19.619 & 0.6661 & --                  & --     & --                \\
J154720.32+425736.47 & EXGAL   & 1396186047070655744 & 20.172 & 0.0055 & --                  & --     & --                \\
J154826.41+431824.30 & EXGAL   & 1396337023761451648 & 20.213 & 0.0070 & --                  & --     & --                \\
J154828.43+443059.97 & EXGAL   & 1396653408232623872 & 20.147 & 0.0285 & --                  & --     & --                \\
J155231.80+440213.07 & EXGAL   & 1396711338751405056 & 20.284 & 0.0323 & --                  & --     & --                \\
J155800.15+143629.05 & STAR    & 1192145894733450240 & 20.154 & 0.0101 & --                  & --     & --                \\
J155824.75+430407.41 & STAR    & 1384415294059868544 & 19.293 & 0.1696 & 1384415294059868544 & 19.252 & 0.4481            \\
J155940.14+160913.08 & EXGAL   & 1193154662292858880 & 20.186 & 0.0073 & --                  & --     & --                \\
J155940.47+542622.23 & EXGAL   & 1597281058729127936 & 20.218 & 0.0094 & --                  & --     & --                \\
J155947.43+444740.85 & EXGAL   & 1384851731456806784 & 20.272 & 0.0109 & --                  & --     & --                \\
J160019.63+441950.32 & EXGAL   & 1384782157280990976 & 20.580 & 0.0143 & --                  & --     & --                \\
J160037.57+415510.66 & STAR    & 1383512732452176896 & 18.990 & 0.0043 & --                  & --     & --                \\
J160049.05+552622.68 & EXGAL   & 1621420969661660416 & 19.564 & 0.0030 & --                  & --     & --                \\
J160109.36+144223.44 & STAR    & 1192206127354915328 & 19.229 & 0.0210 & --                  & --     & --                \\
J160130.77+153328.12 & EXGAL   & 1192324874611096704 & 20.166 & 0.0067 & --                  & --     & --                \\
J160149.22+442834.93 & EXGAL   & 1386282440898189952 & 19.665 & 0.0572 & --                  & --     & --                \\
J160248.49+445819.03 & EXGAL   & 1386346208276118656 & 20.307 & 0.0454 & --                  & --     & --                \\
J160304.68+201254.66 & STAR    & 1203509454782340096 & 19.713 & 0.0122 & --                  & --     & --                \\
J160333.94+545425.50 & EXGAL   & 1621333902083952896 & 20.317 & 0.0304 & --                  & --     & --                \\
J160354.06+551048.61 & EXGAL   & 1621346340309431936 & 20.509 & 0.1437 & --                  & --     & --                \\
J160454.71+204555.15 & EXGAL   & 1205053096093310080 & 19.760 & 0.0054 & --                  & --     & --                \\
J160508.01+432628.73 & STAR    & 1385229555434134784 & 19.998 & 0.3901 & 1385229555435660032 & 19.948 & 0.0581            \\
J160533.63+155148.15 & STAR    & 1198306149146422528 & 19.708 & 0.3389 & --                  & --     & --                \\
J160634.92+423545.32 & EXGAL   & 1384948247960757248 & 19.601 & 0.0026 & --                  & --     & --                \\
J160643.64+414803.36 & EXGAL   & 1383357843047373568 & 20.124 & 0.1578 & --                  & --     & --                \\
J160745.87+140533.68 & STAR    & 4458535769646731392 & 18.950 & 0.6865 & 4458535769646731392 & 18.924 & 0.6721            \\
J160800.44+154925.51 & EXGAL   & 1198194411277588352 & 20.381 & 0.0471 & --                  & --     & --                \\
J160836.22+182830.67 & STAR    & 1200079700057967488 & 19.557 & 0.1854 & --                  & --     & --                \\
J160902.63+540151.06 & EXGAL   & 1428978672131570816 & 19.864 & 0.0290 & --                  & --     & --                \\
J160941.42+183651.18 & EXGAL   & 1199917758314636416 & 20.015 & 0.0088 & --                  & --     & --                \\
J161004.93+435824.70 & EXGAL   & 1385310365244134784 & 20.508 & 0.8076 & --                  & --     & --                \\
J161008.89+543650.16 & STAR    & 1429011730496376576 & 20.454 & 0.2342 & --                  & --     & --                \\
J161036.98+560349.33 & STAR    & 1621863969769213824 & 20.482 & 0.0239 & --                  & --     & --                \\
J161104.80+185348.76 & EXGAL   & 1201430205277980416 & 19.984 & 0.0045 & --                  & --     & --                \\
J161129.04+545055.52 & EXGAL   & 1429038492436529280 & 20.243 & 0.0356 & --                  & --     & --                \\
J161142.67+563202.07 & EXGAL   & 1621893072466366208 & 20.420 & 0.0137 & --                  & --     & --                \\
J161148.26+191902.19 & EXGAL   & 1201655536442305408 & 20.428 & 0.0427 & --                  & --     & --                \\
J161227.48+541130.55 & STAR    & 1428949088396986240 & 20.164 & 0.9967 & 1428949088396986240 & 20.103 & 0.9768            \\
J161243.90+734002.52 & STAR    & 1702529949577302272 & 19.774 & 0.0199 & --                  & --     & --                \\
J161246.04+734310.12 & STAR    & 1702534656861478912 & 19.987 & 0.0095 & --                  & --     & --                \\
J161246.81+193654.83 & EXGAL   & 1201762326509314816 & 20.531 & 0.0191 & --                  & --     & --                \\
J161319.42+555847.42 & STAR    & 1429698680449262720 & 19.931 & 0.0032 & --                  & --     & --                \\
J161420.49+195512.01 & STAR    & 1201797549535567232 & 19.076 & 0.0285 & --                  & --     & --                \\
J161447.70+434026.88 & EXGAL   & 1385063460459050240 & 20.375 & 0.0482 & --                  & --     & --                \\
J161512.17+191346.76 & STAR    & 1201501398656186752 & 20.378 & 0.2987 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J161552.77+541859.83 & EXGAL   & 1428575598040988544 & 20.173 & 0.0061 & --                  & --     & --                \\
J161602.40+555736.43 & EXGAL   & 1429668546958717184 & 19.556 & 0.0072 & --                  & --     & --                \\
J161608.68+430546.45 & EXGAL   & 1382395353759994112 & 20.311 & 0.0066 & --                  & --     & --                \\
J161611.42+431729.52 & EXGAL   & 1382412224391708160 & 20.450 & 0.0120 & --                  & --     & --                \\
J161801.22+433526.57 & STAR    & 1382434936179070976 & 19.524 & 0.2721 & --                  & --     & --                \\
J161825.56+540205.04 & EXGAL   & 1428512582280616448 & 20.581 & 0.0142 & --                  & --     & --                \\
J161830.09+444620.10 & EXGAL   & 1385636507880907648 & 19.714 & 0.0020 & --                  & --     & --                \\
J161856.22+433253.56 & EXGAL   & 1382431672004189696 & 20.219 & 0.0268 & --                  & --     & --                \\
J161944.85+535502.37 & STAR    & 1428309447508058880 & 19.573 & 0.9962 & 1428309447508058880 & 19.533 & 0.9951            \\
J161952.96+540121.91 & EXGAL   & 1428521176511061504 & 19.573 & 0.0033 & --                  & --     & --                \\
J162002.44+434625.08 & EXGAL   & 1382440644191492608 & 20.184 & 0.0102 & --                  & --     & --                \\
J162025.36+432626.05 & EXGAL   & 1382373058586174208 & 20.396 & 0.1431 & --                  & --     & --                \\
J162039.27+433301.84 & STAR    & 1382376185322302976 & 19.947 & 0.0038 & --                  & --     & --                \\
J162306.01+421234.88 & STAR    & 1381315564622816768 & 19.991 & 0.0028 & --                  & --     & --                \\
J162310.50+425831.19 & sdX     & 1382202909161403776 & 17.767 & 0.2196 & 1382202909161403776 & 17.739 & 0.2809            \\
J162328.41+434742.57 & EXGAL   & 1382311790876254208 & 19.962 & 0.0029 & --                  & --     & --                \\
J162557.51+430616.91 & EXGAL   & 1381469049574501376 & 19.980 & 0.0071 & --                  & --     & --                \\
J162712.69+415642.13 & EXGAL   & 1381164141255825280 & 19.945 & 0.0035 & --                  & --     & --                \\
J162806.83+442232.44 & STAR    & 1406336841498355712 & 19.771 & 0.0751 & --                  & --     & --                \\
J162906.35+314411.95 & STAR    & 1324503352139208832 & 19.765 & 0.0037 & --                  & --     & --                \\
J162933.28+420554.82 & EXGAL   & 1405142050315878016 & 19.972 & 0.0073 & --                  & --     & --                \\
J163007.90+311318.06 & STAR    & 1324193839615574528 & 19.157 & 0.0149 & --                  & --     & --                \\
J163034.08+423257.85 & UNCLASS & 1405204000924351744 & 19.475 & 0.3554 & 1405204000924351744 & 19.441 & 0.9018            \\
J163053.92+305013.36 & STAR    & 1324125364951472256 & 19.802 & 0.3039 & --                  & --     & --                \\
J163205.86+312112.74 & EXGAL   & 1324280254357295232 & 19.791 & 0.0049 & --                  & --     & --                \\
J163226.10+424227.93 & EXGAL   & 1405183316361990272 & 20.092 & 0.0069 & --                  & --     & --                \\
J163233.57+323215.05 & EXGAL   & 1324930581125081984 & 20.284 & 0.0244 & --                  & --     & --                \\
J163335.47+325428.51 & EXGAL   & 1324963772632660608 & 20.583 & 0.0123 & --                  & --     & --                \\
J163539.37+215038.74 & EXGAL   & 1297733679976259328 & 20.456 & 0.0108 & --                  & --     & --                \\
J163558.62+324731.10 & EXGAL   & 1324854856556954240 & 20.400 & 0.0049 & --                  & --     & --                \\
J163638.01+222844.27 & EXGAL   & 1298061922853183616 & 20.424 & 0.0169 & --                  & --     & --                \\
J163803.38+371440.76 & STAR    & 1328363909262647936 & 19.203 & 0.0021 & --                  & --     & --                \\
J163835.64+754015.05 & STAR    & 1703189519115422848 & 19.818 & 0.5045 & 1703189519115422848 & 19.789 & 0.8424            \\
J163905.44+243307.29 & EXGAL   & 1300609250776857984 & 20.606 & 0.0326 & --                  & --     & --                \\
J164005.77+231724.97 & EXGAL   & 1299618723942775936 & 20.326 & 0.0235 & --                  & --     & --                \\
J164105.73+362701.86 & sdX     & 1328081300414229376 & 18.547 & 0.3064 & --                  & --     & --                \\
J164113.56+362440.44 & STAR    & 1328034094433278848 & 19.786 & 0.1826 & --                  & --     & --                \\
J164120.45+363159.14 & STAR    & 1328105420950722560 & 18.570 & 0.0038 & --                  & --     & --                \\
J164123.88+362824.74 & STAR    & 1328104669341383936 & 18.233 & 0.2520 & 1328104669341383936 & 18.200 & 0.1668            \\
J164125.48+364116.10 & sdX     & 1328111743142862720 & 18.699 & 0.4088 & --                  & --     & --                \\
J164127.13+304200.77 & UNCLASS & 1312295027858507776 & 19.325 & 0.0214 & --                  & --     & --                \\
J164128.19+362630.37 & STAR    & 1328057665213091968 & 17.774 & 0.2377 & --                  & --     & --                \\
J164132.07+363200.97 & sdX     & 1328105283517446016 & 18.735 & 0.3108 & 1328105283517446016 & 18.696 & 0.5493            \\
J164135.42+362242.91 & sdX     & 1328056428259951616 & 18.293 & 0.2352 & 1328056428259951616 & 18.263 & 0.3397            \\
J164144.25+363228.39 & sdX     & 1328059898596791040 & 17.918 & 0.4215 & --                  & --     & --                \\
J164152.65+362113.94 & STAR    & 1328053438961427200 & 19.794 & 0.2804 & --                  & --     & --                \\
J164154.91+214103.88 & sdX     & 4564373968662455296 & 18.376 & 0.4293 & 4564373968662455296 & 18.341 & 0.5224            \\
J164155.77+363124.51 & STAR    & 1328059967318072448 & 19.645 & 0.0232 & --                  & --     & --                \\
J164159.85+363051.42 & sdX     & 1328059207109557248 & 18.567 & 0.2191 & 1328059207109557248 & 18.539 & 0.2801            \\
J164204.09+362753.72 & STAR    & 1328058489852173440 & 18.331 & 0.2073 & 1328058489852173440 & 18.297 & 0.2458            \\
J164204.58+362854.22 & STAR    & 1328058558563274624 & 18.077 & 0.1338 & 1328058558563274624 & 18.045 & 0.1284            \\
J164205.79+233352.22 & STAR    & 1299720360048569344 & 19.453 & 0.0578 & --                  & --     & --                \\
J164207.13+362245.05 & STAR    & 1328053537746970112 & 18.293 & 0.2603 & 1328053537746970112 & 18.267 & 0.1999            \\
J164236.25+351432.32 & STAR    & 1326802190433968640 & 18.240 & 0.2369 & 1326802190433968640 & 18.205 & 0.1104            \\
J164338.93+232357.74 & EXGAL   & 1299515713446453248 & 20.465 & 0.0165 & --                  & --     & --                \\
J164445.97+344946.30 & sdX     & 1326961413461592064 & 19.975 & 0.7106 & 1326961413461592064 & 19.923 & 0.8178            \\
J164502.15+335131.81 & EXGAL   & 1326463064112148480 & 20.443 & 0.0360 & --                  & --     & --                \\
J164755.41+334232.56 & EXGAL   & 1314415023716081792 & 20.352 & 0.0219 & --                  & --     & --                \\
J164756.94+330848.84 & EXGAL   & 1314358914265521408 & 20.467 & 0.0099 & --                  & --     & --                \\
J164820.10+331451.83 & STAR    & 1314383481475856768 & 20.486 & 0.9694 & 1314383481475856768 & 20.400 & 0.8243            \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J164919.50+355019.53 & EXGAL   & 1327124141182389760 & 20.215 & 0.0062 & --                  & --     & --                \\
J164959.19+335459.82 & STAR    & 1314784768860340608 & 19.819 & 0.0034 & --                  & --     & --                \\
J165008.94+751423.11 & EXGAL   & 1656568851708181376 & 19.875 & 0.0056 & --                  & --     & --                \\
J165149.80+295600.71 & UNCLASS & 1311296843099487104 & 19.253 & 0.5794 & 1311296843099487104 & 19.215 & 0.4547            \\
J165259.37+352010.22 & STAR    & 1315030131752334336 & 20.076 & 0.9958 & 1315030131752334336 & 20.051 & 0.8650            \\
J165350.49+351120.26 & STAR    & 1314978901382346496 & 20.103 & 0.9524 & 1314978901382346496 & 20.043 & 0.9371            \\
J165449.45+350803.68 & EXGAL   & 1338982172225052544 & 20.549 & 0.1501 & --                  & --     & --                \\
J165458.42+343853.65 & STAR    & 1314756284638224256 & 20.632 & 0.8933 & --                  & --     & --                \\
J165503.73+340800.88 & EXGAL   & 1314663238465735296 & 20.363 & 0.0696 & --                  & --     & --                \\
J165504.38+345703.03 & EXGAL   & 1314957392186378496 & 20.504 & 0.0861 & --                  & --     & --                \\
J165519.60+351755.67 & STAR    & 1338985157226553216 & 18.501 & 0.9993 & 1338985157226553216 & 18.466 & 0.9958            \\
J165707.99+350922.88 & STAR    & 1338795628910635520 & 20.346 & 0.9983 & 1338795628910635520 & 20.274 & 0.9941            \\
J171123.71+581131.25 & EXGAL   & 1433925409305414272 & 19.563 & 0.0164 & --                  & --     & --                \\
J171150.74+564601.50 & EXGAL   & 1432993779359203200 & 20.459 & 0.0147 & --                  & --     & --                \\
J171441.60+593723.28 & sdX     & 1437257170054963968 & 18.834 & 0.8922 & 1437257170054963968 & 18.791 & 0.9632            \\
J171649.84+430746.62 & STAR    & 1360408183518422144 & 19.799 & 0.2900 & --                  & --     & --                \\
J171714.29+430414.26 & STAR    & 1360216662336535808 & 19.986 & 0.0080 & --                  & --     & --                \\
J171725.71+430734.40 & STAR    & 1360406018852501248 & 19.602 & 0.2512 & --                  & --     & --                \\
J171750.25+575912.79 & STAR    & 1433124586882588416 & 20.228 & 0.2913 & --                  & --     & --                \\
J171750.43+424648.54 & STAR    & 1360195973480645888 & 19.745 & 0.0221 & --                  & --     & --                \\
J171832.94+585242.20 & EXGAL   & 1434064841124171136 & 20.217 & 0.0062 & --                  & --     & --                \\
J172017.48+563831.41 & EXGAL   & 1420838815752506368 & 20.275 & 0.0201 & --                  & --     & --                \\
J172035.08+582559.70 & STAR    & 1433983717780810624 & 20.374 & 0.0047 & --                  & --     & --                \\
J172042.43+573955.47 & STAR    & 1433134211905291776 & 20.045 & 0.0252 & --                  & --     & --                \\
J172140.33+575132.10 & STAR    & 1433146615770880256 & 20.111 & 0.0145 & --                  & --     & --                \\
J172156.44+565639.97 & STAR    & 1432858745586804224 & 19.795 & 0.0120 & --                  & --     & --                \\
J172307.49+575355.35 & STAR    & 1433166578778742912 & 20.207 & 0.5113 & --                  & --     & --                \\
J172335.96+575642.78 & STAR    & 1433166918080289792 & 20.000 & 0.2078 & --                  & --     & --                \\
J172456.63+562220.42 & EXGAL   & 1420781812946981504 & 20.404 & 0.0987 & --                  & --     & --                \\
J172751.38+570834.42 & EXGAL   & 1422365006611803008 & 20.474 & 0.3116 & --                  & --     & --                \\
J175109.00+633030.88 & EXGAL   & 1439698017150198912 & 20.039 & 0.0037 & --                  & --     & --                \\
J175144.46+611729.83 & UNCLASS & 1436226824580848128 & 20.271 & 0.9917 & 1436226824580848128 & 20.216 & 0.9917            \\
J175158.77+692245.60 & STAR    & 1637843137895112832 & 19.822 & 0.0042 & --                  & --     & --                \\
J175303.30+810743.55 & EXGAL   & 1709865208259338752 & 19.823 & 0.0043 & --                  & --     & --                \\
J175709.15+623520.79 & EXGAL   & 1436549982215420800 & 20.329 & 0.0286 & --                  & --     & --                \\
J175832.85+624648.36 & STAR    & 1436569807785173248 & 20.421 & 0.8410 & 1436569807785173248 & 20.370 & 0.7602            \\
J175859.48+645338.88 & EXGAL   & 1440775955156103808 & 20.298 & 0.0089 & --                  & --     & --                \\
J175934.35+645636.09 & EXGAL   & 1440776706775349248 & 20.293 & 0.0103 & --                  & --     & --                \\
J175936.80+630943.00 & EXGAL   & 1436629348915645952 & 20.305 & 0.0162 & --                  & --     & --                \\
J180044.26+703508.30 & STAR    & 2260232689913880192 & 19.741 & 0.2194 & --                  & --     & --                \\
J180412.19+614646.05 & STAR    & 2159268144907700224 & 20.410 & 0.9905 & 2159268144907700224 & 20.342 & 0.9814            \\
J180441.77+614828.75 & STAR    & 2159274260941638400 & 20.173 & 0.8008 & 2159274260941638400 & 20.117 & 0.9063            \\
J180445.14+620706.93 & STAR    & 2159302985682708992 & 18.775 & 0.0028 & --                  & --     & --                \\
J180537.01+703317.48 & STAR    & 2260221596014838656 & 19.925 & 0.3968 & --                  & --     & --                \\
J180654.30+620159.13 & EXGAL   & 2159256874913786496 & 20.110 & 0.0165 & --                  & --     & --                \\
J180919.83+624716.86 & EXGAL   & 2160884225137681408 & 19.704 & 0.0052 & --                  & --     & --                \\
J180930.55+633808.79 & sdX     & 2161027226073503232 & 18.699 & 0.2406 & 2161027226073503232 & 18.665 & 0.1547            \\
J181038.72+625244.37 & EXGAL   & 2160703935294239232 & 20.415 & 0.0182 & --                  & --     & --                \\
J181114.81+645701.42 & EXGAL   & 2161399616917323904 & 20.484 & 0.0123 & --                  & --     & --                \\
J182555.71+352637.38 & EXGAL   & 2095598518920035456 & 20.442 & 0.0163 & --                  & --     & --                \\
J182728.79+353647.47 & UNCLASS & 2095626865704448000 & 20.664 & 0.0547 & --                  & --     & --                \\
J182941.64+341752.54 & EXGAL   & 2094552677204998528 & 20.057 & 0.0093 & --                  & --     & --                \\
J183005.57+332657.49 & EXGAL   & 4592450509178551040 & 20.316 & 0.0130 & --                  & --     & --                \\
J183045.31+343534.84 & UNCLASS & 2094581608109044864 & 20.269 & 0.0444 & --                  & --     & --                \\
J183138.48+354342.52 & EXGAL   & 2095499940830685056 & 20.531 & 0.0183 & --                  & --     & --                \\
J183337.58+353714.98 & EXGAL   & 2094736123847532160 & 20.475 & 0.0140 & --                  & --     & --                \\
J183928.53+344421.32 & EXGAL   & 2094765054747327872 & 19.986 & 0.0079 & --                  & --     & --                \\
J185909.46+645346.99 & UNCLASS & 2253686683015627776 & 18.680 & 0.8188 & 2253686683015627776 & 18.654 & 0.9287            \\
J190029.75+650130.73 & EXGAL   & 2253691493377444736 & 20.318 & 0.0240 & --                  & --     & --                \\
J190934.77+662231.74 & EXGAL   & 2254985064512092544 & 20.307 & 0.0172 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}

\clearpage

%\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\begin{table*}
\centering
\caption{\textit{Continued.}}
\begin{tabular}{llllllll}
\hline
WDJ name & WD type & Gaia DR2 source ID  & DR2 $G$ mag & DR2 $P_{\textrm{WD}}$ & Gaia DR3 source ID  & DR3 $G$ mag & DR3 $P_{\textrm{WD}}$ \\
\hline
J234437.96+275526.59 & sdX     & 2865318200950784768 & 18.833 & 0.3345 & --                  & --     & --                \\
%
\hline
\end{tabular}
\end{table*}
